CBR: Controlled Burst Recording

Collecting traces from software running in the field is both useful and challenging. Traces may indeed help revealing unexpected usage scenarios, detecting and reproducing failures, and building behavioral models that reflect how the software is actually used. On the other hand, recording traces is an intrusive activity that may annoy users, negatively affecting the usability of the applications, if not properly designed. In this paper we address field monitoring by introducing Controlled Burst Recording, a monitoring solution that can collect comprehensive runtime data without compromising the quality of the user experience. The technique encodes the knowledge extracted from the monitored application as a finite state model that both represents the sequences of operations that can be executed by the users and the corresponding internal computations that might be activated by each operation. Our initial assessment with information extracted from ArgoUML shows that Controlled Burst Recording can reconstruct behavioral information more effectively than competing sampling techniques, with a low impact on the system response time.

==> after rev/bursts.tex <==
% !TEX root =  main.tex

\section{Field Bursts}\label{sec:bursts}

% All this knowledge can be represented as a Finite State Automaton, or \FSA for short, where the states represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. 

% Since several monitoring techniques in the literature collect method calls, eventually annotated with parameters or state information~\cite{ohmann2017lightweight,Jin:BugRedux:ICSE:2012,joshi2007scarpe,prepost,Cornejo:Flexible:ICSEC:2017,Cornejo:DelayedSaving:IEEEAccess:2019}, we also focus on the collection of this data type.

% In a nutshell, \Controlled is an approach that combines chunks of execution recorded at different times to produce insights about the field behavior of the application. With this approach we might loss full ordering of the events in the \FSA model, but since we are going to record partial traces at different times of the execution we expect not to impact on the user experience.

%definire un burst, ne spieghiamo l’utilità e spieghiamo anche l’utilità di metterli assieme.

A \textit{burst} is a stream of consecutive events collected in the field enriched with the state information at the beginning and at the end of each user action. 
In particular, a burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two concrete states of the application, initial and final respectively, and the trace $T$ is the sequence of events collected in the field.

Collecting bursts instead of full traces is useful because it allow us to spend less resources at runtime, in other words, there is no need for the monitor to be always on; since the technique traces bursts signed with program state information, we are not forced to record sequentially all bursts that occur in the field, that would correspond to continuously collect all the program execution interfering with the user activities. The program state information helps us to acquire a logical order of the different independent bursts collected at different times during different executions under monitoring.

All the knowledge learned through the collected bursts can be used to elaborate a Finite State Automaton, or \FSA for short, where the nodes represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. This strategy is useful because it will support practitioners to construct and simulate program scenarios from field executions without impacting on the user experience.


==> after rev/cbr.tex <==
% !TEX root =  main.tex

\section{Controlled Burst Recording}\label{sec:cbr}

%\leo{spiegare il valore dell’informazione estratta dal campo.}

\Controlled is a technique that represents the possible executions of an application in a Finite State Automaton structure; since this approach does not record full executions we might loss the full ordering of field events, but still a good representation of the behavior of the application can be given. From the generated model it is possible to extract accurate and comprehensive traces that could be useful for post-deployment analysis such as debugging, field failures reproduction, protocol verification, among others.

Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques~\cite{walkinshaw2008inferring}, such as detection of anomalous behaviors, protocol verification, testing, among others.

Usually the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon}~\cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 


==> after rev/commands/commands.tex <==
\newcommand{\CODE}[5]{
\lstinputlisting[
     caption={#2},%
     label={#1},%
     basicstyle=\scriptsize\ttfamily,%
     showstringspaces=false,%
     frame={tb},%
     lineskip=-0.4pt,%
     extendedchars=true,%
     numbers=left,%
     numbersep=4pt, 
     stepnumber=1,%
     keepspaces=true,
     firstnumber=#4,
     numberstyle=\tiny,%
     xleftmargin=\parindent,%
     breaklines=true,
     language=#5,%
     tabsize=2,
     captionpos=b,
    backgroundcolor=\color{white},
    morekeywords={aspect,thisJoinPoint,around},
]{code/#3}
\vspace{0.3cm}

}

\newcommand{\JCODESTEP}[4]{
        \CODE{#1}{#2}{#3}{#4}{java}
}

\newcommand{\JCODE}[3]{
        \CODE{#1}{#2}{#3}{1}{java}
}

==> after rev/conclusions.tex <==
% !TEX root =  main.tex

\section{Conclusions}\label{sec:cbr_discussion}

\CBR extracts relevant information about the behavior of a software running in the field by collecting bursts of executions synchronously with the computations. That is, each burst corresponds to the processing of a user \begin{mod}operation\end{mod}. Moreover, each burst is annotated with state information collected at the beginning and the end of the burst: this allows \CBR to recombine the information present in the bursts and build a hierarchical model that well captures the behavior observed in the field for a target application. 

We conducted a case study based on Argo UML as preliminary evaluation.
%
%We have carried out an experimental evaluation for assessing the quality of \CBR in terms of monitoring \textit{performance} with respect to other two sampling approaches. 
%
%Since \CBR works in a probabilistic way and does not trace full executions, we also assessed the \textit{precision} and the \textit{recall} of the traces simulated by \CBR, to understand the usefulness of the sampling approach in an attempt to decrease monitoring overhead and to reduce the impact on the user environment.
When assessing performance, we discovered that the overhead introduced by \CBR (in the worst case) with respect to other sampling approaches can be higher for short operations, but similar for the other operations. The higher overhead for short actions is relatively harmless, since it can be hardly recognized by users~\cite{NIER17, Cornejo:FunctionCallMonitoring:JSS:2020}.

When assessing the quality of the extracted information, we discovered that \CBR can reconstruct behavioral information more effectively than sampling techniques, which are highly precise but can hardly produce a fairly comprehensive picture of the observed behaviors. 
Thus, \CBR succeeds in recording useful field data with hardly recognizable impact on the system response time of the monitored application.

As part of future work, we would like to extend the empirical evaluation with other applications and case studies, as well as exploiting the information that can be effectively collected in the field to support program analysis tasks.

==> after rev/controlledbust.tex <==
% !TEX root =  2018-PhDThesis-OscarCornejo.tex

\chapter{Controlled Burst Recording}\label{chapter:cbr}

This chapter presents \Controlled, a sampling technique for monitoring applications and for inferring knowledge from field executions with little impact on the user experience. This solution has been designed based on the results obtained with the user study we conducted for understanding the impact of monitoring on the user experience. This chapter presents also an empirical evaluation carried out on a real world application for assessing the efficiency and the quality of the approach, compared to other sampling-based techniques.

The presentation of the chapter is organized as follows. Section \ref{sec:inferring} presents an overview of the technique. Section \ref{sec:CBR} presents the \Controlled Framework and its different steps. Section \ref{sec:empirical_cbr} presents the empirical validation we conducted to assess our technique. Finally, Sections \ref{sec:cbr_results} and \ref{sec:cbr_discussion} discuss the obtained results and findings respectively.

\section{Inferring Knowledge from Field Executions}\label{sec:inferring}

\Controlled, or \textit{CBR} for short, is a technique to collect partial traces from the field. These traces could be used to produce a comprehensive knowledge about how an \textit{object-oriented} application is used by different users in a wide range of possible scenarios and configurations. 
In general, our goal is to efficiently monitor interactive applications, that is, applications that continuously interact with users. Since \CBR is \textit{user-oriented} we aim to monitor traces that start and finish with a user interaction.

Sampling-based techniques are useful to lower the monitoring overhead, since the amount of samples gathered from field are strongly reduced in a probabilistic way. In literature, sampling techniques have been widely used for isolating bugs \cite{Liblit:BugIsolation:SIGPLAN:2003,Jin:Sampling:SIGPLAN:2010}, runtime verification \cite{Bartocci:Adaptive:ICRV:2012,joshi2017runtime,BabaeeGF18} and bursty monitors \cite{Hirzel:BurstyTracing:FDDO:2001} (as described in Chapter \ref{chapter:related}).

\CBR has been designed based on the results obtained in the user studies presented in Chapter \ref{chapter:userstudy}. 
Interestingly, we discovered that users hardly perceive important overhead levels if introduced for a limited time (see Section \ref{sec:overheadTolerant}), in particular, we observed that even for overhead levels of 140\% users struggle to recognize variations in the system response time with the exception of some long lasting operations. 

\CBR leverages these results: since a significant overhead can often be tolerated by users, traces of non-trivial length might be feasibly collected from the field, but at the same time, since the impact of the monitoring activity changes with the operation that is executed, monitoring must be cleverly limited to prevent the introduction of an excessive overhead for specific operations.

Given \textit{EV} as the set of every possible event that can be produced by a monitored application, a trace 
$T = \langle e_1,e_2,...,e_n \rangle$, with $e_i \in \textit{EV}$, $i = 1\ldots n$ is an ordered sequence of events observed in the field. 

In order to obtain a comprehensive information about the sequentiality of the traces, we might collect state information at the moment the execution traces are collected in the field.  

All this knowledge can be represented as a Finite State Automaton, or \textit{FSA} for short, where the states represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. 

Since several monitoring techniques in the literature collect method calls, eventually annotated with parameters or state information \cite{ohmann2017lightweight,Jin:BugRedux:ICSE:2012,joshi2007scarpe,prepost,Cornejo:Flexible:ICSEC:2017}, we also focus on the collection of this data type.

In a nutshell, \Controlled is an approach that combines chunks of execution recorded at different times to produce insights about the field behavior of the application. With this approach we might loss full ordering of the events in the \FSA model, but since we are going to record partial traces at different times of the execution we expect not to impact on the user experience.

In the following section, we present an overview of \Controlled and the main steps of the approach.

\subsection{Overview of the Technique}\label{sec:cbr_overview}

\begin{figure}[h!]
  \centering
    \includegraphics[width=\textwidth]{figures/CBR}
    \caption{Overview of \Controlled approach.}
    \label{fig:CBR}
\end{figure}

Figure \ref{fig:CBR} shows the steps that must be performed to apply \CBR. 

To start, practitioners indicate to \CBR the components they would like to monitor in the field. To extract data from the chosen components, \CBR identifies all the classes that may influence the usage of the components (step 1).

This analysis is done by first selecting a subset of the system (e.g., component) that has been defined as the monitoring goal and then by retrieving all the \textit{relevant classes} and their respective methods that exist inside the selected component, which is the result of step 1.

Given that \CBR has been designed to \textit{sample} executions from the field, in order to decrease monitoring overhead, we can use program state information to give a temporal context to the different traces by calculating the state of the program before and after the set of events observed in the field.

This state information should be accurate enough to recognize different application states between user inputs, and inexpensive enough to be obtained at runtime so it does not add too much monitoring overhead.

One way to represent the state of an application is to consider the set of values of all the variables at a certain moment \textit{t} during the execution. Certainly, acquiring this information is too expensive to be done at runtime.  
An efficient way to perform this operation, is to subset the number of variables and the amount of information \CBR should save for each variable while monitoring.

In the Function Extraction step (see Section \ref{sec:SD}), \CBR analyzes the relevant classes to distill the knowledge about the functions that may influence their execution, and thus influence the interaction with the monitored components. In particular, \CBR identifies a set of functions to be used to derive an abstract representation of the current state: we call the set of functions the \textit{Abstraction Functions}, or \textit{AF} for short.

The most intuitive way to derive the \AF, is to extract from the application's code the functions that the application uses to define its execution path according to the runtime value of the variables. \CBR will only consider those functions that helps to differentiate efficiently between different states at runtime. 

For instance, let us assume that the monitored components control the interaction with the file system: if a method \texttt{write} may actually write to a variable \texttt{file} only if its boolean variable \texttt{open}, which represents if the file has been already open or not, is true, 
the Function Extraction step would output the function \texttt{file.open == true} to indicate that the evaluation of this function may influence the interaction with the monitored components. 
In general, the \AF can capture important state information that could be useful to understand how the application under monitoring changes its state according to user inputs.

The \AF are systematically applied to concrete states of the application to produce an abstract representation of the program state to which they were applied: these representations are called \textit{Abstract Program States}, or \textit{APS} for short.

The \AF should have a proper balance in the abstraction level: too concrete functions can have bad implications, for instance checking all the field values of the program variables would be too expensive to be assessed at runtime (\textit{performance}). 
On the other side, too abstract functions could generate poor program states that are not useful to distinguish different states of the application while running in the field (\textit{precision}).

\smallskip

After having defined the \AF through an automatic extraction process (see Section \ref{sec:SD}), the monitor is then assembled: 
the monitoring component consists of the State Monitor and the Event Monitor. The State Monitor produces concrete values of the \AF at the beginning and at the end of each stream of events, and the Event Monitor collects the events associated with the component under monitoring.

To start using the State Monitor, we need to pass through a Training Phase (step 3) to produce the optimal set of functions for estimating a proper representation of the state of the program. These steps are described in details in Section \ref{sec:monitor}.

Then, in the field, \CBR uses the Abstraction Functions to produce a compact and relevant representation of the state of the program, immediately before and after a stream of events is recorded (step 4). 

A \textit{burst} is a stream of consecutive events collected in the field enriched with the state information at the beginning and at the end of each user action. 
In particular, a burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two \APS produced by the \AF and the trace $T$ is the sequence of events collected in the field.

Since \CBR is implemented as a sampling technique, the different bursts are collected probabilistically by turning on and off the monitor while running in the field.

The evaluation of the Abstraction Functions to a concrete state of the program during runtime (i.e., the \APS) is used within bursts to represent the state of the application at a certain point of the execution.

The collected bursts are then analyzed offline. The \APS at the beginning and at the end of each burst abstractly represent the state of the system at the time the trace was recorded. 
Since a program state directly depends on the conditions actually computed by the program while interacting with the monitored components, the \APS is representative of how the execution may proceed, specifically in terms of the interaction with the monitored components. 

In principle, a set of bursts might be used to form a Finite State Automaton, to show real uses of the application (step 5), where the edges of the \FSA represent the different user actions and the nodes represent the possible program states. Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques \cite{walkinshaw2008inferring}, such as detection of anomalous behaviors, protocol verification, testing, among others.

%%Literature on FSAs

The literature on synthesizing \FSAs that describe the behavior of a system is vast, some particularly relevant works include Wil van der Aalst's \cite{van2016process} book, entirely devoted to mining processes from observed data. 
Also, Lorenzoli et al. \cite{lorenzoli2008automatic} worked on \textit{GK-Tail}, a technique for automatically generating extended finite state machines from interaction traces. The technique focuses on the relations between constraints on data values on component interactions, retrieving more accurate models for analysis and testing techniques.
In the same direction, Krka et al. \cite{krka2010using} developed a \FSA inference technique that uses not only execution traces but also program invariants in order to obtain relevant internal state information of the program variables and to produce more reliable models. 
Recently, Walkinshaw et al. \cite{walkinshaw2016inferring} proposed an approach for inferring extended \FSAs from software executions, this work focuses on addressing the non-determinism and the inflexibility problem of automatically generated \FSAs.

Usually the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon} \cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 

To create the \FSA, we merge the different bursts collected in the field that have a common state, intuitively a burst that ends with a certain state can be concatenated with a burst that starts with the same abstract program state, because it represents two consecutive actions performed by the user in the application.

The main reason for generating these \FSA is representing the possible executions of an application, which may be useful to analyze the scenarios that may occur in the field.

\section{\Controlled Framework}\label{sec:CBR}

The most important activity performed by \CBR is the identification of the functions that are later used to represent the Abstract Program State, that is, a compact and abstract representation of the state at the time the collection of a burst is started or stopped.

In this section, we use a small example to present the different steps of \Controlled Framework. 

Consider a Java program that includes the \texttt{Cart} class (see Listing \ref{code:cart_class}), which represents a shopping cart of an online store. The \texttt{Cart} class implements four different methods and the \texttt{Product} inner class: 
the \texttt{addItem} method adds a \texttt{Product} object to the shopping cart, which is represented by an array of \texttt{Product} type,
the \texttt{emptyCart} method empties the shopping cart,
the \texttt{calculateTotal} method estimates the total price of all the products in the cart and
the \texttt{applyDiscount} method applies a discount to the total price.

Let us assume that we want to collect data about how a certain program uses the \texttt{Cart} class, focusing on the sequences of method calls produced by the program. Capturing every call to every method of the \texttt{Cart} class might be expensive for operations that extensively use the public methods implemented by the \texttt{Cart} class.

\JCODESTEP{code:cart_class}{Shopping Cart Class}{Cart.java}{1}

\subsection{Step 1: Classes Identification}

The \textit{Classes Identification} step produces the set of classes that directly or indirectly determine the sequence of invocations to the methods in the monitored component. To derive the set of classes, practitioners need to indicate the component(s) of interest within the application under monitoring. Since one of the goals of \CBR is to generate as little monitoring overhead as possible, it is important to include under the monitoring objective only those classes that are directly involved within the functionalities being monitored.

The set of classes is determined statically by extracting from the monitored component all the classes that exist inside the program.
Then, with the help of WALA \cite{WALA} static analysis tool, \CBR constructs the Class Hierarchy of the program under monitoring and extracts all the classes that match the scope of the monitoring. 

Later, we save the meta-data of all methods existing inside the classes we already gathered through the Class Hierarchy.

In our example, we are interested in understanding the behavior of the class \texttt{Cart}, so \CBR considers the \texttt{Cart} and its \texttt{Product} inner class for the analysis.

\subsection{Step 2: Function Extraction}\label{sec:SD}

\CBR uses the classes produced during the step 1 to extract the \textbf{Abstraction Functions} that represent how the value of the state variables that may influence the execution of the monitored program. These functions are exploited at runtime to record state information efficiently, that is, representing the state of the application with a proper abstraction level so we avoid performance and precision issues as stated in Section \ref{sec:cbr_overview}.
% abstractly with a limited risk of losing information relevant to the program.

The Abstraction Functions computed by the monitored program, and in particular the ones computed in the relevant classes, are a set of functions that can be naturally exploited to define an efficient abstraction strategy that can be applied at runtime to generate the program state.

\begin{figure}[h]
  \centering
    \includegraphics[width=0.9\textwidth]{figures/abstract_functions}
    \caption{Function Extraction process.}
    \label{fig:abstract_functions}
\end{figure} 

To extract the Abstraction Functions from the code (see Figure \ref{fig:abstract_functions}), we symbolically execute each method in each selected class and use the \textit{path conditions} resulting from the analysis of each method as functions for state abstraction. 
A \textit{path condition} is a condition on the state variables of a program, and the Abstraction Functions are the application of these conditions to the program state.

We use the JBSE \cite{Braione:Enhancing:FSE:2013} symbolic executor to compute the Abstraction Functions from the relevant classes, bounding the exploration of loops. 

Note that a \textit{path condition} represents how the inputs to a method, that is, the values of the parameters and the values of state variables, relate to the execution of a specific path inside the method. \textit{Path conditions} are a good abstraction because they show how applications use inputs and state variables.

For instance, the Abstraction Functions could be composed by a particular function that
checks if the number of products in a shopping cart is greater than zero to decide how to use the shopping cart,
in this case it would be enough to record whether the condition \texttt{nrProducts > 0} is true or not when saving state information, with no need of recording the actual number of products, which would be irrelevant to determine how the execution may proceed.

The Abstraction Functions capture relevant state properties and represent the different execution paths, that in turn may produce different sequences of invocations to the monitored classes.  
Each evaluation of these functions at runtime produces the program state of the application.

From our \texttt{Cart} class example, the resulting Abstraction Functions include the following functions for each method:

\JCODESTEP{code:addItem}{Functions for method addItem}{addItem_2.log}{1}

\JCODESTEP{code:applyDiscount}{Functions for method applyDiscount}{applyDiscount_1.log}{1}

\JCODESTEP{code:calculateTotal}{Functions for method calculateTotal}{calculateTotal_1.log}{1}

\JCODESTEP{code:emptyCart}{Functions for method emptyCart}{emptyCart_1.log}{1}

Applying the Abstraction Functions to a certain program state produces a compact vector of ternary values: the size of the vector depends on the number of functions that are evaluated and the values are the result of the evaluation of a function to the current program state. The result of the evaluation of a function can be True (T), False (F), and Unknown (U). The vector of ternary values is called the Abstract Program State. 

A single function evaluates to true if the values of the program variables at the time the function is evaluated satisfy the function. 
Similarly, a function evaluates to false if the values of the program variables at the time the function is evaluated do not satisfy the function. 
If some of the elements that appear in a function cannot be evaluated, for instance because an object with an attribute that should be considered in the evaluation of a function is null or even non existing, the function evaluates to unknown. 

From our example, the Function 1 in Listing \ref{code:addItem} for the method \texttt{addItem}:

\smallskip
\noindent \begin{small}\texttt{Cart.nProducts != 0 \&\& Cart.products.length >= 0}\end{small}
\smallskip

evaluates to true when there is more than one \texttt{Product} in the shopping cart, while it evaluates to false if the shopping cart is empty. Finally, it evaluates to unknown if the \texttt{Cart} object is not available.

In the other hand, for example the Function 4 in Listing \ref{code:applyDiscount} for the method \texttt{applyDiscount} :

\smallskip
\noindent \begin{small}\texttt{Cart.nProducts > 0 \&\& Cart.products.length > 0 \&\&} \newline\texttt{Cart.products.[0].value < Cart.PRICE}\end{small}
\smallskip

evaluates to true when the cart is not empty, and the price of the first \texttt{Product} in the cart is higher than the \texttt{PRICE} constant, evaluates to false whether the cart is empty or the price of the first \texttt{Product} is lower than the \texttt{PRICE} value, and evaluates to unknown when the object Cart does not exist in memory.

When the program under monitoring is executed, \CBR produces a number of bursts consisting of an evaluation of the extracted functions on the state of the program, a sequence of events (each event is a method invocation), and again an evaluation of the functions on the state of the program. 

The organization \texttt{state - burst - state} is useful, because allows \CBR to understand the sequentiality of bursts. Since the states give information about the current program state, it is possible to correlate different bursts collected at different times and compare their states' values, to obtain a more comprehensive knowledge rather than considering only one burst.

Considering the previous example of the program exploiting the \texttt{Cart} class, a burst of its execution could take the form:

\smallskip
\noindent \begin{small}\texttt{(U, U, F, T) addItem(product) calculateTotal() \ldots emptyCart() (T, T, F, T)}\end{small}
\smallskip

where the part between parentheses is the Abstract Program State, which includes the evaluation of every function identified in the function extraction analysis (T, F, U stand for true, false, and unknown, respectively), and the sequence of labels between the two instances of the Abstract Program State is the sequence of events collected at runtime.

Considering the initial Abstract Program State (i.e., the first \APS of the burst), let us assume that the first value refers to the mentioned Function 1 on the method \texttt{addItem}: the U in the program state means that, when the monitor started that trace recording, that function was evaluated as unknown, while at the end of the trace it turned to be true.

\subsection{Step 3: Training Phase}\label{sec:monitor}

The symbolic executor produces a large number of path conditions since it tries to assess every possible execution path for every method under analysis. Including all path conditions to represent the \AFs is not practical, since evaluating a high number of functions at every user interaction might introduce infeasible levels of overhead, and thus affecting the user experience. For this reason, we need to filter out the path conditions produced by the symbolic executor to reach a good compromise between the accuracy of the state information that is traced and the cost of producing such a state information.

From the original set of path conditions, we are interested in those giving unique information about the behavior of the application, that is, information that is not subsumed by the information checked by other functions. 
To find the optimal set of conditions, we need to go through a training phase that consists in empirically finding all the \AFs that are useful for distinguishing the different logical states of the program as identified by the functions themselves. 
In other words, we run the application with a monitor that assesses the complete set of \AFs returned by the symbolic executor to obtain the most representative result for the \AF.

In this training phase, we evaluate the \AF for every method call performed by the application, to clearly distinguish all different Abstract Program States at runtime.  

% \leo{total number of function evaluations (credo...)}

% $E = E_{ij}^1, E_{ij}^2, \ldots, E_{ij}^{}$

For each user execution $l$ we generate a matrix $E_{iJ}^l$, with $i = 1 \ldots k_l$ being $i$ a sample observed in the field with $k_l$ being the number of samples observed in the $l$-th execution, and $J = 1 \ldots n_{af}$ being $J$ the abstraction functions under observation and $n_{af}$ the total number of \AFs.
For instance, in Figure \ref{fig:samples} we show two examples of executions, with $n_{af} = 7$, collected in the field: Execution 1 ($E^1$) with $k_1 = 3$ and Execution 2 ($E^2$) with $k_2 = 2$. 

\vspace*{-0.5cm}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/samples}
\caption{Example of two executions collected in the field.}
\label{fig:samples}
\end{figure}

After collecting information for each execution, we organize the several $\{ E_{ij}^1, E_{ij}^2, \ldots, E_{ij}^{L} \}$ with $L$ the total number of executions, into a matrix $M_{ij}$, where $i$ (rows) ranges from $1$ to the sum of all samples 
$\sum_{l = 1}^L k_l$
gathered at runtime, while $j$ (columns) goes from $1$ to $n_{af}$.
The matrix $M_{ij}$ is obtained as $M = \{E^1 \diamond E^2 \diamond \ldots \diamond E^{L}\}$, where the $\diamond$ operator represents the vertical concatenation of the $E_{iJ}^l$ matrices.
For instance, considering $E^1$ and $E^2$ the executions of our example, the operation $E^1 \diamond E^2$ would generate the matrix presented in Figure \ref{fig:matrix}.

\vspace*{-0.5cm}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/matrix}
\caption{Vertical concatenation of executions $E^1$ and $E^2$.}
\label{fig:matrix}
\end{figure}

During the filtering process, we can apply four type of operations to the matrix $M$ in order to remove samples or \AFs.
Particularly, we identify four operations: \textit{Duplicated Sample}, \textit{Non-Discriminating Abstraction Function}, \textit{Equivalent Abstraction Function} and the \textit{Redundant Abstraction Function} operation.
In Figure \ref{fig:pc_filtering} we show an example of the filtering process and its several steps until we arrive to the reduced matrix, the example starts with the matrix generated in Figure \ref{fig:matrix}.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{figures/pc_filtering}
\caption{Example of filtering process of \AF.}
\label{fig:pc_filtering}
\end{figure}

\textit{Duplicated Sample} is the case in which two samples obtained the same value for all the \AFs. Formally, two samples $M_{I_{1}j}$ and $M_{I_{2}j}$ are duplicated if $M_{I_{1}j} = M_{I_{2}j}$ for all $j = 1 \ldots N$.
% in other words that two rows $i$ and $i+1$ in the matrix $M$ are equivalent for all the \AF such that $M_{ij} = M_{(i+1)j}$.

In our example, in the first matrix we identified Duplicated Samples, in fact Sample 2 and Sample 3 are identical $S_2 = S_3 = \{U, F, T, T, F, F, F\}$, in general we remove the second occurrence of a repeated column/row, so in this case we remove Sample 3. 

\textit{Non-Discriminating Abstraction Function} are those abstraction functions that do not change their values throughout the different samples and thus are not useful to distinguish the program states at runtime. More formally, an abstraction function $af_J$ is non-discriminating if $M_{1J} = M_{2J} = \ldots = M_{IJ}$
 % that exist a column $j$ in the matrix $M$ in which its value is always constant such that $M_{ij} = M_{(i+1)j} = \ldots = M_{mj}$. 

In the second matrix, it is possible to recognize two Non-Discriminating Abstraction Functions, in this case $AF_1$ and $AF_3$, because they always generated the values $U$ and $T$, respectively.

\textit{Equivalent Abstraction Function} is the case in which there are two abstraction functions always produce the same set of abstract values. More formally, two functions $af_I$ and $af_J$ are equivalent if their columns $M_{iI}$ and $M_{iJ}$ are the same, that is, $M_{iI} = M_{iJ}$ for all $i=1...M$.

%in other words, that exist two columns $j$ and $j+1$ in the matrix $M$ that are equivalent such that $M_{ij} = M_{i(j+1)}$.

In the example, it is possible to recognize two equivalent abstraction function, since the abstraction function values represented in column $AF_6$ are already present in column $AF_2$ ($AF_2 = AF_6 = \{U, F, F, F\}$), in this case we remove column $AF_6$.

Finally, the \textit{Redundant Abstraction Function} reduction is a heuristic step that aims to remove those \AFs that are not useful for identifying unique program states. The reduction procedure works by removing one abstraction function at a time and checking if the function was necessary to distinguish a unique program state. 
The procedure consists of removing one column $j$ of the matrix $M$ and applying the \textit{Duplicated Sample} procedure: 
if the number of rows of the new matrix is equivalent to the original matrix $M$, it means that the \textit{removed abstraction function j} is not useful for recognizing a unique program state, 
otherwise, if the number of rows of the new matrix is less than the matrix $M$ it means that the \textit{removed abstraction function} is actually useful and we then reincorporate it to the matrix $M$.

In our example, \CBR attempts first to remove the column $AF_2$. Since $AF_2$ is not useful, $AF_2$ is removed. Along with column $AF_2$, \CBR also removes $AF_4$.

\CBR performs these operations iteratively until it arrives to a minimal representation of the executions with respect to the different \AFs given by the symbolic executor: 
in this example the minimal set is composed by abstraction functions $AF_5, AF_7$ and executions $1, 2, 4$ and $5$.
These \AF are used to generate a monitor that is able to collect bursts during program executions. 

\subsection{Step 4: Bursts Collection}\label{sec:collect_bursts}

One possible way to decrease the overall monitoring overhead in the field is to collect data in a probabilistic way, that is, to record information about an event only under a certain probability.

From our human-subjects study presented in Chapter \ref{chapter:userstudy}, we discovered that for a few actions it is actually possible to monitor applications in the field without impacting the user experience. 
So it makes sense to collect data occasionally when a user performs an action. Also, the monitoring of each burst starts by recording as soon as the user interacts with the application and it stops when the software finishes processing the user request.

The collection of bursts is done probabilistically: since the technique traces bursts of the execution signed with program state information, we are not forced to record sequentially all bursts that occur in the field, that would correspond to continuously collect all the program execution interfering with the user activities. The program state information helps us to acquire a logical order of the different independent bursts collected at different times during different executions under monitoring.

The sampling probability of \CBR will be then estimated experimentally, testing with different probabilities to search for the best cost-benefit compromise in terms of quality of the solution.

% Given \textit{EV} as the set of every possible event that can be produced by a monitored application, a trace 
% $T = \langle e_1,e_2,...,e_n \rangle$, with $e_i \in \textit{EV}$, $i=1\ldots n$ is an ordered sequence of events observed in the field. 

Let $Abstraction$ be the \AF that applied to a certain concrete state $S$ of a program produces an Abstract Program State $S_a = Abstraction(S)$.

% A burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two abstract program states produced by the \AF and the trace $T$ is the sequence of events collected in the field.

Following our example, some of the recorded bursts may for example look like:

\smallskip

\noindent \begin{small}\texttt{(U, F) cart.applyDiscount() cart.calculateTotal() \ldots (F, F)}\end{small}
\smallskip

When the action \textit{pay total} is performed, \CBR saves the \APS $(U, F)$ plus the target methods of the analysis, then \CBR saves again a new representation of the \APS equal to $(F, F)$.

\subsection{Step 5: \FSA Synthesis and Traces Simulation}\label{sec:simulating}

At this point, we already gathered several independent bursts from the field, where each burst explains the effect of each user action on the program state. 
The issue is that each burst by itself provides partial information about a full execution.
To overcome this issue, \CBR puts together all the bursts in a common structure. 

The right structure to assemble the different bursts is a \textit{Finite State Automaton}: in fact, a \FSA is a natural representation for traces with states and transitions. In our case, the \FSA will show how the application's state changes according to different users' inputs.

To decide how to synthesize the \FSA, \CBR exploits state information contained in the different bursts. 
That is, if a burst $B_1$ ends with an abstract program state $S_2$ that matches the abstract program state $S_1$ reported at the beginning of another burst $B_2$, then the two bursts $B_1$ and $B_2$ can be concatenated by a node containing the state information in common between both bursts.

The Finite State Automaton is a tuple $G = (S,M,s_0,s_F)$, 
where $S$ is a finite non-empty set of nodes representing the different \APS identified at the beginning and at the end of each burst,
$M$ is a finite set of transitions between states in $S$ representing the different user inputs monitored at runtime,
$s_0 \in S$ is the initial state, and $s_F \subset S$ is the set of final states.

So, for each monitored burst $B = \langle label, S_1\,T\,S_2 \rangle$, \CBR creates a transition $m \in M$ starting from state $S_1$ to $S_2$ with a specific label and a trace $T$. 
Since it is totally possible that different users perform the same action in different scenarios, \CBR enriches the transition $m$ with more traces $T$. 

% \leo{Inoltre devi dire come ogni elemento viene definito. Ad esempio il set di stati sara l'unione di tutti gli stati che occorrono all'inizio e fine dei burst. Poi per ogni burst <label, S1 T S2> creerai una transizione da S1 a S2 con etichetta label e annotazione T. Se ci sono piu burst con stesso valore di label S1 e S2 a questo punto l'annotazione viene arricchita con altri T}

The procedure of concatenating bursts is done iteratively for all bursts collected in the field. Certainly, as more bursts are used to create the graph, an increased number of program behaviors will be represented in it.

To simulate possible traces of the application we again exploit state information. 
Since we already built the \FSA as the tuple $G = (S,M,s_0,s_F)$, the procedure is straightforward: 
consider two transitions $m_1, m_2 \in M$ connected by a common state $S_1 \in S$, \CBR generates a new burst $B'$ with (1) the initial state $S_i$ of transition $m_1$, (2) a new trace $T'$ made by the concatenation of the trace $T_1$ from $m_1$ with the trace $T_2$ from $m_2$ and (3) the final state $S_f$ of transition $m_2$.
The new burst $B' = \langle label, S_i\,T'\,S_f \rangle$ contains the simulated trace represented by $T'$.
% for a certain state $S_k$ in $G$ we pickup an incoming $m_{in}$ and an outgoing transition $m_{out}$, from both transitions respectively we select the bursts $B_{incoming}$ and $B_{outgoing}$ and merge them by concatenating the traces $T_{incoming}$ inside $B_{incoming}$ with the events $T_{outgoing}$ inside burst $B_{outgoing}$. 

The idea is to repeat this process until a larger trace is created.

\begin{figure}[h]
\centering
\includegraphics[width=0.70\textwidth]{figures/burst_plus}
\caption{Example of simulation of traces.}
\label{fig:burst_plus}
\end{figure}

In Figure \ref{fig:burst_plus}, for our example we have two transitions: actions \textit{clickOnAddItem} and \textit{clickOnPay}, that have in common the \APS \texttt{(U, F)}. In this case, we might concatenate Bursts 1 and 2 and produce the following trace:

% \danyB{questa e' la parte che puo' generare tracce sbagliate giusto? lo accennerei qui per poi riprenerlo dopo nella valutazione}

\smallskip
\noindent \begin{small}\texttt{(U, U) cart.addItem(product1) \ldots cart.applyDiscount()\newline cart.calculateTotal()} \texttt{\ldots (F, F)}\end{small}
\smallskip

The generated traces could represent possible behaviors of the application, nevertheless if the quality of the model is not good, the procedure could derived unfeasible traces. This aspect will be covered in the next section.  

In a nutshell, \CBR provides useful information at two different levels:
(1) shows how the application is used in the field (\FSA) and 
(2) through the traces simulated by the \FSA shows different possible uses of the component under monitoring.

\subsubsection{\CBR model validity}\label{sec:precision}

For evaluating the validity of the \CBR model we consider two aspects: \textit{precision} and \textit{trace-level recall} of the traces generated by \CBR.

The building process and the semantics of the \FSA has a direct relationship with the precision of the technique. In some cases, it is possible that the generated traces are behaviors that do not occur in the field, which is the reason why we need to assess the precision of the generated \FSA.

Particularly, to evaluate precision we check if the traces produced by the \FSA model are possible outcomes of the application, in other words, we check if the derived traces from the \FSA model exists in the original trace.

The precision is evaluated first locally (i.e., \textit{node precision}) and then globally (i.e., \textit{overall node precision}), in other words, we first assess if the local decisions taken in each node of the \FSA are right. 
The assumption is that if on average the local decisions taken for each node are right, so the decisions taken globally by an execution derived from the model is also probably right.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/node}
\caption{\FSA node with state information and incoming and outgoing transitions.}
\label{fig:node}
\end{figure}

To assess \textit{node precision}, for each node present in the \FSA model we check that every possible sequence is a possible program behavior or not. 
For example, for the node in Figure \ref{fig:node} we first generate all the possible combinations of sequence of actions, that is, $A_1 \rightarrow B_1$, $A_1 \rightarrow B_2$, \ldots, $A_3 \rightarrow B_3$, then we verify if the traces produced by these sequences are present in the reworded traces, that is, traces recorded with a monitor that collects all the events sequentially.

The node precision for a particular node $i$ is estimated with the following formula:
\begin{equation}
	Precision(node_i) = \frac{CS_i}{TS_i}\label{eq:precision}
\end{equation}

where $CS_i$ is the amount of correct sequences for the node $i$ and $TS_i$ is the total of possible combinations of sequences for the node $i$.
The \textit{overall node precision} is obtained by estimating the mean \textit{node precision} of the \FSA model, for simplicity in the rest of the document we refer to \textit{overall node precision} simply as \textit{precision}.

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/completeness}
\caption{Recall validation process.}
\label{fig:recall}
\end{figure}

The \textit{trace-level recall} is assessed by estimating how complete are the traces generated by the technique with respect to the original trace. In the rest of the document we refer to \textit{trace-level recall} simply as \textit{recall}.

In particular, we incrementally consider the single events contained in the original trace, checking if the incremental trace is accepted by the \FSA (see Figure \ref{fig:recall}). We thus estimate the recall of the longest trace accepted by the \FSA model.

Particularly, the recall for a trace $j$ is estimated with the following formula:

\begin{equation}
	Recall(trace_j) = \frac{E_j}{EO_j}\label{eq:recall}
\end{equation}

where $E_j$ is the number of events contained in the generated trace $j$, and $EO_j$ is the number of events in the original trace representing the execution of trace $j$.

\subsubsection{Finite State Automaton Example}

Since the final step of the technique consists in generating a \FSA and then producing simulations of possible field executions, we show an example of a possible \FSA and how we assess the validity of the model.

Consider the GUI application for the shopping cart example of the previous sections that enables users to perform operations such as: adding items to the shopping cart, paying for all the items in the cart and starting a new session (emptying the shopping cart). 
If we monitor this application using \CBR with the \textit{Abstraction Functions} derived in the previous steps, we can for example collect the following bursts during an user execution (we show only methods related to the \texttt{Cart} class):

\JCODESTEP{code:log1}{Burst 1: clickOnAddItem}{log1.log}{1}

\JCODESTEP{code:log2}{Burst 2: clickOnAddItem}{log2.log}{1}

\JCODESTEP{code:log3}{Burst 3: clickOnPay}{log3.log}{1}

\JCODESTEP{code:log4}{Burst 4: clickOnStartNewSession}{log4.log}{1}

\JCODESTEP{code:log5}{Burst 5: clickOnStartNewSession}{log5.log}{1}

\begin{figure}[h]
\centering
\includegraphics[width=0.75\textwidth]{figures/fsa_example}
\caption{Example of resulting \FSA}
\label{fig:fsa_example}
\end{figure}

By following the procedure for joining the collected bursts in a \FSA, we could obtain the model shown in Figure \ref{fig:fsa_example}.

\JCODESTEP{code:trace1}{Trace 1}{trace1.log}{1}

\JCODESTEP{code:trace2}{Trace 2}{trace2.log}{1}

\JCODESTEP{code:trace3}{Trace 3}{trace3.log}{1}

We assess the validity of the model against traces 1, 2 and 3, represented respectively in Listings \ref{code:trace1}, \ref{code:trace2} and \ref{code:trace3}. These traces has been observed by a monitor that collects all the events in the field, so we highlight only the methods related to the \texttt{Cart} class. 

As described previously, to assess the validity of the model we first need to evaluate the precision of the \FSA. 
We use Equation \ref{eq:precision} to estimate the precision for nodes $PS\_0$, $PS\_1$ and $PS\_2$ in the \FSA. In particular, we check that all possible traces combination from nodes actually exist in traces 1, 2 or 3.

\begin{table}[h]
\centering
\caption{Precision for each node in the \FSA}
\label{table:fsa_precision_ex}
\begin{tabular}{ll}
\hline
\textbf{Node} & \textbf{Node precision} \\ \hline
$PS\_0$         &       100\%            \\ \hline
$PS\_1$         &       100\%            \\ \hline
$PS\_2$         &       100\%            \\ \hline
\end{tabular}
\end{table}

The reported precision for each node is shown in Table \ref{table:fsa_precision_ex}. The average precision of the \FSA is $100\%$.

We then use Equation \ref{eq:recall} to evaluate the recall of the traces produced through the \FSA. In other words, make sure that traces 1, 2 and 3 are a possible outcome of the model.

\begin{table}[h]
\centering
\caption{Recall of each trace generated by the \FSA}
\label{table:fsa_recall_ex}
\begin{tabular}{ll}
\hline
\textbf{Trace} & \textbf{Recall} \\ \hline
$Trace_1$         &       100\%            \\ \hline
$Trace_2$         &       100\%            \\ \hline
$Trace_3$         &       100\%            \\ \hline
\end{tabular}
\end{table}

The recall of each trace is reported in Table \ref{table:fsa_recall_ex}. The average recall of the traces produced from the \FSA is $100\%$.

Considering the values we achieved for \textit{precision} and \textit{recall}, we conclude that the \FSA presented in Figure \ref{fig:fsa_example} will produce trustful traces of high quality for the example.

However, if \CBR would identified a \textit{clickOnAddItem} action with a transition going from node $PS\_2$ to $PS\_0$, the node precision of node $PS\_2$ would be dropped to $50\%$, since the sequence of actions \textit{clickOnPay} followed by \textit{clickOnAddItem} was never observed in the field.

\section{Empirical Validation}\label{sec:empirical_cbr}

This Section presents the empirical validation we conducted for \Controlled, in order to assess the quality of the solution with respect to the performance, recall and precision in comparison to sampling techniques.
We provide information about the details of the experiments, the investigated aspects and the results we obtained for \CBR.

\subsection{Goal and Research Questions}

The goal of the experiment is to evaluate the performance, the precision and the recall of the traces produced by \Controlled, by comparing results with different approaches present in the literature.

With this experiment we aim to answer the following research questions:

\begin{itemize}
	\item \textbf{RQ1: What is the overhead introduced by \Controlled?} In this research question, we measure the performance of our technique with respect to other sampling techniques.

	\item \textbf{RQ2: What is the precision of the model generated by \Controlled?} In this research question, we measure the precision of the \FSA model with respect to the traces collected with monitoring.

	\item \textbf{RQ3: What is the recall of the traces produced by \Controlled?} In this research question, we measure the recall of the technique with respect to the monitored traces.
\end{itemize}

\subsection{Experiment Design}\label{sec:cbr_exp_design}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/experiment_design_4}
\caption{\Controlled Validation.}
\label{fig:experiment_design_4}
\end{figure}

Figure \ref{fig:experiment_design_4} shows the high-level work-flow of the experiment.
The main idea of the experiment is to compare \CBR to other sampling techniques, with respect to the performance, precision and recall of the technique itself. The monitoring objective is to collect the method calls related to a certain execution, including the runtime value of the parameters associated to each method call.

Sampling monitors have been used widely for monitoring applications in the field \cite{Jin:Sampling:SIGPLAN:2010,liblit2005scalable,joshi2017runtime,BabaeeGF18}: this type of monitors decrease the overall monitoring overhead by observing events only under a certain probability.
When analyzing interactive applications, each time the user interacts with the application the sampling monitor records with a certain probability. When the monitor is activated, it registers a defined amount of events.

For the experimentation, we implemented two sampling monitors, one with a sampling probability of $5\%$ and a second one with a $10\%$ of probability. Both sampling monitors trace a fixed number of events, in this case we fixed the amount to $30$ events per trace: a similar configuration setup has been used in \cite{Hirzel:BurstyTracing:FDDO:2001} for a sampling monitor.  

For assessing the \textit{performance} we measure execution times of a program being monitored with the three approaches compared to a program execution without any monitoring. 
The granularity of the monitoring is the single user action, that is to say measuring the execution time from the moment the user interacts with the application to the moment the program has finished processing the user request and gives a feedback to the user.
Since we care about how monitoring impacts on different functionalities, we analyze overhead with respect to the different categories of operations of the system response time categorization (see Chapter \ref{chapter:userstudy}).

To address the validity of the \CBR model we consider the procedure specified in Section \ref{sec:precision}: 
we assess \textit{precision} by applying Equation \ref{eq:precision} to every single node of the \FSA produced from the traces generated during the experimentation.   
Instead, we assess \textit{recall} by estimating how complete are the traces generated by each approach with respect to the original traces, in particular, we use Equation \ref{eq:recall} to calculate the Recall indicator of a certain trace.

\subsection{Experimental Subject}

To empirically answer the research questions, we use \Controlled to monitor ArgoUML \cite{ArgoUML:website:2018}.
ArgoUML is a UML diagramming application written in Java (389,952 lines of code): within the features of ArgoUML is possible to design Use Case, Class, Sequence, Collaboration, State-chart, Activity and Deployment diagrams. We selected ArgoUML because is a representative program of the target applications we are studying here: an user-interactive software application of medium-big size.

We considered the package \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small} as the target of monitoring, in particular, this package manages all the functionalities related to the design and management of activity diagrams in ArgoUML. We chose this package since activity diagrams are a very common way to represent behavioral information about software systems, so it is easy to make examples of this type of diagrams.

\subsubsection{Definition of the Abstract Program State}

% Since \CBR is a technique that consists in pre- and post-deployment operations, we first calibrate the tool to work with the program being analyzed. In particular, we define the corresponding representation of the Abstract Program State (see Section \ref{sec:SD}).

To define the Abstract Program State we start by doing static analysis of the component to be analyzed: Table \ref{table:target_jbse} offers some information about this process. 
To start, static analysis process discovered 16 classes and 199 methods inside component \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}, then the discovered methods are used as inputs to the symbolic executor, which processes each method and produce the corresponding abstraction functions. The symbolic executor produced 5,732 abstraction functions.

\begin{table}[h]
\caption{Monitoring Target and Symbolic Execution Outcome}
\label{table:target_jbse}
\begin{tabular}{|l|l|}
\hline
\textbf{Monitoring Target}                  & \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}        \\ \hline
\multirow{3}{*}{\textbf{Packages Analyzed}} & \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}        \\ \cline{2-2} 
                                            & \begin{small}\texttt{org.argouml.uml.diagram.activity.layout}\end{small} \\ \cline{2-2} 
                                            & \begin{small}\texttt{org.argouml.uml.diagram.activity.ui}\end{small}     \\ \hline
\textbf{Classes Analyzed}            & 16                   \\ \hline
\textbf{Methods Analyzed}            & 199 	              \\ \hline
\textbf{Abstraction Functions}          & 5,732                \\ \hline
\end{tabular}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.55\textwidth]{figures/argouml_example}
\caption{Activity Diagram example in ArgoUML}
\label{fig:argouml_example}
\end{figure}

In order to recreate proper executions of ArgoUML we have written 30 automatically executable test cases that encode typical usage scenarios for \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small} component: each test case consists in simulating the drawing of one activity diagram on the application (e.g. diagrams such as Figure \ref{fig:argouml_example}). These 30 test cases are used along the calibration and experimentation process.
To avoid non-determinism and for reproducibility of the test cases we implemented them with the Sikulix \cite{sikulix} capture and replay tool.

To train and produce the optimal representation of the program state, we run the application with the monitor using the original 5,732 abstraction functions. Once we execute the 30 test cases, we produce a single log file with all the possible program states detected across the simulations. As specified in Section \ref{sec:monitor}, our technique filters out all the \textit{Non-Discriminating}, \textit{Equivalent} and \textit{Redundant} Abstraction Functions. 

\begin{table}[h]
\caption{Details from the abstraction function filtering process.}
\label{table:filtered_set}
\centering
\scriptsize
\begin{tabular}{ll}
\hline
 & \textbf{Number of Abstraction Functions} \\ \hline
Original Set from JBSE & 5,732 \\ \hline
\textit{Non-Discriminating Abstraction Function} & 1,631 \\ \hline
\textit{Equivalent Abstraction Function} & 2,646 \\ \hline
\textit{Redundant Abstraction Function} & 1,298 \\ \hline
\textbf{Filtered Set} & \textbf{157} \\ \hline
\end{tabular}
\end{table}

The result of the filtering process is shown in Table \ref{table:filtered_set}: the procedure filtered out 5,575 functions, leaving 157 \AF as the optimal representation for \APS. In particular, 
the \textit{Non-Discriminating Abstraction Functions} were 1,631,
the \textit{Equivalent Abstraction Functions} were 2,646 
and the \textit{Redundant Abstraction Functions} were 1,298. 

\section{Results}\label{sec:cbr_results}

In this section we present the results of the experiment we conducted to validate \Controlled. All the experiments were executed on a computer running macOS version 10.13.6 with a 3.1 GHz Intel Core i7 processor and 16 GB of RAM.

The following sections describe the results obtained to answer to the different research questions.

\subsection{Performance Results}

To answer the research question \textbf{RQ1: What is the overhead introduced by \Controlled?} we assessed the impact of the monitors, specifically we measured the overhead by comparing the execution times of the monitored version with those without monitoring.
Then, we ran our set of 30 test cases, each test has been repeated 3 times and mean values have been used to mitigate any effect due to the non-determinism of the execution environment. 
Overall, we collected near 3,459 samples about the execution time of actions.

In addition to measuring execution times, we collect the execution traces that will be useful for answering the research questions \textbf{RQ2} and \textbf{RQ3}.

Since this work is focused on understanding the impact of the monitoring on the user experience, we classify user actions according to its system response time category, in particular we used the categorization presented in Chapter \ref{chapter:userstudy} (i.e., Instantaneous, Immediate, Continuous and Captive actions).
Along the 30 test cases, we identified 915 actions of the Instantaneous category, 25 actions from the Immediate category and 213 actions from the Continuous category. Given the nature of the functionalities we tested, we did not identify Captive actions.

\begin{table}[h]
\centering
\caption{Performance results with respect to system response time categories.}
\label{table:performance_results}
\scriptsize
\begin{tabular}{llll}
\hline
 & \multicolumn{3}{c}{\textbf{Monitoring Overhead {[}\%{]}}} \\ \hline
\textbf{Monitoring Technique} & \textbf{Instantaneous} & \textbf{Immediate} & \textbf{Continuous} \\ \hline
\CBR & 123.78 & 40.70 & 0.71 \\ \hline
Sampling 1 (P: 10\%) & 17.03 & 4.65 & 1.37 \\ \hline
Sampling 2 (P: 5\%) & 7.12 & 2.88 & 0.28 \\ \hline
\end{tabular}
\end{table}

The results for performance can be found in Table \ref{table:performance_results}: specifically, we present overhead data for the different monitors used in the experimentation with respect to the different system response time categories. 

In the table, \CBR represents \Controlled, \textit{Sampling 1} the monitor that traces in a sampling way with 10\% probability and \textit{Sampling 2} the monitor that samples with 5\% probability.

The first thing we can notice is that for the actions categories that employ less than one second, i.e., Instantaneous and Immediate actions, \CBR introduces considerable more overhead than the other techniques, 123.78\% of \CBR compared to 17.03\% of Sampling 1, 7.12\% of Sampling 2 for Instantaneous actions, or the 40.70\% of \CBR compared to the 4.65\% and 2.88\% of Sampling 1 and 2 respectively for Immediate actions. 

The increased overhead for actions $< 1$ second is explained by the fact that \CBR, besides tracing events, needs to evaluate 157 conditions at the beginning and at the end of each action, plus the fact that Instantaneous and Immediate actions are volatile and very sensitive to any additional time.

The second thing we notice is that contrary to Instantaneous and Immediate actions, \CBR performs equally for actions $> 1$ second (i.e., Continuous actions), in fact \CBR introduced 0.71\% of overhead, which is similar to the performance of Sampling 1 (1.37\%) and Sampling 2 (0.28\%). Since these actions are less volatile, the task of evaluating program state does not impact on the final overhead.

However, from our human-subject studies results (see Section \ref{sec:results}) we discovered that users do not perceive high monitoring overhead levels for Instantaneous actions, and that users perceive a degradation of the system response time only at 140\% for Immediate actions, meaning that in practice, users would not perceive monitoring overhead when \Controlled is activated.

Moreover, Sampling 1 and 2 techniques are not useful for simulating possible executions from the field, since they are observing only small percentages from the execution and do not provide contextual information, while \CBR is capable of representing comprehensive behaviors from the traces signed with program state information.

\subsection{Precision Results}\label{sec:acc_results}

For answering the research question \textbf{RQ2: What is the precision of the model generated by \Controlled?} we measured the precision of each node when simulating possible traces from the \FSA generated by \Controlled.

\input{tables/accuracy_results}
\input{tables/completeness_results}

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{figures/accuracy_results}
\caption{Precision results with respect to different runs of the application.}
\label{fig:precision_results}
\end{figure}

We show results only for \CBR, since it is the only technique in this work that simulates possible execution traces, meaning that the precision of the traces recorded by sampling monitors is 100\%.

Table \ref{table:accuracy_results} and Figure \ref{fig:precision_results} show information about precision of \CBR given the sampling probability and the amount of runs of the application. 

As explained in Section \ref{sec:collect_bursts}, \CBR works in a probabilistic way, meaning that the monitoring of each interaction between the user and the application occurs only under a certain probability. 
If \CBR is deployed to monitor data with a probability lower than 100\%, it is necessary to run several times the same functionality in order to observe the whole behavior in the field. 
Since in practice a program is executed several times in different instances, we would observe several repeated observations of the same functionality throughout the monitoring process, and by increasing the number of runs of the monitor fewer samples will be needed in order to derive accurate results.

In Table \ref{table:accuracy_results} we present how the overall precision changes according to the number of observed runs of the application, in this case, we experimented with 1, 5, 10, 15 and 20 runs.

First, we observe that the maximum precision of the technique is around 81\%, this means that for every node in the \FSA, 81\% of the possible combinations of bursts are a feasible behavior of the application, while the remaining 19\% are traces that we never observed in the traces recorded when activating \CBR all the times. 

However, not all the 19\% are unfeasible traces: a subset of the traces represented by the remaining 19\% could still be possible behaviors of the software (e.g., we do not developed all the necessary test cases to cover the remaining 19\%).

Second, we note that with 5 runs of the application we achieve the maximum of the precision for our technique with a sampling probability of 50\%. 
Instead, when considering 10, 15 or even 20 runs, the maximum precision can be achieved with a 25\% sampling probability, which seems to be the more balanced result for all measurements.

Nevertheless, considering 5, 10, 15 or 20 runs are a very small number of executions in comparison to running the application thousands of times across the several instances in the field. Hence, taking into account thousands of samples for a same user action would allow us to considerably reduce the \CBR sampling probability.

\subsection{Recall Results}

\begin{figure}[h]
\centering
\includegraphics[width=0.85\textwidth]{figures/completeness_results}
\caption{Recall results with respect to different runs of the application.}
\label{fig:recall_results}
\end{figure}

In this section, we present results for the research question \textbf{RQ3: What is the recall of the traces produced by \Controlled?}. 
As stated in Section \ref{sec:cbr_exp_design}, to estimate the recall we measure the percentage covered by traces obtained with each monitor in comparison to those obtained with \CBR monitor activated all the time.

For \Controlled we present both in Table \ref{table:recall_results} and Figure \ref{fig:recall_results} the recall of the technique according to the sampling probability and how it changes according to the number of runs of the application. The recall is presented in two measures, the \textbf{RB} and \textbf{RE} indicators: 
the \textbf{RB} indicator shows the recall percentage with respect to the number of bursts that can be identified within the original traces in comparison to the simulated trace.
Instead, the \textbf{RE} indicator shows the recall percentage with respect to the number of events that can be identified in the original traces in comparison to the trace simulated by the \FSA.

We notice that considering only one run of the application we only achieve 100\% recall with sampling strategy at 100\%, which means having the monitor always on. When we decrease the sampling probability to 90\%, the recall of the technique decreases rapidly to 36\%. 

Given that we are considering only one run, it is very likely that our \FSA is missing several transitions and thus producing very short and incomplete traces. In fact, when considering 5 runs of the application it is possible to achieve a good recall percentage with 65\% of sampling probability.

Now, if we consider 10 runs of the application we obtain approximately $90\%$ of recall at a 45\% of sampling probability. Going further, for 20 runs of the applications we already obtain a good recall level for 25\%. Which is also a similar result obtained for precision in Section \ref{sec:acc_results}.

On the other side, for sampling monitors we obtained a recall value of 4.15\%, with a maximum recall of 7.77\%, meaning that the traces collected by this approach contains on average 4.15\% events from the total events contained in the traces obtained when activating \CBR all the times. 

\section{Discussion}\label{sec:cbr_discussion}

We have carried out an experimental evaluation for assessing the quality of \CBR in terms of monitoring \textit{performance} with respect to other two sampling approaches. 

Since \CBR works in a probabilistic way and does not trace full executions, we also assessed the \textit{precision} and the \textit{recall} of the traces simulated by \CBR, to understand the usefulness of the sampling approach in an attempt to decrease monitoring overhead and to reduce the impact on the user environment.

When assessing performance, we discovered that the monitoring overhead introduced by \CBR with respect to other sampling approaches was higher for user actions employing less than one second, and similar for those user actions employing more than one second.

However, by considering our earlier results obtained in Chapter \ref{chapter:userstudy} about the impact of monitoring overhead on the user experience, we conclude that \CBR would not be perceived by users, since the overhead introduced by the technique is always lower than 140\%, which is the limit for tolerating monitoring overhead in the users' environment, while allowing the technique to obtain traces with enriched information for generating more comprehensive knowledge of the application usage.

About the quality of the traces produced by \CBR, we discovered that the precision of the simulations we produced were 81\% with respect to the original traces.
Unfortunately, our experimentation was not enough to prove if the remaining 19\% were actually infeasible behaviors or they were simply unobserved behaviors of the application.

On the other side, \CBR was able to simulate traces that were 100\% complete with respect to the original traces. A very different result compared to the 4\% recall obtained by the other sampling approaches.  

Nevertheless, we noticed that by using a sampling rate fixed to 25\% was possible for \CBR to reproduce safe traces that represent reliable behaviors of field executions.
We are also aware that by increasing the amount of users, that is, increasing the monitored executions, we might considerably decrease the sampling rate to make \CBR a less expensive solution.

We also discovered the importance of adding state information to traces: as a matter of fact by using the \CBR monitoring approach we were able to observe complete user executions, while other sampling approaches not employing state information only observed small percentages of the user execution.

In the overall, \CBR is a good monitoring approach that can be used for constructing and simulating knowledge from field executions without impacting on the user experience.



==> after rev/empirical.tex <==
% !TEX root =  main.tex

\section{Empirical Evaluation}\label{sec:empirical_cbr}

This section presents the empirical evaluation that we conducted for \Controlled, to assess the approach in comparison to  sampling techniques. Note that here, even if \CBR itself record bursts with a given probability, we use the term sampling techniques to refer to the techniques that collect bursts in an uncontrolled way (i.e., not synchronously with the processing of user \begin{mod}operations\end{mod}).
%We provide information about the details of the experiment, the investigated aspects and the results we obtained for \CBR.
In particular, we aim to answer the following research questions.

\begin{itemize}
	\item \textbf{RQ1: What is the overhead introduced by \Controlled?} This research question studies the overhead introduced by \CBR in comparison to other sampling techniques.

	\item \textbf{RQ2: What is the precision of the model generated by \Controlled?} This research question investigates the precision of the information captured in the model produced by \CBR with respect to the behaviors shown by the system. Since sampling techniques do not recombine the recorded traces, their precision is always 1 and do not need to be studied empirically.

	\item \textbf{RQ3: What is the completeness of the model generated by \Controlled?} This research question studies the capability of \CBR to capture the actual behaviors shown by the system, in comparison to sampling techniques.
\end{itemize}


\subsection{Prototype}
Our tool is implemented in Java and targets Java programs. It integrates third-party tools for static analysis, symbolic execution, and monitoring. In particular, \CBR uses WALA~\cite{WALA} to statically analyze the code of the monitored program and identify the relevant classes. In addition, it uses JBSE~\cite{Braione:Enhancing:FSE:2013} to symbolically analyze the relevant classes and produce the path conditions that are transformed into abstraction functions. %bounding the exploration of loops to ?????. in each selected class and use the path conditions resulting from the analysis of each method as functions for state abstraction. 
The generation of the conditions from each analyzed method is bounded by limiting the number of branches and the number of states that can be traversed sequentially to 10 and 1000, respectively. The analysis time of each method is also limited to 60 seconds.
Finally, \CBR uses AspectJ~\cite{AspectJ:website:2018} to collect data about the executed methods. %The tool is available in \url{https://github.com/cbr-paper/CBR_Experimental}.


\subsection{Experimental Subject}

To empirically answer the three research questions, we selected ArgoUML~\cite{ArgoUML:website:2018}, which is a non-trivial (389,952 locs) open source Java application for editing UML diagrams that can be used in a variety of ways (e.g., to produce largely different diagrams) and whose behavior can be studied in terms of the executions produced in the field.  

To consider the situation in which %a user is 
% in realta' l'utente qui è ambiguo, sarebbe il nostro utente, cioè il developer o il tester, ma qui con utente abbiamo sempre inteso l'utente finale dell'applicazione sotto monitoring
\begin{mod}we are\end{mod} interested in a specific part of the application, we selected the entire  \begin{small}\texttt{activity}\end{small} package as the target of the monitoring activity. This package manages all the functionalities related to the design and management of activity diagrams in ArgoUML. %We chose this package since activity diagrams are a very common way to represent behavioral information about software systems, so it is easy to make examples of this type of diagrams.
As monitoring objective, we consider collecting calls to methods implemented in the classes of the target package, including the values of the parameters. In order to recreate proper executions of ArgoUML, we have \begin{mod}implemented 25 test cases reproducing typical usage scenarios for the \begin{small}\texttt{activity}\end{small} package. Each test case consists of drawing a different activity diagram using different elements and features. \end{mod}%written 25 automatically executable test cases that encode typical usage scenarios for the \begin{small}\texttt{activity}\end{small} package. 
%Each test case consists of simulating the drawing of one activity diagram on the application, using different elements and features. 
To avoid non-determinism and for the reproducibility of the test cases, we %implemented 
\begin{mod}recorded and executed\end{mod} them with the Sikulix testing tool~\cite{sikulix}. All the measurements have been obtained by repeating the execution of the tests three times. 

The test cases, our tool, and the experimental material are available in the following repository \url{https://github.com/cbr-paper/CBR_Experimental}.

\subsection{Function Filtering}

%When defining the Abstract Program State, the static analysis process discovered 3 packages, 16 classes and 199 methods inside component \begin{small}\texttt{activity}\end{small}, then the discovered methods were used as inputs to the symbolic executor, which processes each method and produces the corresponding abstraction functions. 


% \begin{table}[h]
% \centering
% \scriptsize
% \caption{Monitoring Target and Symbolic Execution Outcome}
% \label{table:target_jbse}
% \begin{tabular}{|l|l|}
% \hline
% \textbf{Monitoring Target}                  & activity       \\ \hline
% \multirow{3}{*}{\textbf{Packages Analyzed}} & activity       \\ \cline{2-2} 
%                                             & activity.layout \\ \cline{2-2} 
%                                             & activity.ui     \\ \hline
% \textbf{Classes Analyzed}            & 16                   \\ \hline
% \textbf{Methods Analyzed}            & 199 	              \\ \hline
% \textbf{Abstraction Functions}          & 5,732                \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[h]
% \caption{Details from the abstraction function filtering process.}
% \label{table:filtered_set}
% \centering
% \scriptsize
% \begin{tabular}{ll}
% \hline
%  & \textbf{No of Abstraction Functions} \\ \hline
% Original Set from SE & 5,732 \\ \hline
% \textit{Non-Discriminating Abstraction Function} & 1,631 \\ \hline
% \textit{Equivalent Abstraction Function} & 2,646 \\ \hline
% \textit{Redundant Abstraction Function} & 1,298 \\ \hline
% \textbf{Filtered Set} & \textbf{157} \\ \hline
% \end{tabular}
% \end{table}

%The result of the filtering process is shown in Table~\ref{table:filtered_set}: 

In this section, we discuss the result of the filtering process applied to our experimental subject (step 3). When running \CBR in the considered setting, the symbolic executor produced 5,732 abstraction functions. \CBR then identified and filtered out all the \textit{Non-Discriminating}, \textit{Equivalent}, and \textit{Redundant} Abstraction Functions. Overall, \CBR reduced the number of abstraction functions to be used to generate the abstract program states from 5,575 to 157 abstraction functions, filtering out 97.2\% of the functions. %In particular, \CBR found 1,631 \textit{Non-Discriminating Abstraction Functions}, 2,646 \textit{Equivalent Abstraction Functions}, and 1,298 \textit{Redundant Abstraction Functions}, as summarized in 
Table~\ref{table:filtering} shows the number of functions that have been filtered out in each step by \CBR, confirming the usefulness of all the steps.

\begin{table}[h]
\centering
\caption{Function Filtering}
\label{table:filtering}
\scriptsize
\begin{tabular}{lc}
%\toprule
 & \# Abstraction Functions \\ 
%\midrule
\toprule
Initial number of abstraction functions & 5,732 \\ 
\midrule
Non-Discriminating Abstraction Functions & 1,631\\
Equivalent Abstraction Functions & 2,646\\
Redundant Abstraction Functions & 1,298\\
\midrule
Final set of Abstraction Functions & 157\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Experiment Design}\label{sec:cbr_exp_design}
%The CBR sampling monitor records a number of method calls (a burst) with a certain probability every time the user interacts with the monitored application. 

In our assessment, we compare \CBR to sampling techniques, which have been used widely for monitoring applications in the field~\cite{Jin:Sampling:SIGPLAN:2010,liblit2005scalable,joshi2017runtime,BabaeeGF18}. These solutions limit the overhead by collecting data  with a given probability. %\begin{TBF}Please consider that in our framework an event is a user interaction with the application, while in these other solutions an event is directly a function call.\end{TBF}
%In our setting, every time the user interacts with the monitored application, the sampling monitor records a number of method calls (a burst) with a certain probability. 
Note that differently from \CBR, these bursts have neither a semantics associated with the processing of the user requests nor the state annotations, but consist of traces containing a fixed number of method calls. 
We considered sequences of length $30$, similarly to the configuration setup \begin{mod}used for \textit{Bursty Tracing}~\cite{Hirzel:BurstyTracing:FDDO:2001}, which is the closest technique to \CBR.\end{mod}

In our evaluation, we compare \CBR to Sampling monitoring configured with two sampling probabilities: $5\%$ and $10\%$ (higher sampling frequencies might be hardly considered since they may interfere with the user activity). %Both sampling monitors trace a fixed number of \begin{TBF}function calls\end{TBF}: in this case we fixed the amount to $30$ events per trace (a similar configuration setup has been used in~\cite{Hirzel:BurstyTracing:FDDO:2001} for a sampling monitor.)  
We thus compared three solutions: \CBR, Sampling monitoring with 5\% sampling probability, and Sampling monitoring with 10\% sampling probability.

\smallskip

To answer \emph{RQ1}, we measure the overhead introduced in the subject program by the three monitoring techniques when running the available test cases. To measure overhead, we collect the system response time of each user operation that is executed. 

%The granularity of the monitoring is the single user interaction, that is to say measuring the execution time from the moment the user interacts with the application to the moment the program has finished processing the user request and gives a feedback to the user.
%\begin{TBF}For both the \CBR traces and those of the two sampling monitors, we save on other files the starting and ending time of each user action so that we are able to calculate their system response time.\end{TBF}

To capture how monitoring may impact the execution of operations of different nature, we organize the data based on the well-known and widely accepted classification from the human computer interaction area proposed by Seow~\cite{seow}. In this classification, operations are organized according to four categories, which have been derived from direct user engagement. Each category represents a different type of operation and has a foreseen maximum system response time. The four categories are: 

\begin{itemize}
\item \emph{Instantaneous}: these are the simplest operations that can be performed on an application, such as entering inputs
or navigating throughout menus. Their system response time is expected to be 200ms at most.
\item \emph{Immediate}: these are the operations that generate acknowledgments or very simple outputs. Their system response time is expected to be 1s at most.
\item \emph{Continuous}: these are operations that produce a result within a short period of time to not interrupt the
dialog with the user. Their system response time is expected to be 5s at most.
\item \emph{Captive}: these are operations requiring some relevant processing for which users will wait for results. Their system response time is expected to be 10s at most. These operations are not present in ArgoUML.
\end{itemize}

We study the impact of the monitoring activity per category because the relative overhead can be quite different for each type of operation.

\smallskip


%For evaluating the validity of the \CBR model, we consider two aspects: \textit{precision} and \textit{trace-level recall} of the traces generated by \CBR.
%
%The building process and the semantics of the \FSA has a direct relationship with the precision of the technique. In some cases, it is possible that the generated traces are behaviors that do not occur in the field, which is the reason why we assess the precision of the generated \FSA.

To answer \emph{RQ2}, we measure to what extent the behaviors represented in the model generated by \CBR correspond to actual (original) traces of the monitored program (we collected the complete traces of execution, with all the generated function calls, once at the beginning of the experiment). We study this aspect locally to each node in comparison to the actual set of observed behaviors because nodes are the joint points between bursts, which may introduce imprecision. 
%Since verifying if a full trace accepted by the model can be produced by the program is almost infeasible for applications with the complexity of ArgoUML, we measure the precision of the model at two levels.
That is, we evaluate precision locally (i.e., \textit{node precision}) and then globally (i.e., \textit{overall nodes precision}). In particular, we first assess if the local decisions taken in each node have a corresponding evidence in the original traces, and then we compute a global metric as mean of the local precision of each node.  
%The assumption is that if on average the local decisions taken for each node are right, so decisions taken globally by an execution derived from the model is also probably right.


%represented in the model produced by \CBR exists in the original traces: the ground truth we compare to (that is, the set of compete traces including all the function calls with values of the parameters), has been created once using a simple monitor always recording function calls and parameters.
%The precision is evaluated first locally (i.e., \textit{node precision}) and then globally (i.e., \textit{overall nodes precision}): in other words, we first assess if the local decisions taken in each node of the \FSA are right, and then we deduce the global correctness. 
%The assumption is that if on average the local decisions taken for each node are right, so the decisions taken globally by an execution derived from the model is also probably right.

\begin{figure}[h]
\centering
\includegraphics[width=0.35\columnwidth]{figures/node.png}
\caption{\FSA node with state information and incoming and outgoing transitions.}
\label{fig:node}
\end{figure}

To assess \textit{node precision}, for each node in the model we check if every possible sequence of events of length 2 which involves that node is an actual program behavior. 
For example, for the node in Figure~\ref{fig:node} we first generate all the possible combinations of sequence of actions, that is, $A_1 \rightarrow B_1$, $A_1 \rightarrow B_2$, \ldots, $A_3 \rightarrow B_3$, then we verify if the traces produced by these sequences are present in the set of original recorded traces. % used to produce the model.

In particular, the node precision for a particular node $node_i$ is computed with the formula $precision(node_i) = CS_i\mathbin{/}TS_i$ where $CS_i$ is the number of sequences of length 2 that traverse $node_i$ and that have a  counterpart in the original traces, and $TS_i$ is the total number of sequences of length 2 that traverse node $i$.
The \textit{overall nodes precision} is obtained by computing the mean \textit{node precision} of all the nodes in the model. For simplicity in the rest of the document we refer to \textit{overall nodes precision} simply as \textit{precision}.

Note that we do not compute precision for sampling techniques because they do not provide any form of generalization of the collected traces, and thus the precision of the extracted information is always 1.

\smallskip

To answer \emph{RQ3}, we measure \textit{trace-level recall} that is, we measure how complete the extracted information is with respect to the complete traces of executions produced by the monitored application. Note that all the monitoring techniques collect only a subset of these traces when the sampling is activated: both \CBR and sampling techniques collect bursts while missing the rest of the computation.  %However, across multiple executions, the full traces might still be reconstructed.
However, the information that is not recorded from an execution can still be recorded in future executions, thus finally obtaining a more complete picture of the behavior observed in the field.

To measure the ability of the monitoring technique to extract complete traces from the bursts collected from the field, we measure the trace recall for a given trace as  $recall(trace_j) = E_j\mathbin{/}EO_j$ where $E_j$ is the number of calls captured by the monitoring technique, and $EO_j$ is the overall number of method calls in the original trace. We use the available test cases to obtain the program traces. Note that while sampling techniques extract sequences of fixed length, \CBR can reconstruct longer executions combining multiple samples thanks to the state information attached to bursts. In the rest of the document we refer to \textit{trace-level recall} simply as \textit{recall}.

\smallskip

Let us remark that both \CBR and sampling techniques are used to reconstruct information about behaviors observed in the field, and not the general behavior of an application. For this reason, both the precision and the recall metrics are defined with respect to the full traces produced by running the test cases of the monitored application, and not about all the feasible behaviors of the monitored program.


==> after rev/esempio.tex <==

% \oscar{I would not include the following section...}
% \begin{TBR}
% \subsubsection{Finite State Automaton Example}

% Since the final step of the technique consists in generating a \FSA and then producing simulations of possible field executions, we show an example of a possible \FSA and how we assess the validity of the model.

% Consider the GUI application for the shopping cart example of the previous sections that enables users to perform operations such as: adding items to the shopping cart, paying for all the items in the cart and starting a new session (emptying the shopping cart). 
% If we monitor this application using \CBR with the \textit{Abstraction Functions} derived in the previous steps, we can for example collect the following bursts during an user execution (we show only methods related to the \texttt{Cart} class):

% \JCODESTEP{code:log1}{Burst 1: clickOnAddItem}{log1.log}{1}

% \JCODESTEP{code:log2}{Burst 2: clickOnAddItem}{log2.log}{1}

% \JCODESTEP{code:log3}{Burst 3: clickOnPay}{log3.log}{1}

% \JCODESTEP{code:log4}{Burst 4: clickOnStartNewSession}{log4.log}{1}

% \JCODESTEP{code:log5}{Burst 5: clickOnStartNewSession}{log5.log}{1}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.75\columnwidth]{figures/fsa_example}
% \caption{Example of resulting \FSA}
% \label{fig:fsa_example}
% \end{figure}

% By following the procedure for joining the collected bursts in a \FSA, we could obtain the model shown in Figure~\ref{fig:fsa_example}.

% \JCODESTEP{code:trace1}{Trace 1}{trace1.log}{1}

% \JCODESTEP{code:trace2}{Trace 2}{trace2.log}{1}

% \JCODESTEP{code:trace3}{Trace 3}{trace3.log}{1}

% We assess the validity of the model against traces 1, 2 and 3, represented respectively in Listings~\ref{code:trace1},~\ref{code:trace2} and~\ref{code:trace3}. These traces has been observed by a monitor that collects all the events in the field, so we highlight only the methods related to the \texttt{Cart} class. 

% As described previously, to assess the validity of the model we first need to evaluate the precision of the \FSA. 
% We use the $Precision$ equation to estimate the precision for nodes $PS\_0$, $PS\_1$ and $PS\_2$ in the \FSA. In particular, we check that all possible traces combination from nodes actually exist in traces 1, 2 or 3.

% \begin{table}[h]
% \centering
% \caption{Precision for each node in the \FSA}
% \label{table:fsa_precision_ex}
% \begin{tabular}{ll}
% \hline
% \textbf{Node} & \textbf{Node precision} \\ \hline
% $PS\_0$         &       100\%            \\ \hline
% $PS\_1$         &       100\%            \\ \hline
% $PS\_2$         &       100\%            \\ \hline
% \end{tabular}
% \end{table}

% The reported precision for each node is shown in Table~\ref{table:fsa_precision_ex}. The average precision of the \FSA is $100\%$.

% We then use the $Recall$ equation to evaluate the recall of the traces produced through the \FSA. In other words, make sure that traces 1, 2 and 3 are a possible outcome of the model.

% \begin{table}[h]
% \centering
% \caption{Recall of each trace generated by the \FSA}
% \label{table:fsa_recall_ex}
% \begin{tabular}{ll}
% \hline
% \textbf{Trace} & \textbf{Recall} \\ \hline
% $Trace_1$         &       100\%            \\ \hline
% $Trace_2$         &       100\%            \\ \hline
% $Trace_3$         &       100\%            \\ \hline
% \end{tabular}
% \end{table}

% The recall of each trace is reported in Table~\ref{table:fsa_recall_ex}. The average recall of the traces produced from the \FSA is $100\%$.

% Considering the values we achieved for \textit{precision} and \textit{recall}, we conclude that the \FSA presented in Figure~\ref{fig:fsa_example} will produce trustful traces of high quality for the example.

% However, if \CBR would identified a \textit{clickOnAddItem} action with a transition going from node $PS\_2$ to $PS\_0$, the node precision of node $PS\_2$ would be dropped to $50\%$, since the sequence of actions \textit{clickOnPay} followed by \textit{clickOnAddItem} was never observed in the field.
% \end{TBR}

==> after rev/framework.tex <==
% !TEX root =  main.tex

\section{CBR Framework}\label{sec:CBRFramework}

%In particular, a burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two concrete states of the application, initial and final respectively, and the trace $T$ is the sequence of events collected in the field.

\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{figures/CBR}
    \caption{Overview of \Controlled approach.}
    \label{fig:CBR}
\end{figure}


\Controlled (\CBR) is a technique that can reconstruct an approximate representation of the behavior shown in the field by a program and represents it as a hierarchical finite state model. The resulting model is approximated because its states and transitions are obtained by heuristically combining the information in the recorded bursts, especially exploiting the state information that appears at the beginning and end of each burst. 
%recording strategy produces partial information in the form of bursts, rather than full traces, to avoid annoying the users. The information available in the bursts is heuristically recombined. 
Figure~\ref{fig:CBR} shows the steps that compose \CBR. 


%represents the possible executions of an application in a Finite State Automaton structure; since this approach does not record full executions we might loss the full ordering of field events, but still a good representation of the behavior of the application can be given. From the generated model it is possible to extract accurate and comprehensive traces that could be useful for post-deployment analysis such as debugging, field failures reproduction and protocol verification, among others.
%
%Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques~\cite{walkinshaw2008inferring}: detection of anomalous behaviors, protocol verification and testing are only some examples of operations that could exploit these abstractions.

%Usually, the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon}~\cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 


The first step of the technique requires that 
%In the first step, 
the developer specifies the components that must be monitored in the field. Although the full application can be monitored, the developers might be interested in the behavior of some components only. Based on this input, \CBR analyzes the code of the application and identifies the scope of the instrumentation that must be added to the program, which includes all the classes that may directly or indirectly affect the behavior of the monitored components (step 1). We refer to the identified classes as the \emph{relevant classes}.  

% To extract data from the chosen components, \CBR identifies all the classes that may influence the usage of the components (step 1): this analysis is done by first selecting a subset of the system (e.g., components) that has been defined as the monitoring target and then by retrieving all the \textit{relevant classes} and their respective methods that exist inside the selected components. This set of \textit{relevant classes} is the result of step 1.

To associate contextual information useful to generate the final finite state model with the recorded data, \CBR records bursts that both start and end with state information. The state information should be accurate enough to distinguish the different logical states of the components, and inexpensive enough to be obtained at runtime without introducing a significant overhead. 
%
To identify a small but relevant amount of state information to be recorded with bursts, \CBR \emph{automatically} derives the \textit{Abstraction Functions} %, or \AF for short, 
that can be used at runtime to produce abstract representations of the concrete program states (step 2). The intuition is that the values of the state variables are relevant only to the extent they can affect the actual execution of the program, and this largely depends on the conditions that are computed on the state variables. For this reason, \CBR analyzes the set of relevant classes looking for Boolean functions that can capture the behavior of the program. For example, if a relevant class implements an operation \texttt{op} whose code checks if the state variable \texttt{x} is positive, \CBR will output the \texttt{x>0} abstraction function, which is assumed to capture a relevant state property. This is intuitively true by construction since it is a condition that is known to influence a computation in one of the relevant classes, that is, the execution takes different paths in \texttt{op} depending on the value of \texttt{x}. Note that only the satisfaction of the condition is relevant, while the specific value of \texttt{x} is not relevant for the computation. This is why \CBR embeds the evaluation of the conditions and not the values of the program variables in the abstract program states.
\CBR obtains the abstract representation (i.e., an abstract state) of a concrete state by applying all the available abstraction functions (i.e., conditions), thus producing a set of function evaluations. 


%abstract the state of the target components mimicking the way the program itself analyzes its state variables.

%The abstraction functions are derived by analyzing the set of relevant classes looking for functions that can abstract the state of the target components mimicking the way the program itself analyzes its state variables.

%For instance, let us assume that a monitored component controls the interaction with the file system and that a method \texttt{write} may actually write to a variable \texttt{file} only if its boolean variable \texttt{open}, which represents if the file has been already open or not, is true, 
%The Function Extraction step will output the abstraction function \texttt{file.open == true} to indicate that the evaluation of this Boolean function may influence the behavior of the monitored components. 

Once \CBR has derived the abstraction functions from all the relevant classes, it analyzes and compares the resulting functions to eliminate the ones that are redundant (e.g., an abstraction function defined as the negation of another abstraction function adds no information about a concrete state of the program). Reducing the set of abstraction functions is useful to improve the performance of the approach, which has to compute fewer functions at runtime and to save smaller abstract states. The set of the remaining functions are embedded into the software monitor that is used at runtime to collect bursts decorated with state information (step 3). 

%After having defined the \AF through an automatic extraction process, the monitor is then assembled:  the monitoring component consists of the State Monitor and the Event Monitor. The State Monitor produces concrete values of the \AF at the beginning and at the end of each stream of events, and the Event Monitor collects the events associated with the component under monitoring.

In the field, \CBR collects bursts coherently with computations (step 4), that is, every time the application starts \begin{mod}a new user operation, a burst is collected with a given probability. A user operation starts with a user input (e.g., a click or a keyboard input) and ends with a feedback to the user (e.g., a result shown on the GUI)\end{mod}. When the burst is recorded, the resulting trace includes a representation of the abstract program state, the sequence of the executed methods, and again a representation of the abstract program state reached at the end of the computation caused by the user \begin{mod}operation\end{mod}. %More formally, a burst $B$ is a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action performed on the program, $S_1$ and $S_2$ are two \APS produced by the \AF and the trace $T$ is the sequence of methods executed in the field.


%\CBR has been designed to \textit{sample} executions from the field in order to decrease monitoring overhead: we can use program state information to give a temporal context to the different traces by calculating the state of the program before and after the set of events are observed in the field.


%One way to represent the state of an application is to consider the set of values of all the variables at a certain moment \textit{t} during the execution. Certainly, acquiring this information is too expensive to be done at runtime.  
%An efficient way to perform this operation is to subset the number of variables and the amount of information \CBR should save for each variable while monitoring.

%In the Function Extraction step (step 2), \CBR analyzes the relevant classes to distill the knowledge about the functions that may influence their execution, and thus influence the interaction with the monitored components. In particular, \CBR identifies a set of functions to be used to derive an abstract representation of the current state: we call the set of functions the \textit{Abstraction Functions}, or \AF for short.

%The most intuitive way to derive the \AF, is to extract from the application's code the functions that the application uses to define its execution path according to the runtime value of the variables. \CBR will only consider those functions that help to differentiate efficiently between different states at runtime. 



%The \AF are systematically applied to concrete states of the application to produce an abstract representation of the program state to which they were applied: these representations are called \textit{Abstract Program States}, or \textit{APS} for short.

%The \AF should have a proper balance in the abstraction level: too concrete functions can have bad implications, for instance checking all the field values of the program variables would be too expensive to be assessed at runtime (\textit{performance}). 
%On the other side, too abstract functions could generate poor program states that are not useful to distinguish different states of the application while running in the field (\textit{precision}).

%Since a program state directly depends on the conditions actually computed by the program while interacting with the monitored components, the \APS is representative of how the execution may proceed, specifically in terms of the interaction with the monitored components. 

% In principle, a set of bursts might be used to form a Finite State Automaton, to show real uses of the application (step 5), where the edges of the \FSA represent the different user actions and the nodes represent the possible program states. Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques~\cite{walkinshaw2008inferring}, such as detection of anomalous behaviors, protocol verification, testing, among others.

% Usually the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon}~\cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 

The collected bursts are finally analyzed offline. The abstract program states at the beginning and at the end of each burst %($S_1$ and $S_2$) 
abstractly represent the state of the system at the time the trace %$T$ 
was recorded. To summarize the observed executions, \CBR creates a Finite State Model (step 5), where each abstract state that occurs in the bursts is a different state of the model and each user \begin{mod}operation\end{mod} that causes a transitions between two abstract states is represented with a transition of the model. The sequences of method calls that can be executed as a consequence of a user \begin{mod}operation\end{mod} are represented as annotations of the transitions. 

The resulting model thus captures the activity observed in the field at multiple abstraction levels \begin{mod}(for this reason it is a hierarchical model)\end{mod}: the states and transitions show how the operations performed by users affect the status of the system, while the annotations show the actual methods involved in the computations.


% The main reason for generating these \FSA is representing the possible executions of an application, which may be useful to analyze the scenarios that may occur in the field.

In the next section, we introduce a running example that we use in the paper to present the steps of the approach.

\subsection{Running example}

Let us consider a Java program that includes the \texttt{Cart} class (see Listing~\ref{code:cart_class}), which represents a simplified shopping cart of an online store. The \texttt{Cart} class implements four different methods and includes the \texttt{Product} class: 
the \texttt{addItem} method adds a \texttt{Product} object to the shopping cart, %which is represented by an array of \texttt{Product} type,
the \texttt{emptyCart} method empties the shopping cart,
the \texttt{calculateTotal} method estimates the total price of all the products in the cart, and
the \texttt{applyDiscount} method applies a discount to the total price.

\JCODESTEP{code:cart_class}{Shopping Cart Class}{Cart.java}{1}


Let us assume that the developer wants to collect data about how a certain program uses the \texttt{Cart} class. %, focusing on the sequences of method calls produced by the program. %Capturing every call to every method of the \texttt{Cart} class might be expensive for operations that extensively use the methods implemented by the \texttt{Cart} class. 
In the following sections, we discuss how \CBR can address this scenario. Of course, here we consider the monitoring of a single class in a small program for simplicity. In reality,  multiple classes and packages can be selected as targets.

\input{step1.tex}
\input{step2.tex}
\input{step3.tex}
\input{step4.tex}
\input{step5.tex}

==> after rev/introduction.tex <==
% !TEX root =  main.tex

\section{Introduction}

%nell’introduzione farei riferimento al paper su burst recording per descrivere la strategia di registrazione come qualcosa di già sperimentato. Quanto proposto ha però il difetto di produrre bust isolati. Il contributo del paper è quello di definire una strategia per comporli

Field data is an essential source of information for a number of tasks, such as discovering emerging usage scenarios~\cite{Srivastava:WebUsage:SIGKDD:2000}, profiling users~\cite{Elbaum:Profiling:TSE:2005}, obtaining data about the reliability of the software~\cite{Gazzola:FieldFailures:ISSRE:2017}, mining models~\cite{ohmann2017lightweight,Mariani:Revolution:ISSRE:2012}, and validating software~\cite{Ohmann:OptimizedCoverage:ASE:2016,Pavlopoulou:ResidualCoverage:ICSE:1999}. The importance of observing the software while running in the field has been also well-recognized by industry: for instance, the video streaming company Netflix has started testing and collecting data directly from the field, using fault-injection and monitoring techniques~\cite{Basiri:Netflix:ISSRE:2016}. 


%understand if a software application is reliable or not, unfortunately assessing the robustness of software applications with only in-house data could lead to serious faults since we would be ignoring precious information about stimuli, environment and configurations that applications handle in the field.

%In the same way, field monitoring techniques are useful because they can capture precise data about the behavior of software systems. 
%They can reveal how applications are actually used by their users, capturing scenarios and configurations relevant to practitioners, and how failures manifest and impact user activity~\cite{Gazzola:2017:FTS:3098344.3098487}.

Collecting data from the field can be \emph{challenging}. In particular, monitoring and data collection can easily interfere with the user activity~\cite{Orso:DeployedSoftware:FoSER:2010}. %, that is, applications whose execution is driven by frequent interactions with users.  
While some solutions, such as simple crash reporting features, require collecting relatively few data for a short amount of time (e.g., a snapshot of the system at the time of the crash~\cite{Eclipse:website:2018,Windows:website:2019,Delgado:TaxonomyFaultMonitoring:TSE:2004}), many interesting and sophisticated approaches require monitoring applications more extensively. 
For example, many approaches collect \emph{sequences of method calls} to reproduce failures~\cite{Jin:BugRedux:ICSE:2012}, detect malicious behaviors~\cite{Gorji:MalwareDetection:ACMSE:2014}, debug applications~\cite{Murtaza:FaultLocalizationTheory:GTSE:2015}, profile software~\cite{Elbaum:Profiling:TSE:2005}, optimize applications~\cite{Zhao:Optimization:OOPSLA:2014}, and mine models~\cite{Mariani:Revolution:ISSRE:2012,Mariani:DynamicAnalysis:TSE:2011,7927993}. 
Unfortunately, extensively recording sequences of function calls might introduce an annoying overhead and cause unacceptable slowdowns, as for example experienced by Jin et al.~\cite{Jin:BugRedux:ICSE:2012}. Slow software is a major threat to the success of a project, indeed it is reported as one of the main reasons why users stop using applications~\cite{Ceaparu2004,Miller1968,Hoxmeier00systemresponse}.

Since preventing any interference with the user activity is a mandatory requirement, in many cases monitoring techniques have to limit the amount of collected data. This can be achieved in several ways: by limiting the portion of the system that is monitored~\cite{Pavlopoulou:ResidualCoverage:ICSE:1999,apiwattanapong2002selective,orso2005selective}; by distributing the monitoring activity among multiple instances of a same application running on different machines~\cite{Bowring:MonitoringDeployedSoftware:PASTE:2002,Orso:GammaSystem:ISSTA:2002}; by collecting events probabilistically~\cite{Bartocci:Adaptive:ICRV:2012,Jin:Sampling:SIGPLAN:2010,chilimbi2009holmes,Liblit:BugIsolation:SIGPLAN:2003}; and by collecting bursts of events rather than full executions~\cite{Hirzel:BurstyTracing:FDDO:2001,prepost}. Limiting the amount of collected data %is not always an option, and when applicable it anyway 
reduces the effectiveness of the approaches that must work with a limited number of samples. 

Since non-negligible overhead levels can be hardly recognized by users as long as the overhead lasts for few interactions~\cite{NIER17,Cornejo:FunctionCallMonitoring:JSS:2020,killeen_optimal_1987}, monitors could be feasibly used to collect fairly complete traces for a limited amount of time. In particular, a monitor might be turned on and off several times during a program execution in order to collect \textit{bursts}, that is, chunks of executions with no internal gaps~\cite{Hirzel:BurstyTracing:FDDO:2001}. Since the monitor is used intermittently, its impact on the user experience is limited. %, while multiple bursts can be combined together to obtain a better picture of the behavior of the monitored application.


%Although bursts include only partial information about a monitored execution, they are complete when restricted to their time interval (i.e., every monitored event produced by the application after the first event of the trace fragment and before the last event of the trace fragment also occurs in the burst).



%descrivere la strategia di registrazione come qualcosa di già sperimentato. Quanto proposto ha però il difetto di produrre bust isolati

%Although this monitoring strategy has been already studied and experimented, known as Bursty Tracing~\cite{Hirzel:BurstyTracing:FDDO:2001}, it has a very important flaw, which is the impossibility to correlate bursts of execution between each other, and so the full picture of the running execution.
%Since techniques such as software testing, debugging and profiling needs to process traces that show the complete behavior of the application we introduce a strategy to compose isolated bursts into a more comprehensive structure. 


Unfortunately, individual bursts capture only part of the history of an execution, providing scattered evidence of the behavior of the monitored software. To \begin{mod}obtain additional information while controlling the overhead, \end{mod}this paper \begin{mod}proposes \Controlled (CBR), a novel monitoring technique for recording bursts whose activation and deactivation is controlled by the operations performed by the users on the target application.\end{mod}
%controlled way introducing \Controlled, or \CBR for short, a monitoring technique that collects bursts by synchronizing the activation and deactivation of the monitor with the computations performed by the monitored application in reaction to user inputs. 
In particular, when a new user \begin{mod}operation is started,\end{mod}
%input is received, 
the monitor that records the burst is activated, and once the user request has been fully processed, the burst is finalized and the monitor is turned off. 

Since the recording of the burst is controlled, \CBR can also recombine the recorded bursts a-posteriori to obtain a comprehensive picture of the behavior of the monitored software. In particular, \CBR annotates bursts with state information that captures the state of the monitored application at the beginning and at the end of each burst (i.e., before and after a user %request 
\begin{mod}operation\end{mod}
 is performed). This information allows \CBR to generate a hierarchical finite state model that represents the behavior of the monitored application when used in the field. In this work we refer to bursts composed of sequences of method calls due to their wide applicability, but the same concepts can be applied to bursts that include other information. 



% We assess our approach in a restricted, although common, scenario, that is, \textit{recording the sequence of function calls produced by an application, annotated with parameters and state information}. 

% Many techniques exploit this type of field data, such as techniques for reproducing failures \cite{Jin:BugRedux:ICSE:2012}, profiling users \cite{Elbaum:Profiling:TSE:2005}, Finite State Automaton synthesis from traces \cite{lorenzoli2008automatic}, and controlling software evolution \cite{Orso:GammaSystem:ISSTA:2002}). 

We evaluated \CBR on ArgoUML and found that \CBR provides a valuable tradeoff between overhead and data accuracy compared to regular sampling techniques that probabilistically record bursts without controlling when the execution of the burst begins and ends. %Moreover, we discover that from the generated model it is possible to extract accurate and comprehensive traces that could be useful for post-deployment analysis such as debugging, field failures reproduction, protocol verification, among others.

This paper is organized as follows. %Section~\ref{sec:bursts} defines bursts. Section~\ref{sec:cbr} presents the benefits of using \CBR to extract field information. 
Section~\ref{sec:CBRFramework} describes \CBR. Section~\ref{sec:empirical_cbr} presents the empirical validation we conducted to assess our technique. Sections~\ref{sec:cbr_results} reports the empirical results. Finally, sections~\ref{sec:related} and~\ref{sec:cbr_discussion} discuss related work and provide concluding remarks, respectively.





==> after rev/related.tex <==
% !TEX root =  main.tex

\section{Related Work}\label{sec:related}

Our work focuses on the cost-effectiveness of monitoring, aimed at collecting field data in a non-intrusive way, possibly missing a limited amount of information. To this end, we relate \CBR to probabilistic and state-based monitoring approaches.


\textit{Probabilistic monitoring} accounts for lowering the impact of monitoring by collecting runtime information within a certain probability.
Liblit et al.~\cite{Liblit:BugIsolation:SIGPLAN:2003} exploited this strategy to isolate bugs by profiling a large, distributed user community and using logistic regression to find the program predicates that could be faulty. 
Similarly, Jin et al.~\cite{Jin:Sampling:SIGPLAN:2010} presented a monitoring framework called Cooperative Crug (Concurrency Bug) Isolation to diagnose production run failures caused by concurrency bugs. This technique uses sampling to monitor different types of predicates while keeping the monitoring overhead low.
In the same way, Hirzel et al.~\cite{Hirzel:BurstyTracing:FDDO:2001} developed Bursty Monitors, which collect subsequences of events with ad-hoc strategies to construct a temporal program profile.

In general, Probabilistic Monitoring is designed to collect partial information about executions with little ambition to reconstruct a wider picture of the behavior that can be observed in the field, while \CBR focuses on the construction of extended evidence by combining multiple bursts.

% The program state $PS$ of a certain application on a instant $t$ can be defined as $PS(t) = \{pv_{1}, pv_{2}, \ldots, pv_{r}\}$, where $pv_r$ represents the runtime value of a program variable on a moment $t$.

\emph{State-based} monitoring approaches focus on using a small subset of variables to represent a significant program state. These techniques are often used either for replaying field executions or for trace analysis (e.g., debugging).

For instance, Orso et al. \cite{orso2005selective} proposed a technique for selectively capturing and replaying program executions. This technique allows to select a subsystem of interest, capture at runtime all the interactions of the applications with its subsystem and then replay the recorded interactions in a controlled environment. For each interaction of the application, the technique captures a minimal subset of the application's state and environment required to replay the execution.
Similar to \CBR, this framework exploits the idea of tracing just the entities defined inside the subsystem of interest. However, this framework is not designed to derive extensive knowledge about the behavior of the system, but focuses on reproduction. 

Diep et al. \cite{Diep:Trace:ISSRE:2008} presented a technique for analyzing traces produced by field applications, in particular to identify and delete irrelevant events from traces that do not offer interesting information for offline analyses.
Before deploying the application, practitioners select a subset of program variables to be used to represent the program state, then while the application is running in the field, the state of these variables is regularly saved before and after each monitored event.
In a second step (i.e., offline time), the technique divides the full trace in several pieces using the variables state as splitting points. After this operation, the technique deletes all the events that do not change the program state and those events that whose occurrence can be re-ordered without affecting the program state, leaving in the trace only the most relevant information for understanding the program behavior.

Contrary to \CBR, this technique does not take into account the monitoring overhead introduced by the action of regularly saving state information, besides the fact that the way the state representation is obtained is specified manually, while  \CBR performs this operation in an automated way.

The heuristic used in \CBR to merge abstract states and produce a finite-state representation of the observed behavior is similar to the one used in some automata inference techniques~\cite{Dallmeier:Adabu:WODA:2006,Marchetto:Ajax:ICST:2008,Mariani:Revolution:ISSRE:2012}. However, none of these approaches are designed to work with bursts as defined in this paper.


Finally, some techniques can be generally useful to optimize resource consumptions and further reduce overhead, such as Delayed Saving that can reduce the cost of persisting the information about the collected events~\cite{Cornejo:DelayedSaving:IEEEAccess:2019}. These kinds of approaches can be integrated in \CBR to further improve its performance. 

%%Literature on FSAs

% The literature on synthesizing \FSAs that describe the behavior of a system is vast, some particularly relevant works include Wil van der Aalst's~\cite{van2016process} book, entirely devoted to mining processes from observed data. 
% Also, Lorenzoli et al.~\cite{lorenzoli2008automatic} worked on \textit{GK-Tail}, a technique for automatically generating extended finite state machines from interaction traces. The technique focuses on the relations between constraints on data values on component interactions, retrieving more accurate models for analysis and testing techniques.
% In the same direction, Krka et al.~\cite{krka2010using} developed a \FSA inference technique that uses not only execution traces but also program invariants in order to obtain relevant internal state information of the program variables and to produce more reliable models. 
% Recently, Walkinshaw et al.~\cite{walkinshaw2016inferring} proposed an approach for inferring extended \FSAs from software executions, this work focuses on addressing the non-determinism and the inflexibility problem of automatically generated \FSAs.

==> after rev/results.tex <==
% !TEX root =  main.tex

\section{Results}\label{sec:cbr_results}

In this section we present the results of the experiment we conducted to validate \CBR. All the experiments were executed on a computer running macOS version 10.13.6 with a 3.1 GHz Intel Core i7 processor and 16 GB of RAM.

%The following sections describe the results obtained to answer to the different research questions

\subsection{RQ1: Performance}

To answer the research question \textbf{RQ1: What is the overhead introduced by \Controlled?} we assessed the impact of the monitors, collecting data about their overhead. To this end, we repeated the execution of our 25 test cases 3 times obtaining 3,459 measurements of the response time of each operation when the various types of monitors are active. Based on the categorization of the operations presented in the previous sections (we assigned the category to each operation considering the system response time of the application without any monitoring), we collected data from 915 operations in the Instantaneous category, 25 operations in the Immediate category, and 213 operations in the Continuous category. Given the nature of the functionalities tested, we did not identify operations in the Captive category.

%In addition to measuring execution times, we collect the execution traces that will be useful for answering the research questions \textbf{RQ2} and \textbf{RQ3}.
%Since this work is focused on understanding the impact of the monitoring on the system response time (imaging how a future user may then perceive the resulting system), %user experience, 
%we classify user actions according to its original system response time category (i.e., Instantaneous, Immediate, Continuous and Captive actions).


\begin{table}[h]
\centering
\caption{Performance results with respect to SRT categories.}
\label{table:performance_results}
\scriptsize
\begin{tabular}{lcccc}
\toprule
  \multirow{ 2}{*} {\textbf{Monitoring Technique}} & \multicolumn{3}{c}{\textbf{Monitoring Overhead {[}\%{]}}} \\ 
\cmidrule(l){2-4}
%\textbf{Monitoring Technique} & \textbf{Instantaneous} & \textbf{Immediate} & \textbf{Continuous} \\ 
& \textbf{Instantaneous} & \textbf{Immediate} & \textbf{Continuous} \\ 
\midrule
\CBR & 123.78 & 40.70 & 0.71 \\ 
Sampling (P: 10\%) & 17.03 & 4.65 & 1.37 \\ 
Sampling (P: 5\%) & 7.12 & 2.88 & 0.28 \\ 
\bottomrule
\end{tabular}
\end{table}

The mean overhead introduced by each approach can be found in Table~\ref{table:performance_results}. Note that the overhead produced by \CBR corresponds to the overhead experienced while recording every call executed while processing an operation. On the contrary, sampling techniques record only a subset of the methods executed while processing operations. 

%In the table, \CBR represents \Controlled, \textit{Sampling 1} the monitor that traces in a sampling way with 10\% probability and \textit{Sampling 2} the monitor that samples with 5\% probability.
%\begin{TBF}We used a setup where \CBR is always recording: this is the worst case (and not the foreseen one, since \CBR should monitor with some probability), so that we can report the highest overhead we could get, and from this value we could derive the others overhead simply calculating the percentage of the applied recording probability. For the other two monitors, we report the mean of all the system response times, considering both those recorded (so with overhead) and those not recorded (so with the original system response time).\end{TBF}
%\danyB{ma qui CBR ogni quanto e' attivato?}

For the operations that require less than a second to execute (i.e., Instantaneous and Immediate), \CBR introduces considerable more overhead than the other sampling techniques. %(123.78\% compared to 17.03\% and 7.12\% when monitoring Instantaneous actions, and 40.70\% compared to 4.65\% and 2.88\% when monitoring Immediate actions). 

The higher overhead introduced for operations that can be completed in less than a second is explained by the need of recording the information about the abstract states before and after each burst. Indeed the absolute overhead is still small: for instance, the slowest Instantaneous operations may go from 200ms (its maximum time from the category) to 450ms with the overhead, which is still a difference that can be hardly recognized by users, as also confirmed in other studies where overhead levels up to 180\% are reported as hard to detect for Instantaneous operations, as long as introduced for a few operations in a row~\cite{NIER17, Cornejo:FunctionCallMonitoring:JSS:2020}. 

On the contrary, \CBR performs well with Continuous operations, where high overhead values may result in noticeable slowdowns for the users. Indeed, the cost of collecting state data is well compensated by the duration of the operations.

%The second thing we notice is that contrary to Instantaneous and Immediate actions, \CBR performs equally for actions $> 1$ second (i.e., Continuous actions), in fact \CBR introduced 0.71\% of overhead, which is similar to the performance of Sampling 1 (1.37\%) and Sampling 2 (0.28\%). Since these actions are less volatile, the task of evaluating program state does not impact on the final overhead.

%Finally, sampling monitors collect function calls probabilistically, which imply that only a subset of the method calls generated by user actions are collected, while \CBR collects all the method calls produced in the scope of a user action.  %for each user action: in this setup consequently, the overheads obtained with the sampling monitors are a mean of actions with and without monitored function calls, while all the user actions in \CBR are interested by the monitoring activities.
% \begin{TBF}
% 	However, from our human-subject studies results (see X) we discovered that users do not perceive high monitoring overhead levels for Instantaneous actions, and that users perceive a degradation of the system response time only at 140\% for Immediate actions, meaning that in practice, users would not perceive monitoring overhead when \Controlled is activated.
% \end{TBF}

%However, previous user studies~\cite{NIER17} proved that users do not perceive high monitoring overhead levels for Instantaneous actions, and that users start to perceive a degradation of the system response time only within the range 80-180\% for Immediate actions, meaning that in practice users would not perceive monitoring overhead when \Controlled is activated.

%Moreover, Sampling 1 and 2 techniques are not useful for simulating possible executions from the field, since they are observing only small percentages from the execution and do not provide contextual information, while \CBR is capable of representing comprehensive behaviors from the traces signed with program state information.

In summary, \CBR is more expensive than sampling techniques due to the state abstraction and recording activities performed when a burst is recorded. The relative extra overhead is significant for operations that complete quickly, but still hardly recognizable in terms of the absolute slowdown, while the overhead introduced in longer operations to record state information is compensated by the length of the operation. 


\subsection{RQ2: Precision}\label{sec:acc_results}


% \input{tables/accuracy_results}
% \input{tables/completeness_results}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/accuracy_results}
\caption{Precision results with respect to different runs of the application.}
\label{fig:precision_results}
\end{figure}

For answering the research question \textbf{RQ2: What is the precision of the model generated by \Controlled?} we measured the precision of the information reported in the model generated by \CBR with respect to the set of original traces. % collected with monitoring.
We only show results for \CBR, since it is the only technique that recombines bursts to obtain a more comprehensive model, possibly introducing imprecision. On the contrary, sampling techniques do not recombine the recorded information, thus the portion of traces collected are always precise, that is, every sequence of method calls recorded corresponds to an actual sequence produced while running the software.

Since \CBR collects a burst with a given probability, we studied how precision changes with respect to the probability to record the bursts and the number of executions of the monitored software. The results are reported in Figure~\ref{fig:precision_results}. 

%\CBR works in a probabilistic way, meaning that the monitoring of each interaction between the user and the application occurs only under a certain probability. 
%If \CBR is deployed to monitor data with a probability lower than 100\%, it is necessary to run several times the same functionality in order to observe the whole behavior in the field. 
%Since in practice a program is executed several times in different instances, we would collect several repeated observations of the same functionality throughout the monitoring process, and by increasing the number of runs of the monitor fewer samples will be needed in order to derive accurate results. In our experiment, we executed \CBR ranging the probability of monitoring a user action from 5\% to 100\% with a step of 5\%, and for each setup we executed 1, 5, 10, 15 and 20 runs.

%Figure~\ref{fig:precision_results} shows information about precision of \CBR given the sampling probability and the amount of runs of the application. 
%In Table~\ref{table:accuracy_results} we present how the overall precision changes according to the number of observed runs of the application, in this case, we experimented with 1, 5, 10, 15 and 20 runs.

The ability to recombine bursts produces a loss of precision of about 20\%. Interestingly, \CBR reaches its maximum precision level quite quickly. With the exception of data collected from a single execution, which clearly provides imprecise and unstable information, 15-20 runs with a sampling rate of 20\% are already sufficient to reach the maximum precision. If we reduce the sampling rate, we proportionally need more executions to  obtain the same amount of information. For instance, the same results obtained for 15 runs observed with a probability to collected a burst equals to  20\% could be approximatively obtained with a probability equals to 2\% after having observed 150 runs. Assuming to keep \CBR active in the field for long time, bursts could be feasibly collected with a probability lower than 1\%.

%A lower sampling rate could also be used, this would proportionally require more execution to achieve the same amount of evidence collected and thus the same precision. In particular, monitoring applications for long time observing hundreds or thousands of executions feasibly allow to reduce the sampling rate below 1\%.

%Note that the 20\% of combinations of bursts that occur in the model but do not occur in the traces are not necessarily infeasible behaviors, but can also be feasible behaviors that have not been exercised so far.

%all the other configurations reach   
%
%First, we observe that the maximum precision of the technique is around 81\% (with only one run is normal that the possible traces from the generated FSA are more realistic since there are less possible combinations, so that we reach 100\% too once), this means that for every node in the \FSA, 81\% of the possible combinations of bursts are a feasible behaviors of the application, while the remaining 19\% are traces that we never observed in the traces recorded when activating \CBR all the times (complete traces). 
%
%However, not all the 19\% are unfeasible traces for sure: a subset of the traces represented by the remaining 19\% could still be possible behaviors of the software, but we may have not developed all the necessary test cases to cover the remaining 19\%.
%
%Second, we note that with 5 runs of the application we achieve the maximum of the precision for our technique with a sampling probability of 50\%. 
%Instead, when considering 10, 15 or even 20 runs, the maximum precision can be achieved with a 25\% sampling probability, which seems to be the more balanced result for all measurements.

In summary, recombining bursts in a model as \CBR does may introduce imprecision. Based on our preliminary results, \CBR manages to represent combinations of bursts that correspond to actually observed behaviors in 80\% of the cases, while 20\% of these combinations represent behavior not observed in the traces.

\subsection{RQ3: Recall}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/completeness_results}
\caption{Recall results with respect to different runs of the application.}
\label{fig:recall_results}
\end{figure}

In this section, we present the results for the research question \textbf{RQ3: What is the recall of the traces produced by \Controlled?} 
% To estimate the recall we measure the percentage covered by traces obtained with each monitor in comparison to those obtained with \CBR monitor activated all the time.


We consider the ability of the various monitoring techniques to capture the behavior observed in the field. Sampling techniques do not have the ability to recombine observations, thus they can capture only short prefixes of the executions that happen in the field. Thus, if sampling has a precision equals to 1 by construction, it has also a nearly 0 recall by construction. In our evaluation, the recall of the sampling techniques ranged from 4.15\% to 7.77\%.

The main objective of \CBR is to obtain a better recall recombining the collected bursts \begin{mod}without annoying the end user\end{mod}. In Figure~\ref{fig:recall_results} we plot how the recall of the model produced by \CBR changes for different sampling probabilities (i.e., different probabilities of recording a burst when a user %action 
\begin{mod}operation\end{mod}
is performed) and different number of collected executions.   


%Figure~\ref{fig:recall_results} shows the recall of the technique according to the sampling probability and how it changes according to the number of runs of the application. 
% The recall is presented in two measures, the \textbf{RB} and \textbf{RE} indicators: 
% the \textbf{RB} indicator shows the recall percentage with respect to the number of bursts that can be identified within the original traces in comparison to the simulated trace.
% Instead, the \textbf{RE} 

%The lines in Figure~\ref{fig:recall_results} represent the recall percentage with respect to the number of events that can be identified in the original traces in comparison to the traces simulated by the \FSA.

Interestingly, 10 runs of the applications are already sufficient to obtain 90\% recall with a 30\% sampling probability. Again, collecting additional executions allows to reduce the sampling probability still retaining a similar recall, that is, a 3\% sampling probability may approximatively lead to similar recall after the observation of 100 runs. 

%Assuming to run \CBR consistently in the field and collecting thousands of executions, a similar recall level can realistically be achieved with a sampling rate below 1\%.

%We notice that considering only one run of the application we only achieve 100\% recall with sampling strategy at 100\%, which means having the monitor always on. When we decrease the sampling probability to 90\%, the recall of the technique decreases rapidly to 36\%. 
%
%Given that we are considering only one run, it is very likely that our \FSA is missing several transitions and thus producing very short and incomplete traces. In fact, when considering 5 runs of the application it is possible to achieve a good recall percentage with 65\% of sampling probability.
%
%Now, if we consider 10 runs of the application we obtain approximately $90\%$ of recall at a 45\% of sampling probability. Going further, for 20 runs of the applications we already obtain a good recall level for 25\%, which is also a similar result obtained for precision in the previous section.

%On the other side, for sampling monitors we obtained a recall value of 4.15\% (in Figure \ref{fig:recall_results} the two lines are overlapping), with a maximum recall of 7.77\%, meaning that the traces collected by this approach contains on average 4.15\% events from the total events contained in the traces obtained when activating \CBR all the times. %\danyB{io purtroppo non riesco ancora a capire la differenza fra questi monitor probabilistici e CBR attivato con probabilita'... e non capisco perche' per la precision non li abbiamo riportati}

In summary, sampling strategies largely miss the ability to reconstruct the observed executions. On the contrary, \CBR can obtain high recall values by recombining the collected bursts.


%\subsection{Threats to Validity}
%We studied the effectiveness of \CBR with a case study based on ArgoUML that we used to compare the effectiveness of the presented approach to sampling strategies. Our study provides an initial evidence of the effectiveness of the approach in the specific setting that we  



\subsection{Threats to Validity and Discussion}
We studied the effectiveness of \CBR in comparison to sampling strategies with a case study based on ArgoUML. We cannot make claims about the generalizability of the results, however, the presented study provides an initial evidence of the complementarity between \CBR and sampling. 
Sampling techniques are useful when collecting extensive evidence of the field behavior is not important, but collecting small but precise evidence is the priority. On the contrary, \CBR can be used when full precision of the extracted information is not a mandatory requirement, and obtaining a comprehensive representation of the observed behavior is more important, for instance to support heuristic program analysis and profiling techniques: \begin{mod}in these cases, \CBR represents a good tradeoff between the introduced overhead, almost not recognizable when using a low sampling rate, the high recall of the collected traces, and the good precision of the reconstructed traces.\end{mod}

==> after rev/step1.tex <==
% !TEX root =  main.tex
\subsection{Step 1: Class Detection}

The \textit{Class Detection} step identifies the set of classes that may directly or indirectly determine the sequence of execution of the methods in the target components specified by the developer. These classes are automatically identified by first computing the dependency graph of the classes in the program. Then \CBR transitively follows the dependency edges in the graph starting from the target classes. Every class reached during this process is included in the set of the relevant classes analyzed in the second step of the process. 

In the running example the process is quite simple and both the \texttt{Cart} and the \texttt{Product} classes are selected. 


%Then, with the help of WALA~\cite{WALA} static analysis tool, \CBR constructs the Class Hierarchy of the program under monitoring and extracts all the classes that match the scope of the monitoring. 
%So in our example \CBR considers the \texttt{Cart} and its \texttt{Product} inner class for the analysis.
%
%Later, we save the meta-data of all methods existing inside the classes we already gathered through the Class Hierarchy.


==> after rev/step2.tex <==
% !TEX root =  main.tex
\subsection{Step 2: Function Extraction}\label{sec:SD}

\CBR analyzes the relevant classes identified with step 1 to extract the abstraction functions, which capture \emph{conditions} that represent how the values of the state variables may influence the execution of the monitored program. The abstraction functions provide a natural and efficient abstraction mechanism that can be applied at runtime to generate an abstract representation of a program state.
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=\columnwidth]{figures/abstract_functions}
%    \caption{Function Extraction process.}
%    \label{fig:abstract_functions}
%\end{figure} 

To generate the abstraction functions, we use symbolic execution~\cite{Baldoni:2018:SSE:3212709.3182657,Braione:Enhancing:FSE:2013}. The main intuition is that each method in each relevant class can be executed symbolically to derive the \emph{path conditions} corresponding to all the paths that can be executed up to a given bound. Each path condition represents a set of conditions over the state variables and the inputs of the program that may drive the execution toward a specific computation (i.e., towards a specific path from the entry of the method to an exit point). For example, the condition \texttt{Cart.products.length==0} identifies a specific path of the program in the \texttt{calculateTotal} method (the path that does not enter in the \texttt{for} loop at line 33) and can be evaluated at runtime to distinguish the state that may lead to one path rather than another when the \texttt{calculateTotal} method is executed. 

When deriving path conditions from methods, the conditions may include clauses containing the input parameters of the processed methods. Since these path conditions are used to derive abstraction functions that might be computed at any time of the execution of a program, and not necessarily when methods with specific parameters are invoked, these clauses are removed from the path conditions when turning them into abstraction functions. For instance, the abstraction functions resulting from the symbolic execution of the methods in the \texttt{Cart} class are shown in Table~\ref{table:abstractfunctions}.


%In particular, we use the JBSE~\cite{Braione:Enhancing:FSE:2013} symbolic executor bounding the exploration of loops to ?????. in each selected class and use the path conditions resulting from the analysis of each method as functions for state abstraction. 
%A \textit{path condition} is a condition on the state variables of a program, and the Abstraction Functions are the application of these conditions to the program state.

%Note that a \textit{path condition} represents how the inputs to a method, that is, the values of the parameters and the values of state variables, relate to the execution of a specific path inside the method. \textit{Path conditions} are a good abstraction because they explain how applications use inputs and state variables.

%For instance, the Abstraction Functions could be composed by a particular function that checks if the number of products in a shopping cart is greater than zero to decide how to use the shopping cart: in this case it would be enough to record whether the condition \texttt{nrProducts > 0} is true or not when saving state information, with no need of recording the actual number of products, which would be irrelevant to determine how the execution may proceed.

%The abstraction functions capture relevant state properties and represent the different execution paths, which in turn may produce different sequences of invocations to the monitored classes.  
%Each evaluation of these functions at runtime produces the program state of the application.

\input{tables/af.tex}

When an abstraction function is evaluated at runtime, it is evaluated against the state of the program. \CBR uses a monitor to intercept the creation and the destruction of the monitored objects of the program so that functions can be evaluated efficiently on the existing objects. A function evaluates to true if it exists a set of objects in the program state that can satisfy it. For instance, the first abstraction function in Table~\ref{table:abstractfunctions} evaluates to true if there exists a cart with at least one element.

In addition to true and false values, an abstraction function can also produce the value \emph{unknown}. This happens when some of the elements that appear in the abstraction function cannot be evaluated. For instance, the clause \texttt{Cart.products.[0].taxFree == true} evaluates to \emph{unknown} if there is no element at the position 0 of the array. If a clause evaluates to unknown, the full abstract function returns unknown.


The result of the evaluation of a set of abstraction functions is an array of ternary values, referred as the \emph{Abstract Program State}. More formally, given a program $P$ with a concrete state $S$, its abstract program state $abs(S)= \{v_i | v_i = f_i(S), \forall f_i \in AF\}$, where $AF$ is \begin{mod}an ordered\end{mod} set of the available abstraction functions. \begin{mod}Note that the specific ordering is not important, but it is important to keep it consistent across all the evaluations so that the abstract states are comparable, that is, the value $v_i$ in an abstract state must be produced by the same function $f_i$ every time the abstract state is computed.\end{mod} 

%
%\smallskip
%\noindent \begin{footnotesize}\texttt{Cart.nProducts != 0 \&\& Cart.products.length >= 0}\end{footnotesize}
%\smallskip
%
%evaluates to \texttt{true} when there is at least one \texttt{Product} in the shopping cart, while it evaluates to \texttt{false} if the shopping cart is empty. Finally, it evaluates to \texttt{unknown} if the \texttt{Cart} object is not available.
%
%Similarly, the \texttt{applyDiscount - Function 4} in Table~\ref{table:abstractfunctions}
%
%\smallskip
%\noindent \begin{footnotesize}\texttt{Cart.nProducts > 0 \&\& Cart.products.length > 0 \&\&} \newline\texttt{Cart.products.[0].value < Cart.PRICE}\end{footnotesize}
%\smallskip
%
%evaluates to true when the cart is not empty and the price of the first \texttt{Product} in the cart is higher than the \texttt{PRICE} constant, and evaluates to false whether the cart is empty or the price of the first \texttt{Product} is lower than the \texttt{PRICE} value. It evaluates to unknown when the object \texttt{Cart} does not exist in memory.



%=================== DOPO 
%When the program under monitoring is executed, \CBR produces a number of bursts consisting of an evaluation of the extracted functions on the state of the program, a sequence of events (each event is a method invocation), and again an evaluation of the functions on the state of the program. 
%
%The organization \texttt{state - burst - state} is useful because allows \CBR to understand the sequentiality of bursts. Since the states give information about the current program state, it is possible to correlate different bursts collected at different times comparing their states' values, to obtain a more comprehensive knowledge rather than considering only one burst.
%
%Considering the previous example of the program exploiting the \texttt{Cart} class, a burst of its execution could take the form:
%
%\smallskip
%\noindent \begin{footnotesize}\texttt{(U, U, F, T) addItem(product) calculateTotal() \ldots emptyCart() (T, T, F, T)}\end{footnotesize}
%\smallskip
%
%where the part between parentheses is the Abstract Program State, which includes the evaluation of the functions identified in the function extraction analysis  \danyB{ma non sono quelle in tabella 1? sono molte di piu, qui invece son 4. Ci aggiungo questa frase, ma non se se sia giusta: and filtered in the training phase, as explained in the next section, to keep the most relevant ones only}, and the sequence of labels between the two instances of the Abstract Program State is the sequence of events collected at runtime.
%
%Considering the first \APS of the burst, let us assume that the first value refers to the mentioned Function 1 on the method \texttt{addItem}: the U in the program state means that, when the monitor started that trace recording, that function was evaluated as unknown, while at the end of the trace it turned to be true.
%=================== DOPO 



==> after rev/step3.tex <==
% !TEX root =  main.tex

\subsection{Step 3: Function Filtering}\label{sec:monitor}

Symbolic execution normally produces a large number of path conditions since it considers every possible execution path for every method under analysis up to a given bound. Turning all the resulting path conditions into abstraction functions to be used in the field would not be practical and would cause unacceptable overhead levels. %, and thus affecting the user experience. 
For this reason, \CBR filters out the least useful path conditions returned by symbolic execution, to guarantee a good compromise between the accuracy of the state information that is traced and the cost of producing such a state information.

From the original set of path conditions, \CBR just needs the ones that give unique information about the behavior of the application, that is, information that is not subsumed by the information provided by the evaluation of the other functions. 
To find the optimal set of conditions to be used as abstraction functions, \CBR assesses the available conditions against a set of test executions and discards the ones that do not contribute in distinguishing the program states. 

In particular, \CBR executes the monitored program covering diverse scenarios (e.g., using a set of system test cases) and evaluates all the available abstraction functions every time a method of the program is invoked. This produces a large number of evaluations for all the available abstraction functions. The collected data can be represented in a matrix where the abstraction functions appear on the columns and the evaluations on the rows. Each row corresponds to an evaluation of all the abstraction functions performed at the time a method was invoked (the specific method is not relevant). On the other hand, each column includes all the values that have been returned by an abstraction function across all the function evaluations that have been performed. Each cell may evaluate to true (T), false (F), or unknown (U). Figure~\ref{fig:matrix} shows a sample matrix with 7 abstraction functions evaluated 5 times.


%
%\danyB{La descrizione sotto della matrice mi sembra poco comprensibile, non sono sicura di capirla neppure io (non ricordando piu' bene come funzioni questa fase... ma non so bene come aggiustarla. mi sembra confusa la parte di kl).For every method call, we collect a sample, that is in our case, the set of the values produced by evaluating each \AF in that moment. We collect these samples as rows in a matrix with \AF columns. So, we will have $l$ matrixes coming from $l$ executions of different parts of the program under monitoring, each one with the same number of columns (the \AF 's number) and different rows (depending on the function calls of each execution).}
%
%For each user execution $l$ we generate a matrix $E_{iJ}^l$, with $i = 1 \ldots k_l$ being $i$ a sample observed in the field with $k_l$ being the number of samples observed in the $l$-th execution, and $J = 1 \ldots n_{af}$ being $J$ the abstraction functions under observation and $n_{af}$ the total number of \AFs.
%For instance, in Figure~\ref{fig:samples} we show two examples of executions, with $n_{af} = 7$, collected in the field: Execution 1 ($E^1$) with $k_1 = 3$ and Execution 2 ($E^2$) with $k_2 = 2$. 
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.6\columnwidth]{figures/samples}
%\caption{Sample matrix with 5 evaluations of 7 abstraction functions.}
%\label{fig:samples}
%\end{figure}
%
%After collecting information for each execution, we organize the several $\{ E_{ij}^1, E_{ij}^2, \ldots, E_{ij}^{L} \}$, with $L$ the total number of executions, into a matrix $M_{ij}$, where $i$ (rows) ranges from $1$ to the sum of all samples 
%$\sum_{l = 1}^L k_l$
%gathered at runtime, while $j$ (columns) goes from $1$ to $n_{af}$.
%The matrix $M_{ij}$ is obtained as $M = \{E^1 \diamond E^2 \diamond \ldots \diamond E^{L}\}$, where the $\diamond$ operator represents the vertical concatenation of the $E_{iJ}^l$ matrices.
%For instance, considering $E^1$ and $E^2$ the executions of our example, the operation $E^1 \diamond E^2$ would generate the matrix presented in Figure~\ref{fig:matrix}.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\columnwidth]{figures/matrix}
\caption{Sample matrix with 5 evaluations of 7 abstraction functions.}
\label{fig:matrix}
\end{figure}

The filtering process goes through four steps that reduce the size of the matrix, until reaching a small number of abstraction functions that are really indispensable to generate the abstract program states. The four steps are: \textit{Removal of Duplicated Samples}, \textit{Removal of Non-Discriminating Abstraction Functions}, \textit{Removal of Equivalent Abstraction Functions}, and finally \textit{Removal of Redundant Abstraction Functions}. Figure~\ref{fig:pc_filtering} shows the four steps applied to the matrix in Figure~\ref{fig:matrix}. We describe the four steps below.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{figures/pc_filtering}
\caption{Example filtering process.}
\label{fig:pc_filtering}
\end{figure}

\smallskip

\textit{Removal of Duplicated Samples}: this step reduces the size of the matrix by removing duplicated rows, which are useless for the purpose of determining the ability of the functions to distinguish different concrete states. In addition to increase the efficiency of the next steps, since the matrix becomes smaller, this step is necessary to facilitate the identification of the redundant functions (see last rule). Formally, given the matrix $M_{ij}$ with $i=1 \ldots K$, $j=1 \ldots N$, two rows $M_{i_{1}}$ and $M_{i_{2}}$ are duplicated if $M_{i_{1}j} = M_{i_{2}j}$ for all $j = 1 \ldots N$.
In our example, the second and third rows are duplicated and thus only one of them is preserved for the rest of the analysis. 

\smallskip

\textit{Removal of Non-Discriminating Abstraction Functions}: this step eliminates those abstraction functions that never change their values throughout all the evaluations, being de facto constant, and thus not contributing to distinguishing the program states at runtime. These functions can be for instance the result of the analysis of infeasible program paths. More formally, an abstraction function in column $J$ is non-discriminating if $M_{1J} = M_{2J} = \ldots = M_{kJ}$.
In our example, the abstraction functions AF1 and AF3 are non-discriminating and are thus removed from the matrix.

\smallskip

\textit{Removal of Equivalent Abstraction Functions}: this step eliminates abstraction functions that consistently return the same abstract values. Indeed, keeping only one of this function is enough. More formally, two functions in columns $j_1$ and $j_2$ are equivalent if their columns are the same, that is, $M_{ij_1} = M_{ij_2}$ for all $i=1...k$. In the example, AF2 and AF6 are equivalent, thus AF6 is dropped from the matrix.

\smallskip

\textit{Removal of Redundant Abstraction Functions}: this step %\begin{mod}empirically\end{mod} 
removes the abstraction functions that are not needed to actually distinguish the possible program states. The process works by removing one abstraction function at time (i.e., one column at time) and checking if the remaining functions are still sufficient to distinguish all the abstract program states collected so far. If a column is not needed, no rows become equal due to a column dropped from the matrix, that is, the available states can still be distinguished with the remaining functions. Note that after the application of the first rule, only distinct rows remained in the matrix: each row is thus a distinct abstract program state discovered by the tests. If the removal of a column generates two equal rows, it implies that the remaining functions are not sufficient to distinguish the actual states of the program. 
The application of this process to our example causes the removal of functions AF2 and AF4.

\smallskip

The functions that remain at the end of this process (i.e., the remaining columns) are the ones used to produce the abstract states at runtime. In our example, the two remaining functions are AF5 and AF7.

==> after rev/step4.tex <==
% !TEX root =  main.tex
\subsection{Step 4: Bursts Collection}\label{sec:collect_bursts}

\CBR records bursts synchronously with user \begin{mod}operations\end{mod}, to make sure to collect state information when the monitored application is in a sound and steady state. In particular, when the user interacts with the application \begin{mod}asking for an operation, \end{mod}%producing a request, 
\CBR decides with a given probability if a burst must be collected. If the burst is collected, the abstract state corresponding to the current concrete state is collected, the actual burst is recorded (e.g., the sequences of methods executed as a consequence of the \begin{mod}request\end{mod}), and when the monitored application has completed the computation and has produced a result, the abstract state is collected again. More formally, a burst $B$ is a tuple $B = \langle label, abs(S_a), trace, abs(S_b) \rangle$, where $label$ is the user \begin{mod}operation\end{mod} that originated the burst, $abs(S_a)$ and $abs(S_b)$ are two abstract states collected before and after the execution of the burst, and the trace $trace$ is the sequence of events (method calls in our case) collected in the field.

While a program is used, a number of bursts $B_1 \ldots B_n$ are collected and used in the final step to reconstruct a representation of the behavior of the program.

%
%%Since the technique traces bursts of the execution signed with program state information, we are not forced to record sequentially all bursts that occur in the field, that would correspond to continuously collect all the program execution interfering with the user activities. The program state information helps us to acquire a logical order of the different independent bursts collected at different times during different executions under monitoring.
%
%%The sampling probability of \CBR will be then estimated experimentally, testing with different probabilities to search for the best cost-benefit compromise in terms of quality of the solution.
%
%Let $Abstraction$ be the \AF (the set resulting from step 3) that applied to a certain concrete state $S$ of a program produces an Abstract Program State $S_a = Abstraction(S)$.
%
%Following our example, some of the recorded bursts may for example look like:
%
%\smallskip
%
%\noindent \begin{footnotesize}\texttt{(U, F) cart.applyDiscount() cart.calculateTotal() \ldots (F, F)}\end{footnotesize}
%\smallskip
%
%When the action \textit{pay total} is performed, \CBR saves the \APS $(U, F)$ plus the target methods of the analysis, then \CBR saves again a new representation of the \APS equal to $(F, F)$.


==> after rev/step5.tex <==
% !TEX root =  main.tex

\subsection{Step 5: Model Synthesis}\label{sec:simulating}

The set of bursts represent chunks of executions collected in different instants. Each burst carries some knowledge about the behavior of the system, that is, how a user %request 
\begin{mod}operation\end{mod}
made the monitored system to change from a given (abstract) state to another (abstract) state, and the relative internal computation that has been observed (e.g., the sequence of method calls). It is however important to gain a comprehensive picture of how an application or a set of components behave in the field, putting the collected bursts in context. This is something sampling techniques that collect bursts without context cannot do~\cite{Hirzel:BurstyTracing:FDDO:2001}, while controlled burst recording can do thanks to the presence of the state annotations.

\CBR generates a finite state model to capture the knowledge extracted in the field. In particular, it produces a finite state model (FSM) where state transitions are annotated with information about the computations that may happen in the target components when that specific transition is executed.

The way the FSM is reconstructed is driven by the abstract states, that is, each distinct abstract state in the recorded bursts is a different state of the FSM, and the user %requests 
\begin{mod}operations\end{mod}
are transitions in the FSM. The content of the burst produces the annotations.  More formally, an annotated FSM is a tuple $G = (S,T, a)$, where $S$ is a finite non-empty set of states,  $T \subseteq Label \times S \times S $ is a finite set of transitions between states in $S$ with a label in $Label$, and $a: T \rightarrow \mathbb{TRACE}$ is a function that associates each transition in the model with a set of traces ($\mathbb{TRACE}$ denotes the powerset of all the possible traces). Note that the FSM captures various state transitions that have been observed in the field without encoding a notion of initial and final states.  


Given a set of bursts $B=\{B_1, \ldots B_n\}$, with $B_i = \langle label_i, abs(S_a)_i, trace_i, abs(S_b)_i \rangle$, the corresponding FSM $(S,T, a)$ is defined as follows.
\begin{itemize}
\item $S=\bigcup_i (abs(S_a)_i \cup abs(S_b)_i)$ is the union of all the states in the bursts,
\item $T=\{(l, s_a,s_b) | \exists b \in B \wedge b= \langle l, s_a, trace, s_b \rangle \}$, is a representation of all the state transitions caused by the user \begin{mod}operations\end{mod} present in the bursts,
\item $a(t)=A$ with $t = (l, s_a,s_b) \in T$ implies $A= \bigcup_{\langle l, s_a, trace_j, s_b \rangle} trace_j$, is a function that annotates each transition with the corresponding set of traces. 
\end{itemize}
 
The model is simply created by sequentially mapping each burst into the corresponding states, transitions, and annotations. 

%At this point, we already gathered several independent bursts from the field, where each burst explains the effect of each user action on the program state. 
%The issue is that each burst by itself provides partial information about a full execution. To overcome this issue, \CBR puts together all the bursts in a common structure. 
%
%The right structure to assemble the different bursts is a \textit{Finite State Automaton}: in fact, a \FSA is a natural representation for traces with states and transitions. In our case, the \FSA will show how the application's state changes according to different users' actions. \danyB{oscar, hai una ref da mettere qui?}
%
%To decide how to synthesize the \FSA, \CBR exploits state information contained in the different bursts: if a burst $B_1$ ends with an abstract program state $S_2$ that matches the abstract program state $S_1$ reported at the beginning of another burst $B_2$, then the two bursts $B_1$ and $B_2$ can be concatenated by a node containing the state information in common between both bursts.

%The Finite State Automaton is a tuple $G = (S,M,s_0,s_F)$, where $S$ is a finite non-empty set of nodes representing the different \APS identified at the beginning and at the end of each burst, $M$ is a finite set of transitions between states in $S$ representing the different user actions monitored at runtime, $s_0 \in S$ is the initial state, and $s_F \subset S$ is the set of final states.
%
%So, for each monitored burst $B = \langle label, S_1\,T\,S_2 \rangle$, \CBR creates a transition $m \in M$ starting from state $S_1$ to $S_2$ with a specific label and a trace $T$. 
%Since it is natural that different users perform the same action in different scenarios, \CBR enriches the transition $m$ with more traces $T$. 
%
%The procedure of concatenating bursts is done iteratively for all bursts collected in the field. Certainly, as more bursts are used to create the graph, an increased number of program behaviors will be represented in it.
%
%To simulate possible traces (longer bursts, representing the function calls coming from longer application usages) of the application we again exploit state information. 
%Since we already built the \FSA as the tuple $G = (S,M,s_0,s_F)$, the procedure is straightforward: 
%consider two transitions $m_1, m_2 \in M$ connected by a common state $S_1 \in S$, \CBR generates a new burst $B'$ with (1) the initial state $S_i$ of transition $m_1$, (2) a new trace $T'$ made by the concatenation of the trace $T_1$ from $m_1$ with the trace $T_2$ from $m_2$ and (3) the final state $S_f$ of transition $m_2$.
%The new burst $B' = \langle label, S_i\,T'\,S_f \rangle$ contains the simulated trace represented by $T'$.
%
%The idea is to repeat this process until a larger trace is created.

\begin{figure}[h]
\centering
\includegraphics[width=0.70\columnwidth]{figures/burst_plus}
\caption{Excerpt of FSM derived from a set of bursts.}
\label{fig:burst_plus}
\end{figure}

Figure~\ref{fig:burst_plus} shows an excerpt of the resulting model. Each state of the model is a different abstract state of the program (for simplicity we only report two values in the represented states). The transitions show changes in the current state of the monitored components. Each transition is annotated with traces (as represented with dotted arrows in Figure~\ref{fig:burst_plus}). 

Note that all the steps of the approach are driven by the initial selection made by the user. Thus, both the derived abstraction functions and the resulting model specifically capture the behavior of the monitored components.  

In a nutshell, \CBR provides useful information at two different levels:
(1) it shows how the usage of the application affects the state of the monitored components, and 
(2) it shows the computations that might be produced in the monitored components every time a transition is traversed.

In the next section, we evaluate \CBR in comparison to other approaches for sampling executions from the field.

%
%
% \textit{clickOnAddItem} and \textit{clickOnPay}, that have in common the \APS \texttt{(U, F)}. In this case, we might concatenate Bursts 1 and 2  producing the following trace:
%
%\smallskip
%\noindent \begin{footnotesize}\texttt{(U, U) cart.addItem(prod1) \ldots cart.applyDiscount()\newline cart.calculateTotal()} \texttt{\ldots (F, F)}\end{footnotesize}
%\smallskip
%
%The generated traces could represent possible behaviors of the application: nevertheless, if the quality of the model is not good, the procedure could derived unfeasible traces. This aspect will be covered in the next section.  
%
%In a nutshell, \CBR provides useful information at two different levels:
%(1) shows how the application is used in the field (\FSA) and 
%(2) through the traces simulated by the \FSA shows different possible uses of the components under monitoring.


==> after rev/tables/accuracy_results.tex <==
% !TEX root =  ../main.tex
\begin{table}[h]
\centering
\scriptsize
\caption{Precision results for \CBR.}
\label{table:accuracy_results}
\begin{tabular}{llllll}
\hline
 & \textbf{1 run} & \textbf{5 runs} & \textbf{10 runs} & \textbf{15 runs} & \textbf{20 runs} \\ \hline
\textbf{Probability {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} \\ \hline
5 & 0 & 66.67 & 68.42 & 70.21 & 68.11 \\ \hline
10 & 50.00 & 68.42 & 63.39 & 72.51 & 74.22 \\ \hline
15 & 100 & 70.73 & 72.36 & 76.62 & 78.83 \\ \hline
20 & 66.00 & 65.24 & 79.98 & 77.80 & 79.70 \\ \hline
25 & 55.35 & 66.67 & 80.27 & 79.97 & 80.43 \\ \hline
30 & 47.83 & 72.10 & 81.15 & 80.34 & 80.55 \\ \hline
35 & 38.89 & 79.61 & 80.83 & 81.22 & 80.25 \\ \hline
40 & 72.73 & 75.89 & 79.84 & 80.52 & 81.02 \\ \hline
45 & 64.62 & 79.95 & 80.55 & 80.62 & 79.88 \\ \hline
50 & 72.92 & 80.89 & 80.75 & 80.57 & 81.12 \\ \hline
55 & 65.87 & 80.16 & 80.66 & 80.62 & 80.39 \\ \hline
60 & 65.88 & 80.00 & 80.29 & 81.17 & 80.20 \\ \hline
65 & 66.82 & 80.98 & 80.52 & 80.43 & 79.92 \\ \hline
70 & 71.55 & 80.38 & 80.57 & 80.66 & 80.34 \\ \hline
75 & 78.14 & 80.41 & 80.89 & 80.75 & 80.48 \\ \hline
80 & 74.44 & 80.43 & 80.48 & 81.23 & 80.56 \\ \hline
85 & 75.23 & 81.23 & 81.07 & 80.48 & 80.41 \\ \hline
90 & 78.69 & 80.98 & 80.66 & 79.98 & 80.70 \\ \hline
95 & 79.52 & 80.70 & 80.75 & 81.02 & 80.49 \\ \hline
100 & 80.71 & 80.70 & 80.70 & 80.66 & 81.21 \\ \hline
\end{tabular}
\end{table}

==> after rev/tables/af.tex <==
% !TEX root =  ../main.tex

\begin{table*}[ht]
\scriptsize
\centering
\caption{Abstract Functions extracted from \texttt{Cart} class example.}
\label{table:abstractfunctions}
\begin{tabular}{lll}
\toprule
\textbf{Identifier}          & \textbf{Code ref.} & \textbf{Abstract Functions}                                \\
\midrule
addItem - Function 1        & Line 13  & \texttt{Cart.nProducts != 0 \&\& Cart.products.length \textgreater{}= 0}                                                           \\
addItem - Function 2        & Line 14  & \texttt{Cart.nProducts == 0 \&\& Cart.CART\_SIZE \textgreater{}= 0 \&\& Cart.nProducts \textless Cart.CART\_SIZE}                           \\
addItem - Function 3        & Line 14  & \texttt{Cart.nProducts == 0 \&\& Cart.CART\_SIZE \textgreater{}= 0 \&\& Cart.nProducts \textgreater{}= Cart.CART\_SIZE}                     \\
addItem - Function 4        & Line 13  & \texttt{Cart.nProducts == 0 \&\& Cart.products.length == 0}                                                                                 \\
applyDiscount - Function 1  & Line 26  & \texttt{Cart.nProducts \textgreater 0 \&\& Cart.products.length \textgreater 0}                                                             \\
applyDiscount - Function 2  & Line 26  & \texttt{Cart.nProducts \textgreater 0 \&\& Cart.products.length == 0}                                                                       \\
applyDiscount - Function 3  & Line 27  & \texttt{Cart.nProducts \textgreater 0 \&\& Cart.products.length \textgreater 0 \&\& Cart.products.{[}0{]}.value \textgreater{}= Cart.PRICE} \\
applyDiscount - Function 4  & Line 27  & \texttt{Cart.nProducts \textgreater 0 \&\& Cart.products.length \textgreater 0 \&\& Cart.products.{[}0{]}.value \textless Cart.PRICE}       \\
calculateTotal - Function 1 & Line 35  & \texttt{Cart.products.length \textgreater 0 \&\& Cart.products.{[}0{]}.taxFree == true}                                                     \\
calculateTotal - Function 2 & Line 37  & \texttt{Cart.products.length \textgreater 0 \&\& Cart.products.{[}0{]}.taxFree == false}                                                    \\
calculateTotal - Function 3 & Line 33  & \texttt{Cart.products.length \textgreater 0}                                                                                                \\
calculateTotal- Function 4  & Line 33  & \texttt{Cart.products.length == 0}                                                                                                          \\
emptyCart- Function 1       & Line 21  & \texttt{Cart.nProducts \textless{}= 0}                                                                                                      \\
emptyCart- Function 2       & Line 21  & \texttt{Cart.nProducts \textgreater 0 \&\& Cart.CART\_SIZE \textgreater{}= 0} \\
\bottomrule                                                             
\end{tabular}
\end{table*}

==> after rev/tables/completeness_results.tex <==
% !TEX root =  ../main.tex
\begin{table*}[!ht]
\scriptsize
\centering
\caption{Recall results for \CBR.}
\label{table:recall_results}
	\begin{tabular}{lllllllllll}
		\hline
		 & \multicolumn{2}{c}{\textbf{1 run}} & \multicolumn{2}{c}{\textbf{5 runs}} & \multicolumn{2}{c}{\textbf{10 runs}} & \multicolumn{2}{c}{\textbf{15 runs}} & \multicolumn{2}{c}{\textbf{20 runs}} \\ \hline
		\textbf{P [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} \\ \hline
		5  & 4.68  & 3.95  & 9.70  & 8.99   & 13.53 & 12.18 & 16.66 & 16.58 & 22.62 & 20.78 \\ \hline
		10 & 5.41  & 4.78  & 13.06 & 11.50  & 21.82 & 21.25 & 28.48 & 28.30 & 38.47 & 41.32 \\ \hline
		15 & 7.24  & 6.13  & 18.34 & 16.61  & 31.57 & 32.34 & 47.33 & 47.91 & 61.56 & 63.85 \\ \hline
		20 & 8.53  & 5.83  & 22.86 & 21.93  & 42.17 & 43.43 & 63.36 & 64.35 & 84.64 & 86.36 \\ \hline
		25 & 9.37  & 7.36  & 29.16 & 27.73  & 49.41 & 51.47 & 75.33 & 78.44 & 95.93 & 96.97 \\ \hline
		30 & 11.74 & 10.20 & 32.25 & 33.05  & 67.65 & 70.82 & 92.02 & 92.14 & 96.89 & 96.89 \\ \hline
		35 & 11.46 & 9.71  & 39.47 & 42.39  & 86.66 & 88.36 & 100 	& 100 	& 100 	& 100 \\ \hline
		40 & 14.32 & 12.21 & 42.65 & 44.97  & 84.80 & 85.45 & 100 	& 100 	& 100 	& 100 \\ \hline
		45 & 15.12 & 11.34 & 67.06 & 68.73	& 98.70 & 98.75 & 100 	& 100 	& 100 	& 100 \\ \hline
		50 & 15.59 & 14.31 & 61.44 & 62.82 	& 98.70 & 99.19 & 100 	& 100 	& 100 	& 100 \\ \hline
		55 & 17.56 & 17.44 & 87.95 & 88.89  & 98.59 & 99.14 & 100 	& 100 	& 100 	& 100 \\ \hline
		60 & 19.29 & 19.55 & 77.51 & 78.87  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		65 & 23.89 & 23.60 & 90.84 & 91.05  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		70 & 26.21 & 25.84 & 98.78 & 99.01  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		75 & 28.31 & 27.08 & 98.99 & 99.23  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		80 & 31.80 & 33.93 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		85 & 31.80 & 33.93 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		90 & 36.60 & 39.44 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		95 & 57.47 & 59.96 & 100   & 100 	& 100 	& 100 	& 100 	& 100  	& 100 	& 100 \\ \hline
		100 & 100  & 100   & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
	\end{tabular}
\end{table*}

==> bursts.tex <==
% !TEX root =  main.tex

\section{Field Bursts}\label{sec:bursts}

% All this knowledge can be represented as a Finite State Automaton, or \FSA for short, where the states represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. 

% Since several monitoring techniques in the literature collect method calls, eventually annotated with parameters or state information~\cite{ohmann2017lightweight,Jin:BugRedux:ICSE:2012,joshi2007scarpe,prepost,Cornejo:Flexible:ICSEC:2017,Cornejo:DelayedSaving:IEEEAccess:2019}, we also focus on the collection of this data type.

% In a nutshell, \Controlled is an approach that combines chunks of execution recorded at different times to produce insights about the field behavior of the application. With this approach we might loss full ordering of the events in the \FSA model, but since we are going to record partial traces at different times of the execution we expect not to impact on the user experience.

%definire un burst, ne spieghiamo l’utilità e spieghiamo anche l’utilità di metterli assieme.

A \textit{burst} is a stream of consecutive events collected in the field enriched with the state information at the beginning and at the end of each user action. 
In particular, a burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two concrete states of the application, initial and final respectively, and the trace $T$ is the sequence of events collected in the field.

Collecting bursts instead of full traces is useful because it allow us to spend less resources at runtime, in other words, there is no need for the monitor to be always on; since the technique traces bursts signed with program state information, we are not forced to record sequentially all bursts that occur in the field, that would correspond to continuously collect all the program execution interfering with the user activities. The program state information helps us to acquire a logical order of the different independent bursts collected at different times during different executions under monitoring.

All the knowledge learned through the collected bursts can be used to elaborate a Finite State Automaton, or \FSA for short, where the nodes represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. This strategy is useful because it will support practitioners to construct and simulate program scenarios from field executions without impacting on the user experience.


==> cbr.tex <==
% !TEX root =  main.tex

\section{Controlled Burst Recording}\label{sec:cbr}

%\leo{spiegare il valore dell’informazione estratta dal campo.}

\Controlled is a technique that represents the possible executions of an application in a Finite State Automaton structure; since this approach does not record full executions we might loss the full ordering of field events, but still a good representation of the behavior of the application can be given. From the generated model it is possible to extract accurate and comprehensive traces that could be useful for post-deployment analysis such as debugging, field failures reproduction, protocol verification, among others.

Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques~\cite{walkinshaw2008inferring}, such as detection of anomalous behaviors, protocol verification, testing, among others.

Usually the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon}~\cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 


==> controlledbust.tex <==
% !TEX root =  2018-PhDThesis-OscarCornejo.tex

\chapter{Controlled Burst Recording}\label{chapter:cbr}

This chapter presents \Controlled, a sampling technique for monitoring applications and for inferring knowledge from field executions with little impact on the user experience. This solution has been designed based on the results obtained with the user study we conducted for understanding the impact of monitoring on the user experience. This chapter presents also an empirical evaluation carried out on a real world application for assessing the efficiency and the quality of the approach, compared to other sampling-based techniques.

The presentation of the chapter is organized as follows. Section \ref{sec:inferring} presents an overview of the technique. Section \ref{sec:CBR} presents the \Controlled Framework and its different steps. Section \ref{sec:empirical_cbr} presents the empirical validation we conducted to assess our technique. Finally, Sections \ref{sec:cbr_results} and \ref{sec:cbr_discussion} discuss the obtained results and findings respectively.

\section{Inferring Knowledge from Field Executions}\label{sec:inferring}

\Controlled, or \textit{CBR} for short, is a technique to collect partial traces from the field. These traces could be used to produce a comprehensive knowledge about how an \textit{object-oriented} application is used by different users in a wide range of possible scenarios and configurations. 
In general, our goal is to efficiently monitor interactive applications, that is, applications that continuously interact with users. Since \CBR is \textit{user-oriented} we aim to monitor traces that start and finish with a user interaction.

Sampling-based techniques are useful to lower the monitoring overhead, since the amount of samples gathered from field are strongly reduced in a probabilistic way. In literature, sampling techniques have been widely used for isolating bugs \cite{Liblit:BugIsolation:SIGPLAN:2003,Jin:Sampling:SIGPLAN:2010}, runtime verification \cite{Bartocci:Adaptive:ICRV:2012,joshi2017runtime,BabaeeGF18} and bursty monitors \cite{Hirzel:BurstyTracing:FDDO:2001} (as described in Chapter \ref{chapter:related}).

\CBR has been designed based on the results obtained in the user studies presented in Chapter \ref{chapter:userstudy}. 
Interestingly, we discovered that users hardly perceive important overhead levels if introduced for a limited time (see Section \ref{sec:overheadTolerant}), in particular, we observed that even for overhead levels of 140\% users struggle to recognize variations in the system response time with the exception of some long lasting operations. 

\CBR leverages these results: since a significant overhead can often be tolerated by users, traces of non-trivial length might be feasibly collected from the field, but at the same time, since the impact of the monitoring activity changes with the operation that is executed, monitoring must be cleverly limited to prevent the introduction of an excessive overhead for specific operations.

Given \textit{EV} as the set of every possible event that can be produced by a monitored application, a trace 
$T = \langle e_1,e_2,...,e_n \rangle$, with $e_i \in \textit{EV}$, $i = 1\ldots n$ is an ordered sequence of events observed in the field. 

In order to obtain a comprehensive information about the sequentiality of the traces, we might collect state information at the moment the execution traces are collected in the field.  

All this knowledge can be represented as a Finite State Automaton, or \textit{FSA} for short, where the states represent the state of the monitored application and the transitions represent how the state of the application changes as a consequence of the execution of a user operation. 

Since several monitoring techniques in the literature collect method calls, eventually annotated with parameters or state information \cite{ohmann2017lightweight,Jin:BugRedux:ICSE:2012,joshi2007scarpe,prepost,Cornejo:Flexible:ICSEC:2017}, we also focus on the collection of this data type.

In a nutshell, \Controlled is an approach that combines chunks of execution recorded at different times to produce insights about the field behavior of the application. With this approach we might loss full ordering of the events in the \FSA model, but since we are going to record partial traces at different times of the execution we expect not to impact on the user experience.

In the following section, we present an overview of \Controlled and the main steps of the approach.

\subsection{Overview of the Technique}\label{sec:cbr_overview}

\begin{figure}[h!]
  \centering
    \includegraphics[width=\textwidth]{figures/CBR}
    \caption{Overview of \Controlled approach.}
    \label{fig:CBR}
\end{figure}

Figure \ref{fig:CBR} shows the steps that must be performed to apply \CBR. 

To start, practitioners indicate to \CBR the components they would like to monitor in the field. To extract data from the chosen components, \CBR identifies all the classes that may influence the usage of the components (step 1).

This analysis is done by first selecting a subset of the system (e.g., component) that has been defined as the monitoring goal and then by retrieving all the \textit{relevant classes} and their respective methods that exist inside the selected component, which is the result of step 1.

Given that \CBR has been designed to \textit{sample} executions from the field, in order to decrease monitoring overhead, we can use program state information to give a temporal context to the different traces by calculating the state of the program before and after the set of events observed in the field.

This state information should be accurate enough to recognize different application states between user inputs, and inexpensive enough to be obtained at runtime so it does not add too much monitoring overhead.

One way to represent the state of an application is to consider the set of values of all the variables at a certain moment \textit{t} during the execution. Certainly, acquiring this information is too expensive to be done at runtime.  
An efficient way to perform this operation, is to subset the number of variables and the amount of information \CBR should save for each variable while monitoring.

In the Function Extraction step (see Section \ref{sec:SD}), \CBR analyzes the relevant classes to distill the knowledge about the functions that may influence their execution, and thus influence the interaction with the monitored components. In particular, \CBR identifies a set of functions to be used to derive an abstract representation of the current state: we call the set of functions the \textit{Abstraction Functions}, or \textit{AF} for short.

The most intuitive way to derive the \AF, is to extract from the application's code the functions that the application uses to define its execution path according to the runtime value of the variables. \CBR will only consider those functions that helps to differentiate efficiently between different states at runtime. 

For instance, let us assume that the monitored components control the interaction with the file system: if a method \texttt{write} may actually write to a variable \texttt{file} only if its boolean variable \texttt{open}, which represents if the file has been already open or not, is true, 
the Function Extraction step would output the function \texttt{file.open == true} to indicate that the evaluation of this function may influence the interaction with the monitored components. 
In general, the \AF can capture important state information that could be useful to understand how the application under monitoring changes its state according to user inputs.

The \AF are systematically applied to concrete states of the application to produce an abstract representation of the program state to which they were applied: these representations are called \textit{Abstract Program States}, or \textit{APS} for short.

The \AF should have a proper balance in the abstraction level: too concrete functions can have bad implications, for instance checking all the field values of the program variables would be too expensive to be assessed at runtime (\textit{performance}). 
On the other side, too abstract functions could generate poor program states that are not useful to distinguish different states of the application while running in the field (\textit{precision}).

\smallskip

After having defined the \AF through an automatic extraction process (see Section \ref{sec:SD}), the monitor is then assembled: 
the monitoring component consists of the State Monitor and the Event Monitor. The State Monitor produces concrete values of the \AF at the beginning and at the end of each stream of events, and the Event Monitor collects the events associated with the component under monitoring.

To start using the State Monitor, we need to pass through a Training Phase (step 3) to produce the optimal set of functions for estimating a proper representation of the state of the program. These steps are described in details in Section \ref{sec:monitor}.

Then, in the field, \CBR uses the Abstraction Functions to produce a compact and relevant representation of the state of the program, immediately before and after a stream of events is recorded (step 4). 

A \textit{burst} is a stream of consecutive events collected in the field enriched with the state information at the beginning and at the end of each user action. 
In particular, a burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two \APS produced by the \AF and the trace $T$ is the sequence of events collected in the field.

Since \CBR is implemented as a sampling technique, the different bursts are collected probabilistically by turning on and off the monitor while running in the field.

The evaluation of the Abstraction Functions to a concrete state of the program during runtime (i.e., the \APS) is used within bursts to represent the state of the application at a certain point of the execution.

The collected bursts are then analyzed offline. The \APS at the beginning and at the end of each burst abstractly represent the state of the system at the time the trace was recorded. 
Since a program state directly depends on the conditions actually computed by the program while interacting with the monitored components, the \APS is representative of how the execution may proceed, specifically in terms of the interaction with the monitored components. 

In principle, a set of bursts might be used to form a Finite State Automaton, to show real uses of the application (step 5), where the edges of the \FSA represent the different user actions and the nodes represent the possible program states. Finite state automaton-based abstractions of software behavior are popular since they can be used as the basis for automated verification and validation techniques \cite{walkinshaw2008inferring}, such as detection of anomalous behaviors, protocol verification, testing, among others.

%%Literature on FSAs

The literature on synthesizing \FSAs that describe the behavior of a system is vast, some particularly relevant works include Wil van der Aalst's \cite{van2016process} book, entirely devoted to mining processes from observed data. 
Also, Lorenzoli et al. \cite{lorenzoli2008automatic} worked on \textit{GK-Tail}, a technique for automatically generating extended finite state machines from interaction traces. The technique focuses on the relations between constraints on data values on component interactions, retrieving more accurate models for analysis and testing techniques.
In the same direction, Krka et al. \cite{krka2010using} developed a \FSA inference technique that uses not only execution traces but also program invariants in order to obtain relevant internal state information of the program variables and to produce more reliable models. 
Recently, Walkinshaw et al. \cite{walkinshaw2016inferring} proposed an approach for inferring extended \FSAs from software executions, this work focuses on addressing the non-determinism and the inflexibility problem of automatically generated \FSAs.

Usually the functions that represent the values of the states of a \FSA are obtained automatically (e.g., \textit{Daikon} \cite{ernst2001dynamically}) or manually (e.g., written by practitioners). \Controlled introduces a new strategy for function extraction that is based on the actual software source code and should produce more precise and personalized \FSA models. 

To create the \FSA, we merge the different bursts collected in the field that have a common state, intuitively a burst that ends with a certain state can be concatenated with a burst that starts with the same abstract program state, because it represents two consecutive actions performed by the user in the application.

The main reason for generating these \FSA is representing the possible executions of an application, which may be useful to analyze the scenarios that may occur in the field.

\section{\Controlled Framework}\label{sec:CBR}

The most important activity performed by \CBR is the identification of the functions that are later used to represent the Abstract Program State, that is, a compact and abstract representation of the state at the time the collection of a burst is started or stopped.

In this section, we use a small example to present the different steps of \Controlled Framework. 

Consider a Java program that includes the \texttt{Cart} class (see Listing \ref{code:cart_class}), which represents a shopping cart of an online store. The \texttt{Cart} class implements four different methods and the \texttt{Product} inner class: 
the \texttt{addItem} method adds a \texttt{Product} object to the shopping cart, which is represented by an array of \texttt{Product} type,
the \texttt{emptyCart} method empties the shopping cart,
the \texttt{calculateTotal} method estimates the total price of all the products in the cart and
the \texttt{applyDiscount} method applies a discount to the total price.

Let us assume that we want to collect data about how a certain program uses the \texttt{Cart} class, focusing on the sequences of method calls produced by the program. Capturing every call to every method of the \texttt{Cart} class might be expensive for operations that extensively use the public methods implemented by the \texttt{Cart} class.

\JCODESTEP{code:cart_class}{Shopping Cart Class}{Cart.java}{1}

\subsection{Step 1: Classes Identification}

The \textit{Classes Identification} step produces the set of classes that directly or indirectly determine the sequence of invocations to the methods in the monitored component. To derive the set of classes, practitioners need to indicate the component(s) of interest within the application under monitoring. Since one of the goals of \CBR is to generate as little monitoring overhead as possible, it is important to include under the monitoring objective only those classes that are directly involved within the functionalities being monitored.

The set of classes is determined statically by extracting from the monitored component all the classes that exist inside the program.
Then, with the help of WALA \cite{WALA} static analysis tool, \CBR constructs the Class Hierarchy of the program under monitoring and extracts all the classes that match the scope of the monitoring. 

Later, we save the meta-data of all methods existing inside the classes we already gathered through the Class Hierarchy.

In our example, we are interested in understanding the behavior of the class \texttt{Cart}, so \CBR considers the \texttt{Cart} and its \texttt{Product} inner class for the analysis.

\subsection{Step 2: Function Extraction}\label{sec:SD}

\CBR uses the classes produced during the step 1 to extract the \textbf{Abstraction Functions} that represent how the value of the state variables that may influence the execution of the monitored program. These functions are exploited at runtime to record state information efficiently, that is, representing the state of the application with a proper abstraction level so we avoid performance and precision issues as stated in Section \ref{sec:cbr_overview}.
% abstractly with a limited risk of losing information relevant to the program.

The Abstraction Functions computed by the monitored program, and in particular the ones computed in the relevant classes, are a set of functions that can be naturally exploited to define an efficient abstraction strategy that can be applied at runtime to generate the program state.

\begin{figure}[h]
  \centering
    \includegraphics[width=0.9\textwidth]{figures/abstract_functions}
    \caption{Function Extraction process.}
    \label{fig:abstract_functions}
\end{figure} 

To extract the Abstraction Functions from the code (see Figure \ref{fig:abstract_functions}), we symbolically execute each method in each selected class and use the \textit{path conditions} resulting from the analysis of each method as functions for state abstraction. 
A \textit{path condition} is a condition on the state variables of a program, and the Abstraction Functions are the application of these conditions to the program state.

We use the JBSE \cite{Braione:Enhancing:FSE:2013} symbolic executor to compute the Abstraction Functions from the relevant classes, bounding the exploration of loops. 

Note that a \textit{path condition} represents how the inputs to a method, that is, the values of the parameters and the values of state variables, relate to the execution of a specific path inside the method. \textit{Path conditions} are a good abstraction because they show how applications use inputs and state variables.

For instance, the Abstraction Functions could be composed by a particular function that
checks if the number of products in a shopping cart is greater than zero to decide how to use the shopping cart,
in this case it would be enough to record whether the condition \texttt{nrProducts > 0} is true or not when saving state information, with no need of recording the actual number of products, which would be irrelevant to determine how the execution may proceed.

The Abstraction Functions capture relevant state properties and represent the different execution paths, that in turn may produce different sequences of invocations to the monitored classes.  
Each evaluation of these functions at runtime produces the program state of the application.

From our \texttt{Cart} class example, the resulting Abstraction Functions include the following functions for each method:

\JCODESTEP{code:addItem}{Functions for method addItem}{addItem_2.log}{1}

\JCODESTEP{code:applyDiscount}{Functions for method applyDiscount}{applyDiscount_1.log}{1}

\JCODESTEP{code:calculateTotal}{Functions for method calculateTotal}{calculateTotal_1.log}{1}

\JCODESTEP{code:emptyCart}{Functions for method emptyCart}{emptyCart_1.log}{1}

Applying the Abstraction Functions to a certain program state produces a compact vector of ternary values: the size of the vector depends on the number of functions that are evaluated and the values are the result of the evaluation of a function to the current program state. The result of the evaluation of a function can be True (T), False (F), and Unknown (U). The vector of ternary values is called the Abstract Program State. 

A single function evaluates to true if the values of the program variables at the time the function is evaluated satisfy the function. 
Similarly, a function evaluates to false if the values of the program variables at the time the function is evaluated do not satisfy the function. 
If some of the elements that appear in a function cannot be evaluated, for instance because an object with an attribute that should be considered in the evaluation of a function is null or even non existing, the function evaluates to unknown. 

From our example, the Function 1 in Listing \ref{code:addItem} for the method \texttt{addItem}:

\smallskip
\noindent \begin{small}\texttt{Cart.nProducts != 0 \&\& Cart.products.length >= 0}\end{small}
\smallskip

evaluates to true when there is more than one \texttt{Product} in the shopping cart, while it evaluates to false if the shopping cart is empty. Finally, it evaluates to unknown if the \texttt{Cart} object is not available.

In the other hand, for example the Function 4 in Listing \ref{code:applyDiscount} for the method \texttt{applyDiscount} :

\smallskip
\noindent \begin{small}\texttt{Cart.nProducts > 0 \&\& Cart.products.length > 0 \&\&} \newline\texttt{Cart.products.[0].value < Cart.PRICE}\end{small}
\smallskip

evaluates to true when the cart is not empty, and the price of the first \texttt{Product} in the cart is higher than the \texttt{PRICE} constant, evaluates to false whether the cart is empty or the price of the first \texttt{Product} is lower than the \texttt{PRICE} value, and evaluates to unknown when the object Cart does not exist in memory.

When the program under monitoring is executed, \CBR produces a number of bursts consisting of an evaluation of the extracted functions on the state of the program, a sequence of events (each event is a method invocation), and again an evaluation of the functions on the state of the program. 

The organization \texttt{state - burst - state} is useful, because allows \CBR to understand the sequentiality of bursts. Since the states give information about the current program state, it is possible to correlate different bursts collected at different times and compare their states' values, to obtain a more comprehensive knowledge rather than considering only one burst.

Considering the previous example of the program exploiting the \texttt{Cart} class, a burst of its execution could take the form:

\smallskip
\noindent \begin{small}\texttt{(U, U, F, T) addItem(product) calculateTotal() \ldots emptyCart() (T, T, F, T)}\end{small}
\smallskip

where the part between parentheses is the Abstract Program State, which includes the evaluation of every function identified in the function extraction analysis (T, F, U stand for true, false, and unknown, respectively), and the sequence of labels between the two instances of the Abstract Program State is the sequence of events collected at runtime.

Considering the initial Abstract Program State (i.e., the first \APS of the burst), let us assume that the first value refers to the mentioned Function 1 on the method \texttt{addItem}: the U in the program state means that, when the monitor started that trace recording, that function was evaluated as unknown, while at the end of the trace it turned to be true.

\subsection{Step 3: Training Phase}\label{sec:monitor}

The symbolic executor produces a large number of path conditions since it tries to assess every possible execution path for every method under analysis. Including all path conditions to represent the \AFs is not practical, since evaluating a high number of functions at every user interaction might introduce infeasible levels of overhead, and thus affecting the user experience. For this reason, we need to filter out the path conditions produced by the symbolic executor to reach a good compromise between the accuracy of the state information that is traced and the cost of producing such a state information.

From the original set of path conditions, we are interested in those giving unique information about the behavior of the application, that is, information that is not subsumed by the information checked by other functions. 
To find the optimal set of conditions, we need to go through a training phase that consists in empirically finding all the \AFs that are useful for distinguishing the different logical states of the program as identified by the functions themselves. 
In other words, we run the application with a monitor that assesses the complete set of \AFs returned by the symbolic executor to obtain the most representative result for the \AF.

In this training phase, we evaluate the \AF for every method call performed by the application, to clearly distinguish all different Abstract Program States at runtime.  

% \leo{total number of function evaluations (credo...)}

% $E = E_{ij}^1, E_{ij}^2, \ldots, E_{ij}^{}$

For each user execution $l$ we generate a matrix $E_{iJ}^l$, with $i = 1 \ldots k_l$ being $i$ a sample observed in the field with $k_l$ being the number of samples observed in the $l$-th execution, and $J = 1 \ldots n_{af}$ being $J$ the abstraction functions under observation and $n_{af}$ the total number of \AFs.
For instance, in Figure \ref{fig:samples} we show two examples of executions, with $n_{af} = 7$, collected in the field: Execution 1 ($E^1$) with $k_1 = 3$ and Execution 2 ($E^2$) with $k_2 = 2$. 

\vspace*{-0.5cm}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/samples}
\caption{Example of two executions collected in the field.}
\label{fig:samples}
\end{figure}

After collecting information for each execution, we organize the several $\{ E_{ij}^1, E_{ij}^2, \ldots, E_{ij}^{L} \}$ with $L$ the total number of executions, into a matrix $M_{ij}$, where $i$ (rows) ranges from $1$ to the sum of all samples 
$\sum_{l = 1}^L k_l$
gathered at runtime, while $j$ (columns) goes from $1$ to $n_{af}$.
The matrix $M_{ij}$ is obtained as $M = \{E^1 \diamond E^2 \diamond \ldots \diamond E^{L}\}$, where the $\diamond$ operator represents the vertical concatenation of the $E_{iJ}^l$ matrices.
For instance, considering $E^1$ and $E^2$ the executions of our example, the operation $E^1 \diamond E^2$ would generate the matrix presented in Figure \ref{fig:matrix}.

\vspace*{-0.5cm}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/matrix}
\caption{Vertical concatenation of executions $E^1$ and $E^2$.}
\label{fig:matrix}
\end{figure}

During the filtering process, we can apply four type of operations to the matrix $M$ in order to remove samples or \AFs.
Particularly, we identify four operations: \textit{Duplicated Sample}, \textit{Non-Discriminating Abstraction Function}, \textit{Equivalent Abstraction Function} and the \textit{Redundant Abstraction Function} operation.
In Figure \ref{fig:pc_filtering} we show an example of the filtering process and its several steps until we arrive to the reduced matrix, the example starts with the matrix generated in Figure \ref{fig:matrix}.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{figures/pc_filtering}
\caption{Example of filtering process of \AF.}
\label{fig:pc_filtering}
\end{figure}

\textit{Duplicated Sample} is the case in which two samples obtained the same value for all the \AFs. Formally, two samples $M_{I_{1}j}$ and $M_{I_{2}j}$ are duplicated if $M_{I_{1}j} = M_{I_{2}j}$ for all $j = 1 \ldots N$.
% in other words that two rows $i$ and $i+1$ in the matrix $M$ are equivalent for all the \AF such that $M_{ij} = M_{(i+1)j}$.

In our example, in the first matrix we identified Duplicated Samples, in fact Sample 2 and Sample 3 are identical $S_2 = S_3 = \{U, F, T, T, F, F, F\}$, in general we remove the second occurrence of a repeated column/row, so in this case we remove Sample 3. 

\textit{Non-Discriminating Abstraction Function} are those abstraction functions that do not change their values throughout the different samples and thus are not useful to distinguish the program states at runtime. More formally, an abstraction function $af_J$ is non-discriminating if $M_{1J} = M_{2J} = \ldots = M_{IJ}$
 % that exist a column $j$ in the matrix $M$ in which its value is always constant such that $M_{ij} = M_{(i+1)j} = \ldots = M_{mj}$. 

In the second matrix, it is possible to recognize two Non-Discriminating Abstraction Functions, in this case $AF_1$ and $AF_3$, because they always generated the values $U$ and $T$, respectively.

\textit{Equivalent Abstraction Function} is the case in which there are two abstraction functions always produce the same set of abstract values. More formally, two functions $af_I$ and $af_J$ are equivalent if their columns $M_{iI}$ and $M_{iJ}$ are the same, that is, $M_{iI} = M_{iJ}$ for all $i=1...M$.

%in other words, that exist two columns $j$ and $j+1$ in the matrix $M$ that are equivalent such that $M_{ij} = M_{i(j+1)}$.

In the example, it is possible to recognize two equivalent abstraction function, since the abstraction function values represented in column $AF_6$ are already present in column $AF_2$ ($AF_2 = AF_6 = \{U, F, F, F\}$), in this case we remove column $AF_6$.

Finally, the \textit{Redundant Abstraction Function} reduction is a heuristic step that aims to remove those \AFs that are not useful for identifying unique program states. The reduction procedure works by removing one abstraction function at a time and checking if the function was necessary to distinguish a unique program state. 
The procedure consists of removing one column $j$ of the matrix $M$ and applying the \textit{Duplicated Sample} procedure: 
if the number of rows of the new matrix is equivalent to the original matrix $M$, it means that the \textit{removed abstraction function j} is not useful for recognizing a unique program state, 
otherwise, if the number of rows of the new matrix is less than the matrix $M$ it means that the \textit{removed abstraction function} is actually useful and we then reincorporate it to the matrix $M$.

In our example, \CBR attempts first to remove the column $AF_2$. Since $AF_2$ is not useful, $AF_2$ is removed. Along with column $AF_2$, \CBR also removes $AF_4$.

\CBR performs these operations iteratively until it arrives to a minimal representation of the executions with respect to the different \AFs given by the symbolic executor: 
in this example the minimal set is composed by abstraction functions $AF_5, AF_7$ and executions $1, 2, 4$ and $5$.
These \AF are used to generate a monitor that is able to collect bursts during program executions. 

\subsection{Step 4: Bursts Collection}\label{sec:collect_bursts}

One possible way to decrease the overall monitoring overhead in the field is to collect data in a probabilistic way, that is, to record information about an event only under a certain probability.

From our human-subjects study presented in Chapter \ref{chapter:userstudy}, we discovered that for a few actions it is actually possible to monitor applications in the field without impacting the user experience. 
So it makes sense to collect data occasionally when a user performs an action. Also, the monitoring of each burst starts by recording as soon as the user interacts with the application and it stops when the software finishes processing the user request.

The collection of bursts is done probabilistically: since the technique traces bursts of the execution signed with program state information, we are not forced to record sequentially all bursts that occur in the field, that would correspond to continuously collect all the program execution interfering with the user activities. The program state information helps us to acquire a logical order of the different independent bursts collected at different times during different executions under monitoring.

The sampling probability of \CBR will be then estimated experimentally, testing with different probabilities to search for the best cost-benefit compromise in terms of quality of the solution.

% Given \textit{EV} as the set of every possible event that can be produced by a monitored application, a trace 
% $T = \langle e_1,e_2,...,e_n \rangle$, with $e_i \in \textit{EV}$, $i=1\ldots n$ is an ordered sequence of events observed in the field. 

Let $Abstraction$ be the \AF that applied to a certain concrete state $S$ of a program produces an Abstract Program State $S_a = Abstraction(S)$.

% A burst $B$ is given by a tuple $B = \langle label, S_1\,T\,S_2 \rangle$, where $label$ is the user action represented in $B$, $S_1$ and $S_2$ are two abstract program states produced by the \AF and the trace $T$ is the sequence of events collected in the field.

Following our example, some of the recorded bursts may for example look like:

\smallskip

\noindent \begin{small}\texttt{(U, F) cart.applyDiscount() cart.calculateTotal() \ldots (F, F)}\end{small}
\smallskip

When the action \textit{pay total} is performed, \CBR saves the \APS $(U, F)$ plus the target methods of the analysis, then \CBR saves again a new representation of the \APS equal to $(F, F)$.

\subsection{Step 5: \FSA Synthesis and Traces Simulation}\label{sec:simulating}

At this point, we already gathered several independent bursts from the field, where each burst explains the effect of each user action on the program state. 
The issue is that each burst by itself provides partial information about a full execution.
To overcome this issue, \CBR puts together all the bursts in a common structure. 

The right structure to assemble the different bursts is a \textit{Finite State Automaton}: in fact, a \FSA is a natural representation for traces with states and transitions. In our case, the \FSA will show how the application's state changes according to different users' inputs.

To decide how to synthesize the \FSA, \CBR exploits state information contained in the different bursts. 
That is, if a burst $B_1$ ends with an abstract program state $S_2$ that matches the abstract program state $S_1$ reported at the beginning of another burst $B_2$, then the two bursts $B_1$ and $B_2$ can be concatenated by a node containing the state information in common between both bursts.

The Finite State Automaton is a tuple $G = (S,M,s_0,s_F)$, 
where $S$ is a finite non-empty set of nodes representing the different \APS identified at the beginning and at the end of each burst,
$M$ is a finite set of transitions between states in $S$ representing the different user inputs monitored at runtime,
$s_0 \in S$ is the initial state, and $s_F \subset S$ is the set of final states.

So, for each monitored burst $B = \langle label, S_1\,T\,S_2 \rangle$, \CBR creates a transition $m \in M$ starting from state $S_1$ to $S_2$ with a specific label and a trace $T$. 
Since it is totally possible that different users perform the same action in different scenarios, \CBR enriches the transition $m$ with more traces $T$. 

% \leo{Inoltre devi dire come ogni elemento viene definito. Ad esempio il set di stati sara l'unione di tutti gli stati che occorrono all'inizio e fine dei burst. Poi per ogni burst <label, S1 T S2> creerai una transizione da S1 a S2 con etichetta label e annotazione T. Se ci sono piu burst con stesso valore di label S1 e S2 a questo punto l'annotazione viene arricchita con altri T}

The procedure of concatenating bursts is done iteratively for all bursts collected in the field. Certainly, as more bursts are used to create the graph, an increased number of program behaviors will be represented in it.

To simulate possible traces of the application we again exploit state information. 
Since we already built the \FSA as the tuple $G = (S,M,s_0,s_F)$, the procedure is straightforward: 
consider two transitions $m_1, m_2 \in M$ connected by a common state $S_1 \in S$, \CBR generates a new burst $B'$ with (1) the initial state $S_i$ of transition $m_1$, (2) a new trace $T'$ made by the concatenation of the trace $T_1$ from $m_1$ with the trace $T_2$ from $m_2$ and (3) the final state $S_f$ of transition $m_2$.
The new burst $B' = \langle label, S_i\,T'\,S_f \rangle$ contains the simulated trace represented by $T'$.
% for a certain state $S_k$ in $G$ we pickup an incoming $m_{in}$ and an outgoing transition $m_{out}$, from both transitions respectively we select the bursts $B_{incoming}$ and $B_{outgoing}$ and merge them by concatenating the traces $T_{incoming}$ inside $B_{incoming}$ with the events $T_{outgoing}$ inside burst $B_{outgoing}$. 

The idea is to repeat this process until a larger trace is created.

\begin{figure}[h]
\centering
\includegraphics[width=0.70\textwidth]{figures/burst_plus}
\caption{Example of simulation of traces.}
\label{fig:burst_plus}
\end{figure}

In Figure \ref{fig:burst_plus}, for our example we have two transitions: actions \textit{clickOnAddItem} and \textit{clickOnPay}, that have in common the \APS \texttt{(U, F)}. In this case, we might concatenate Bursts 1 and 2 and produce the following trace:

% \danyB{questa e' la parte che puo' generare tracce sbagliate giusto? lo accennerei qui per poi riprenerlo dopo nella valutazione}

\smallskip
\noindent \begin{small}\texttt{(U, U) cart.addItem(product1) \ldots cart.applyDiscount()\newline cart.calculateTotal()} \texttt{\ldots (F, F)}\end{small}
\smallskip

The generated traces could represent possible behaviors of the application, nevertheless if the quality of the model is not good, the procedure could derived unfeasible traces. This aspect will be covered in the next section.  

In a nutshell, \CBR provides useful information at two different levels:
(1) shows how the application is used in the field (\FSA) and 
(2) through the traces simulated by the \FSA shows different possible uses of the component under monitoring.

\subsubsection{\CBR model validity}\label{sec:precision}

For evaluating the validity of the \CBR model we consider two aspects: \textit{precision} and \textit{trace-level recall} of the traces generated by \CBR.

The building process and the semantics of the \FSA has a direct relationship with the precision of the technique. In some cases, it is possible that the generated traces are behaviors that do not occur in the field, which is the reason why we need to assess the precision of the generated \FSA.

Particularly, to evaluate precision we check if the traces produced by the \FSA model are possible outcomes of the application, in other words, we check if the derived traces from the \FSA model exists in the original trace.

The precision is evaluated first locally (i.e., \textit{node precision}) and then globally (i.e., \textit{overall node precision}), in other words, we first assess if the local decisions taken in each node of the \FSA are right. 
The assumption is that if on average the local decisions taken for each node are right, so the decisions taken globally by an execution derived from the model is also probably right.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/node}
\caption{\FSA node with state information and incoming and outgoing transitions.}
\label{fig:node}
\end{figure}

To assess \textit{node precision}, for each node present in the \FSA model we check that every possible sequence is a possible program behavior or not. 
For example, for the node in Figure \ref{fig:node} we first generate all the possible combinations of sequence of actions, that is, $A_1 \rightarrow B_1$, $A_1 \rightarrow B_2$, \ldots, $A_3 \rightarrow B_3$, then we verify if the traces produced by these sequences are present in the reworded traces, that is, traces recorded with a monitor that collects all the events sequentially.

The node precision for a particular node $i$ is estimated with the following formula:
\begin{equation}
	Precision(node_i) = \frac{CS_i}{TS_i}\label{eq:precision}
\end{equation}

where $CS_i$ is the amount of correct sequences for the node $i$ and $TS_i$ is the total of possible combinations of sequences for the node $i$.
The \textit{overall node precision} is obtained by estimating the mean \textit{node precision} of the \FSA model, for simplicity in the rest of the document we refer to \textit{overall node precision} simply as \textit{precision}.

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/completeness}
\caption{Recall validation process.}
\label{fig:recall}
\end{figure}

The \textit{trace-level recall} is assessed by estimating how complete are the traces generated by the technique with respect to the original trace. In the rest of the document we refer to \textit{trace-level recall} simply as \textit{recall}.

In particular, we incrementally consider the single events contained in the original trace, checking if the incremental trace is accepted by the \FSA (see Figure \ref{fig:recall}). We thus estimate the recall of the longest trace accepted by the \FSA model.

Particularly, the recall for a trace $j$ is estimated with the following formula:

\begin{equation}
	Recall(trace_j) = \frac{E_j}{EO_j}\label{eq:recall}
\end{equation}

where $E_j$ is the number of events contained in the generated trace $j$, and $EO_j$ is the number of events in the original trace representing the execution of trace $j$.

\subsubsection{Finite State Automaton Example}

Since the final step of the technique consists in generating a \FSA and then producing simulations of possible field executions, we show an example of a possible \FSA and how we assess the validity of the model.

Consider the GUI application for the shopping cart example of the previous sections that enables users to perform operations such as: adding items to the shopping cart, paying for all the items in the cart and starting a new session (emptying the shopping cart). 
If we monitor this application using \CBR with the \textit{Abstraction Functions} derived in the previous steps, we can for example collect the following bursts during an user execution (we show only methods related to the \texttt{Cart} class):

\JCODESTEP{code:log1}{Burst 1: clickOnAddItem}{log1.log}{1}

\JCODESTEP{code:log2}{Burst 2: clickOnAddItem}{log2.log}{1}

\JCODESTEP{code:log3}{Burst 3: clickOnPay}{log3.log}{1}

\JCODESTEP{code:log4}{Burst 4: clickOnStartNewSession}{log4.log}{1}

\JCODESTEP{code:log5}{Burst 5: clickOnStartNewSession}{log5.log}{1}

\begin{figure}[h]
\centering
\includegraphics[width=0.75\textwidth]{figures/fsa_example}
\caption{Example of resulting \FSA}
\label{fig:fsa_example}
\end{figure}

By following the procedure for joining the collected bursts in a \FSA, we could obtain the model shown in Figure \ref{fig:fsa_example}.

\JCODESTEP{code:trace1}{Trace 1}{trace1.log}{1}

\JCODESTEP{code:trace2}{Trace 2}{trace2.log}{1}

\JCODESTEP{code:trace3}{Trace 3}{trace3.log}{1}

We assess the validity of the model against traces 1, 2 and 3, represented respectively in Listings \ref{code:trace1}, \ref{code:trace2} and \ref{code:trace3}. These traces has been observed by a monitor that collects all the events in the field, so we highlight only the methods related to the \texttt{Cart} class. 

As described previously, to assess the validity of the model we first need to evaluate the precision of the \FSA. 
We use Equation \ref{eq:precision} to estimate the precision for nodes $PS\_0$, $PS\_1$ and $PS\_2$ in the \FSA. In particular, we check that all possible traces combination from nodes actually exist in traces 1, 2 or 3.

\begin{table}[h]
\centering
\caption{Precision for each node in the \FSA}
\label{table:fsa_precision_ex}
\begin{tabular}{ll}
\hline
\textbf{Node} & \textbf{Node precision} \\ \hline
$PS\_0$         &       100\%            \\ \hline
$PS\_1$         &       100\%            \\ \hline
$PS\_2$         &       100\%            \\ \hline
\end{tabular}
\end{table}

The reported precision for each node is shown in Table \ref{table:fsa_precision_ex}. The average precision of the \FSA is $100\%$.

We then use Equation \ref{eq:recall} to evaluate the recall of the traces produced through the \FSA. In other words, make sure that traces 1, 2 and 3 are a possible outcome of the model.

\begin{table}[h]
\centering
\caption{Recall of each trace generated by the \FSA}
\label{table:fsa_recall_ex}
\begin{tabular}{ll}
\hline
\textbf{Trace} & \textbf{Recall} \\ \hline
$Trace_1$         &       100\%            \\ \hline
$Trace_2$         &       100\%            \\ \hline
$Trace_3$         &       100\%            \\ \hline
\end{tabular}
\end{table}

The recall of each trace is reported in Table \ref{table:fsa_recall_ex}. The average recall of the traces produced from the \FSA is $100\%$.

Considering the values we achieved for \textit{precision} and \textit{recall}, we conclude that the \FSA presented in Figure \ref{fig:fsa_example} will produce trustful traces of high quality for the example.

However, if \CBR would identified a \textit{clickOnAddItem} action with a transition going from node $PS\_2$ to $PS\_0$, the node precision of node $PS\_2$ would be dropped to $50\%$, since the sequence of actions \textit{clickOnPay} followed by \textit{clickOnAddItem} was never observed in the field.

\section{Empirical Validation}\label{sec:empirical_cbr}

This Section presents the empirical validation we conducted for \Controlled, in order to assess the quality of the solution with respect to the performance, recall and precision in comparison to sampling techniques.
We provide information about the details of the experiments, the investigated aspects and the results we obtained for \CBR.

\subsection{Goal and Research Questions}

The goal of the experiment is to evaluate the performance, the precision and the recall of the traces produced by \Controlled, by comparing results with different approaches present in the literature.

With this experiment we aim to answer the following research questions:

\begin{itemize}
	\item \textbf{RQ1: What is the overhead introduced by \Controlled?} In this research question, we measure the performance of our technique with respect to other sampling techniques.

	\item \textbf{RQ2: What is the precision of the model generated by \Controlled?} In this research question, we measure the precision of the \FSA model with respect to the traces collected with monitoring.

	\item \textbf{RQ3: What is the recall of the traces produced by \Controlled?} In this research question, we measure the recall of the technique with respect to the monitored traces.
\end{itemize}

\subsection{Experiment Design}\label{sec:cbr_exp_design}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/experiment_design_4}
\caption{\Controlled Validation.}
\label{fig:experiment_design_4}
\end{figure}

Figure \ref{fig:experiment_design_4} shows the high-level work-flow of the experiment.
The main idea of the experiment is to compare \CBR to other sampling techniques, with respect to the performance, precision and recall of the technique itself. The monitoring objective is to collect the method calls related to a certain execution, including the runtime value of the parameters associated to each method call.

Sampling monitors have been used widely for monitoring applications in the field \cite{Jin:Sampling:SIGPLAN:2010,liblit2005scalable,joshi2017runtime,BabaeeGF18}: this type of monitors decrease the overall monitoring overhead by observing events only under a certain probability.
When analyzing interactive applications, each time the user interacts with the application the sampling monitor records with a certain probability. When the monitor is activated, it registers a defined amount of events.

For the experimentation, we implemented two sampling monitors, one with a sampling probability of $5\%$ and a second one with a $10\%$ of probability. Both sampling monitors trace a fixed number of events, in this case we fixed the amount to $30$ events per trace: a similar configuration setup has been used in \cite{Hirzel:BurstyTracing:FDDO:2001} for a sampling monitor.  

For assessing the \textit{performance} we measure execution times of a program being monitored with the three approaches compared to a program execution without any monitoring. 
The granularity of the monitoring is the single user action, that is to say measuring the execution time from the moment the user interacts with the application to the moment the program has finished processing the user request and gives a feedback to the user.
Since we care about how monitoring impacts on different functionalities, we analyze overhead with respect to the different categories of operations of the system response time categorization (see Chapter \ref{chapter:userstudy}).

To address the validity of the \CBR model we consider the procedure specified in Section \ref{sec:precision}: 
we assess \textit{precision} by applying Equation \ref{eq:precision} to every single node of the \FSA produced from the traces generated during the experimentation.   
Instead, we assess \textit{recall} by estimating how complete are the traces generated by each approach with respect to the original traces, in particular, we use Equation \ref{eq:recall} to calculate the Recall indicator of a certain trace.

\subsection{Experimental Subject}

To empirically answer the research questions, we use \Controlled to monitor ArgoUML \cite{ArgoUML:website:2018}.
ArgoUML is a UML diagramming application written in Java (389,952 lines of code): within the features of ArgoUML is possible to design Use Case, Class, Sequence, Collaboration, State-chart, Activity and Deployment diagrams. We selected ArgoUML because is a representative program of the target applications we are studying here: an user-interactive software application of medium-big size.

We considered the package \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small} as the target of monitoring, in particular, this package manages all the functionalities related to the design and management of activity diagrams in ArgoUML. We chose this package since activity diagrams are a very common way to represent behavioral information about software systems, so it is easy to make examples of this type of diagrams.

\subsubsection{Definition of the Abstract Program State}

% Since \CBR is a technique that consists in pre- and post-deployment operations, we first calibrate the tool to work with the program being analyzed. In particular, we define the corresponding representation of the Abstract Program State (see Section \ref{sec:SD}).

To define the Abstract Program State we start by doing static analysis of the component to be analyzed: Table \ref{table:target_jbse} offers some information about this process. 
To start, static analysis process discovered 16 classes and 199 methods inside component \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}, then the discovered methods are used as inputs to the symbolic executor, which processes each method and produce the corresponding abstraction functions. The symbolic executor produced 5,732 abstraction functions.

\begin{table}[h]
\caption{Monitoring Target and Symbolic Execution Outcome}
\label{table:target_jbse}
\begin{tabular}{|l|l|}
\hline
\textbf{Monitoring Target}                  & \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}        \\ \hline
\multirow{3}{*}{\textbf{Packages Analyzed}} & \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small}        \\ \cline{2-2} 
                                            & \begin{small}\texttt{org.argouml.uml.diagram.activity.layout}\end{small} \\ \cline{2-2} 
                                            & \begin{small}\texttt{org.argouml.uml.diagram.activity.ui}\end{small}     \\ \hline
\textbf{Classes Analyzed}            & 16                   \\ \hline
\textbf{Methods Analyzed}            & 199 	              \\ \hline
\textbf{Abstraction Functions}          & 5,732                \\ \hline
\end{tabular}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.55\textwidth]{figures/argouml_example}
\caption{Activity Diagram example in ArgoUML}
\label{fig:argouml_example}
\end{figure}

In order to recreate proper executions of ArgoUML we have written 30 automatically executable test cases that encode typical usage scenarios for \begin{small}\texttt{org.argouml.uml.diagram.activity}\end{small} component: each test case consists in simulating the drawing of one activity diagram on the application (e.g. diagrams such as Figure \ref{fig:argouml_example}). These 30 test cases are used along the calibration and experimentation process.
To avoid non-determinism and for reproducibility of the test cases we implemented them with the Sikulix \cite{sikulix} capture and replay tool.

To train and produce the optimal representation of the program state, we run the application with the monitor using the original 5,732 abstraction functions. Once we execute the 30 test cases, we produce a single log file with all the possible program states detected across the simulations. As specified in Section \ref{sec:monitor}, our technique filters out all the \textit{Non-Discriminating}, \textit{Equivalent} and \textit{Redundant} Abstraction Functions. 

\begin{table}[h]
\caption{Details from the abstraction function filtering process.}
\label{table:filtered_set}
\centering
\scriptsize
\begin{tabular}{ll}
\hline
 & \textbf{Number of Abstraction Functions} \\ \hline
Original Set from JBSE & 5,732 \\ \hline
\textit{Non-Discriminating Abstraction Function} & 1,631 \\ \hline
\textit{Equivalent Abstraction Function} & 2,646 \\ \hline
\textit{Redundant Abstraction Function} & 1,298 \\ \hline
\textbf{Filtered Set} & \textbf{157} \\ \hline
\end{tabular}
\end{table}

The result of the filtering process is shown in Table \ref{table:filtered_set}: the procedure filtered out 5,575 functions, leaving 157 \AF as the optimal representation for \APS. In particular, 
the \textit{Non-Discriminating Abstraction Functions} were 1,631,
the \textit{Equivalent Abstraction Functions} were 2,646 
and the \textit{Redundant Abstraction Functions} were 1,298. 

\section{Results}\label{sec:cbr_results}

In this section we present the results of the experiment we conducted to validate \Controlled. All the experiments were executed on a computer running macOS version 10.13.6 with a 3.1 GHz Intel Core i7 processor and 16 GB of RAM.

The following sections describe the results obtained to answer to the different research questions.

\subsection{Performance Results}

To answer the research question \textbf{RQ1: What is the overhead introduced by \Controlled?} we assessed the impact of the monitors, specifically we measured the overhead by comparing the execution times of the monitored version with those without monitoring.
Then, we ran our set of 30 test cases, each test has been repeated 3 times and mean values have been used to mitigate any effect due to the non-determinism of the execution environment. 
Overall, we collected near 3,459 samples about the execution time of actions.

In addition to measuring execution times, we collect the execution traces that will be useful for answering the research questions \textbf{RQ2} and \textbf{RQ3}.

Since this work is focused on understanding the impact of the monitoring on the user experience, we classify user actions according to its system response time category, in particular we used the categorization presented in Chapter \ref{chapter:userstudy} (i.e., Instantaneous, Immediate, Continuous and Captive actions).
Along the 30 test cases, we identified 915 actions of the Instantaneous category, 25 actions from the Immediate category and 213 actions from the Continuous category. Given the nature of the functionalities we tested, we did not identify Captive actions.

\begin{table}[h]
\centering
\caption{Performance results with respect to system response time categories.}
\label{table:performance_results}
\scriptsize
\begin{tabular}{llll}
\hline
 & \multicolumn{3}{c}{\textbf{Monitoring Overhead {[}\%{]}}} \\ \hline
\textbf{Monitoring Technique} & \textbf{Instantaneous} & \textbf{Immediate} & \textbf{Continuous} \\ \hline
\CBR & 123.78 & 40.70 & 0.71 \\ \hline
Sampling 1 (P: 10\%) & 17.03 & 4.65 & 1.37 \\ \hline
Sampling 2 (P: 5\%) & 7.12 & 2.88 & 0.28 \\ \hline
\end{tabular}
\end{table}

The results for performance can be found in Table \ref{table:performance_results}: specifically, we present overhead data for the different monitors used in the experimentation with respect to the different system response time categories. 

In the table, \CBR represents \Controlled, \textit{Sampling 1} the monitor that traces in a sampling way with 10\% probability and \textit{Sampling 2} the monitor that samples with 5\% probability.

The first thing we can notice is that for the actions categories that employ less than one second, i.e., Instantaneous and Immediate actions, \CBR introduces considerable more overhead than the other techniques, 123.78\% of \CBR compared to 17.03\% of Sampling 1, 7.12\% of Sampling 2 for Instantaneous actions, or the 40.70\% of \CBR compared to the 4.65\% and 2.88\% of Sampling 1 and 2 respectively for Immediate actions. 

The increased overhead for actions $< 1$ second is explained by the fact that \CBR, besides tracing events, needs to evaluate 157 conditions at the beginning and at the end of each action, plus the fact that Instantaneous and Immediate actions are volatile and very sensitive to any additional time.

The second thing we notice is that contrary to Instantaneous and Immediate actions, \CBR performs equally for actions $> 1$ second (i.e., Continuous actions), in fact \CBR introduced 0.71\% of overhead, which is similar to the performance of Sampling 1 (1.37\%) and Sampling 2 (0.28\%). Since these actions are less volatile, the task of evaluating program state does not impact on the final overhead.

However, from our human-subject studies results (see Section \ref{sec:results}) we discovered that users do not perceive high monitoring overhead levels for Instantaneous actions, and that users perceive a degradation of the system response time only at 140\% for Immediate actions, meaning that in practice, users would not perceive monitoring overhead when \Controlled is activated.

Moreover, Sampling 1 and 2 techniques are not useful for simulating possible executions from the field, since they are observing only small percentages from the execution and do not provide contextual information, while \CBR is capable of representing comprehensive behaviors from the traces signed with program state information.

\subsection{Precision Results}\label{sec:acc_results}

For answering the research question \textbf{RQ2: What is the precision of the model generated by \Controlled?} we measured the precision of each node when simulating possible traces from the \FSA generated by \Controlled.

\input{tables/accuracy_results}
\input{tables/completeness_results}

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{figures/accuracy_results}
\caption{Precision results with respect to different runs of the application.}
\label{fig:precision_results}
\end{figure}

We show results only for \CBR, since it is the only technique in this work that simulates possible execution traces, meaning that the precision of the traces recorded by sampling monitors is 100\%.

Table \ref{table:accuracy_results} and Figure \ref{fig:precision_results} show information about precision of \CBR given the sampling probability and the amount of runs of the application. 

As explained in Section \ref{sec:collect_bursts}, \CBR works in a probabilistic way, meaning that the monitoring of each interaction between the user and the application occurs only under a certain probability. 
If \CBR is deployed to monitor data with a probability lower than 100\%, it is necessary to run several times the same functionality in order to observe the whole behavior in the field. 
Since in practice a program is executed several times in different instances, we would observe several repeated observations of the same functionality throughout the monitoring process, and by increasing the number of runs of the monitor fewer samples will be needed in order to derive accurate results.

In Table \ref{table:accuracy_results} we present how the overall precision changes according to the number of observed runs of the application, in this case, we experimented with 1, 5, 10, 15 and 20 runs.

First, we observe that the maximum precision of the technique is around 81\%, this means that for every node in the \FSA, 81\% of the possible combinations of bursts are a feasible behavior of the application, while the remaining 19\% are traces that we never observed in the traces recorded when activating \CBR all the times. 

However, not all the 19\% are unfeasible traces: a subset of the traces represented by the remaining 19\% could still be possible behaviors of the software (e.g., we do not developed all the necessary test cases to cover the remaining 19\%).

Second, we note that with 5 runs of the application we achieve the maximum of the precision for our technique with a sampling probability of 50\%. 
Instead, when considering 10, 15 or even 20 runs, the maximum precision can be achieved with a 25\% sampling probability, which seems to be the more balanced result for all measurements.

Nevertheless, considering 5, 10, 15 or 20 runs are a very small number of executions in comparison to running the application thousands of times across the several instances in the field. Hence, taking into account thousands of samples for a same user action would allow us to considerably reduce the \CBR sampling probability.

\subsection{Recall Results}

\begin{figure}[h]
\centering
\includegraphics[width=0.85\textwidth]{figures/completeness_results}
\caption{Recall results with respect to different runs of the application.}
\label{fig:recall_results}
\end{figure}

In this section, we present results for the research question \textbf{RQ3: What is the recall of the traces produced by \Controlled?}. 
As stated in Section \ref{sec:cbr_exp_design}, to estimate the recall we measure the percentage covered by traces obtained with each monitor in comparison to those obtained with \CBR monitor activated all the time.

For \Controlled we present both in Table \ref{table:recall_results} and Figure \ref{fig:recall_results} the recall of the technique according to the sampling probability and how it changes according to the number of runs of the application. The recall is presented in two measures, the \textbf{RB} and \textbf{RE} indicators: 
the \textbf{RB} indicator shows the recall percentage with respect to the number of bursts that can be identified within the original traces in comparison to the simulated trace.
Instead, the \textbf{RE} indicator shows the recall percentage with respect to the number of events that can be identified in the original traces in comparison to the trace simulated by the \FSA.

We notice that considering only one run of the application we only achieve 100\% recall with sampling strategy at 100\%, which means having the monitor always on. When we decrease the sampling probability to 90\%, the recall of the technique decreases rapidly to 36\%. 

Given that we are considering only one run, it is very likely that our \FSA is missing several transitions and thus producing very short and incomplete traces. In fact, when considering 5 runs of the application it is possible to achieve a good recall percentage with 65\% of sampling probability.

Now, if we consider 10 runs of the application we obtain approximately $90\%$ of recall at a 45\% of sampling probability. Going further, for 20 runs of the applications we already obtain a good recall level for 25\%. Which is also a similar result obtained for precision in Section \ref{sec:acc_results}.

On the other side, for sampling monitors we obtained a recall value of 4.15\%, with a maximum recall of 7.77\%, meaning that the traces collected by this approach contains on average 4.15\% events from the total events contained in the traces obtained when activating \CBR all the times. 

\section{Discussion}\label{sec:cbr_discussion}

We have carried out an experimental evaluation for assessing the quality of \CBR in terms of monitoring \textit{performance} with respect to other two sampling approaches. 

Since \CBR works in a probabilistic way and does not trace full executions, we also assessed the \textit{precision} and the \textit{recall} of the traces simulated by \CBR, to understand the usefulness of the sampling approach in an attempt to decrease monitoring overhead and to reduce the impact on the user environment.

When assessing performance, we discovered that the monitoring overhead introduced by \CBR with respect to other sampling approaches was higher for user actions employing less than one second, and similar for those user actions employing more than one second.

However, by considering our earlier results obtained in Chapter \ref{chapter:userstudy} about the impact of monitoring overhead on the user experience, we conclude that \CBR would not be perceived by users, since the overhead introduced by the technique is always lower than 140\%, which is the limit for tolerating monitoring overhead in the users' environment, while allowing the technique to obtain traces with enriched information for generating more comprehensive knowledge of the application usage.

About the quality of the traces produced by \CBR, we discovered that the precision of the simulations we produced were 81\% with respect to the original traces.
Unfortunately, our experimentation was not enough to prove if the remaining 19\% were actually infeasible behaviors or they were simply unobserved behaviors of the application.

On the other side, \CBR was able to simulate traces that were 100\% complete with respect to the original traces. A very different result compared to the 4\% recall obtained by the other sampling approaches.  

Nevertheless, we noticed that by using a sampling rate fixed to 25\% was possible for \CBR to reproduce safe traces that represent reliable behaviors of field executions.
We are also aware that by increasing the amount of users, that is, increasing the monitored executions, we might considerably decrease the sampling rate to make \CBR a less expensive solution.

We also discovered the importance of adding state information to traces: as a matter of fact by using the \CBR monitoring approach we were able to observe complete user executions, while other sampling approaches not employing state information only observed small percentages of the user execution.

In the overall, \CBR is a good monitoring approach that can be used for constructing and simulating knowledge from field executions without impacting on the user experience.



==> esempio.tex <==

% \oscar{I would not include the following section...}
% \begin{TBR}
% \subsubsection{Finite State Automaton Example}

% Since the final step of the technique consists in generating a \FSA and then producing simulations of possible field executions, we show an example of a possible \FSA and how we assess the validity of the model.

% Consider the GUI application for the shopping cart example of the previous sections that enables users to perform operations such as: adding items to the shopping cart, paying for all the items in the cart and starting a new session (emptying the shopping cart). 
% If we monitor this application using \CBR with the \textit{Abstraction Functions} derived in the previous steps, we can for example collect the following bursts during an user execution (we show only methods related to the \texttt{Cart} class):

% \JCODESTEP{code:log1}{Burst 1: clickOnAddItem}{log1.log}{1}

% \JCODESTEP{code:log2}{Burst 2: clickOnAddItem}{log2.log}{1}

% \JCODESTEP{code:log3}{Burst 3: clickOnPay}{log3.log}{1}

% \JCODESTEP{code:log4}{Burst 4: clickOnStartNewSession}{log4.log}{1}

% \JCODESTEP{code:log5}{Burst 5: clickOnStartNewSession}{log5.log}{1}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.75\columnwidth]{figures/fsa_example}
% \caption{Example of resulting \FSA}
% \label{fig:fsa_example}
% \end{figure}

% By following the procedure for joining the collected bursts in a \FSA, we could obtain the model shown in Figure~\ref{fig:fsa_example}.

% \JCODESTEP{code:trace1}{Trace 1}{trace1.log}{1}

% \JCODESTEP{code:trace2}{Trace 2}{trace2.log}{1}

% \JCODESTEP{code:trace3}{Trace 3}{trace3.log}{1}

% We assess the validity of the model against traces 1, 2 and 3, represented respectively in Listings~\ref{code:trace1},~\ref{code:trace2} and~\ref{code:trace3}. These traces has been observed by a monitor that collects all the events in the field, so we highlight only the methods related to the \texttt{Cart} class. 

% As described previously, to assess the validity of the model we first need to evaluate the precision of the \FSA. 
% We use the $Precision$ equation to estimate the precision for nodes $PS\_0$, $PS\_1$ and $PS\_2$ in the \FSA. In particular, we check that all possible traces combination from nodes actually exist in traces 1, 2 or 3.

% \begin{table}[h]
% \centering
% \caption{Precision for each node in the \FSA}
% \label{table:fsa_precision_ex}
% \begin{tabular}{ll}
% \hline
% \textbf{Node} & \textbf{Node precision} \\ \hline
% $PS\_0$         &       100\%            \\ \hline
% $PS\_1$         &       100\%            \\ \hline
% $PS\_2$         &       100\%            \\ \hline
% \end{tabular}
% \end{table}

% The reported precision for each node is shown in Table~\ref{table:fsa_precision_ex}. The average precision of the \FSA is $100\%$.

% We then use the $Recall$ equation to evaluate the recall of the traces produced through the \FSA. In other words, make sure that traces 1, 2 and 3 are a possible outcome of the model.

% \begin{table}[h]
% \centering
% \caption{Recall of each trace generated by the \FSA}
% \label{table:fsa_recall_ex}
% \begin{tabular}{ll}
% \hline
% \textbf{Trace} & \textbf{Recall} \\ \hline
% $Trace_1$         &       100\%            \\ \hline
% $Trace_2$         &       100\%            \\ \hline
% $Trace_3$         &       100\%            \\ \hline
% \end{tabular}
% \end{table}

% The recall of each trace is reported in Table~\ref{table:fsa_recall_ex}. The average recall of the traces produced from the \FSA is $100\%$.

% Considering the values we achieved for \textit{precision} and \textit{recall}, we conclude that the \FSA presented in Figure~\ref{fig:fsa_example} will produce trustful traces of high quality for the example.

% However, if \CBR would identified a \textit{clickOnAddItem} action with a transition going from node $PS\_2$ to $PS\_0$, the node precision of node $PS\_2$ would be dropped to $50\%$, since the sequence of actions \textit{clickOnPay} followed by \textit{clickOnAddItem} was never observed in the field.
% \end{TBR}

==> tables/accuracy_results.tex <==
% !TEX root =  ../main.tex
\begin{table}[h]
\centering
\scriptsize
\caption{Precision results for \CBR.}
\label{table:accuracy_results}
\begin{tabular}{llllll}
\hline
 & \textbf{1 run} & \textbf{5 runs} & \textbf{10 runs} & \textbf{15 runs} & \textbf{20 runs} \\ \hline
\textbf{Probability {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} & \textbf{P {[}\%{]}} \\ \hline
5 & 0 & 66.67 & 68.42 & 70.21 & 68.11 \\ \hline
10 & 50.00 & 68.42 & 63.39 & 72.51 & 74.22 \\ \hline
15 & 100 & 70.73 & 72.36 & 76.62 & 78.83 \\ \hline
20 & 66.00 & 65.24 & 79.98 & 77.80 & 79.70 \\ \hline
25 & 55.35 & 66.67 & 80.27 & 79.97 & 80.43 \\ \hline
30 & 47.83 & 72.10 & 81.15 & 80.34 & 80.55 \\ \hline
35 & 38.89 & 79.61 & 80.83 & 81.22 & 80.25 \\ \hline
40 & 72.73 & 75.89 & 79.84 & 80.52 & 81.02 \\ \hline
45 & 64.62 & 79.95 & 80.55 & 80.62 & 79.88 \\ \hline
50 & 72.92 & 80.89 & 80.75 & 80.57 & 81.12 \\ \hline
55 & 65.87 & 80.16 & 80.66 & 80.62 & 80.39 \\ \hline
60 & 65.88 & 80.00 & 80.29 & 81.17 & 80.20 \\ \hline
65 & 66.82 & 80.98 & 80.52 & 80.43 & 79.92 \\ \hline
70 & 71.55 & 80.38 & 80.57 & 80.66 & 80.34 \\ \hline
75 & 78.14 & 80.41 & 80.89 & 80.75 & 80.48 \\ \hline
80 & 74.44 & 80.43 & 80.48 & 81.23 & 80.56 \\ \hline
85 & 75.23 & 81.23 & 81.07 & 80.48 & 80.41 \\ \hline
90 & 78.69 & 80.98 & 80.66 & 79.98 & 80.70 \\ \hline
95 & 79.52 & 80.70 & 80.75 & 81.02 & 80.49 \\ \hline
100 & 80.71 & 80.70 & 80.70 & 80.66 & 81.21 \\ \hline
\end{tabular}
\end{table}

==> tables/completeness_results.tex <==
% !TEX root =  ../main.tex
\begin{table*}[!ht]
\scriptsize
\centering
\caption{Recall results for \CBR.}
\label{table:recall_results}
	\begin{tabular}{lllllllllll}
		\hline
		 & \multicolumn{2}{c}{\textbf{1 run}} & \multicolumn{2}{c}{\textbf{5 runs}} & \multicolumn{2}{c}{\textbf{10 runs}} & \multicolumn{2}{c}{\textbf{15 runs}} & \multicolumn{2}{c}{\textbf{20 runs}} \\ \hline
		\textbf{P [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} & \textbf{RB [\%]} & \textbf{RE [\%]} \\ \hline
		5  & 4.68  & 3.95  & 9.70  & 8.99   & 13.53 & 12.18 & 16.66 & 16.58 & 22.62 & 20.78 \\ \hline
		10 & 5.41  & 4.78  & 13.06 & 11.50  & 21.82 & 21.25 & 28.48 & 28.30 & 38.47 & 41.32 \\ \hline
		15 & 7.24  & 6.13  & 18.34 & 16.61  & 31.57 & 32.34 & 47.33 & 47.91 & 61.56 & 63.85 \\ \hline
		20 & 8.53  & 5.83  & 22.86 & 21.93  & 42.17 & 43.43 & 63.36 & 64.35 & 84.64 & 86.36 \\ \hline
		25 & 9.37  & 7.36  & 29.16 & 27.73  & 49.41 & 51.47 & 75.33 & 78.44 & 95.93 & 96.97 \\ \hline
		30 & 11.74 & 10.20 & 32.25 & 33.05  & 67.65 & 70.82 & 92.02 & 92.14 & 96.89 & 96.89 \\ \hline
		35 & 11.46 & 9.71  & 39.47 & 42.39  & 86.66 & 88.36 & 100 	& 100 	& 100 	& 100 \\ \hline
		40 & 14.32 & 12.21 & 42.65 & 44.97  & 84.80 & 85.45 & 100 	& 100 	& 100 	& 100 \\ \hline
		45 & 15.12 & 11.34 & 67.06 & 68.73	& 98.70 & 98.75 & 100 	& 100 	& 100 	& 100 \\ \hline
		50 & 15.59 & 14.31 & 61.44 & 62.82 	& 98.70 & 99.19 & 100 	& 100 	& 100 	& 100 \\ \hline
		55 & 17.56 & 17.44 & 87.95 & 88.89  & 98.59 & 99.14 & 100 	& 100 	& 100 	& 100 \\ \hline
		60 & 19.29 & 19.55 & 77.51 & 78.87  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		65 & 23.89 & 23.60 & 90.84 & 91.05  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		70 & 26.21 & 25.84 & 98.78 & 99.01  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		75 & 28.31 & 27.08 & 98.99 & 99.23  & 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		80 & 31.80 & 33.93 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		85 & 31.80 & 33.93 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		90 & 36.60 & 39.44 & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
		95 & 57.47 & 59.96 & 100   & 100 	& 100 	& 100 	& 100 	& 100  	& 100 	& 100 \\ \hline
		100 & 100  & 100   & 100   & 100 	& 100 	& 100 	& 100 	& 100 	& 100 	& 100 \\ \hline
	\end{tabular}
\end{table*}
